Risk of Bitcoin Market: Volatility, Jumps, and Forecasts

Cryptocurrency, the most controversial and simultaneously the most interesting asset, has attracted many investors and speculators in recent years. The visibly significant market capitalization of cryptos also motivates modern financial instruments such as futures and options. Those will depend on the dynamics, volatility, or even the jumps of cryptos. We provide a comprehensive investigation of the risk dynamics of the Bitcoin Market from a realized volatility perspective. The Bitcoin market is extremely risky in the sense of volatility, entangled jumps, and extensive consecutive jumps, which reflect the major incidents worldwide. Empirical study shows that the lagged realized variance increases the future realized variance, while the jumps, especially positive ones, significantly reduce future realized variance. The out-of-sample forecasting model reveals that, in terms of forecasting accuracy and utility gain, investors interested in the long-term realized variance benefit from explicitly modelling the jumps and signed estimators, which is unnecessary for the short-term realized variance forecast.

==> AdaptiveHAR_Results.tex <==



% BTC-D, Square 1-day horizon

% All Jumps

h=1

{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.267 & 0.227 & 0.240 & 0.224 &  0.214 & 0.276 &  0.198 &   0.165 \\
MSE    & 3.636 & 4.023 & 3.983 & 4.113 &  4.069 & 3.807 &  4.855 &   4.832 \\
HRMSE  & 1.569 & 2.031 & 1.577 & 1.792 &  1.737 & 1.768 &  1.845 &   1.757 \\
QLIKE  & 0.846 & 1.151 & 1.101 & 1.000 &  1.172 & 0.988 &  1.176 &   1.545 \\


h=7
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.365 & 0.360 & 0.393 & 0.435 &  0.471 & 0.413 &  0.500 &   0.458 \\
MSE    & 1.643 & 1.795 & 1.605 & 1.610 &  1.291 & 1.763 &  1.479 &   1.280 \\
HRMSE  & 1.359 & 1.646 & 1.284 & 1.361 &  1.303 & 1.460 &  1.248 &   1.279 \\
QLIKE  & 0.984 & 1.146 & 0.998 & 1.026 &  0.996 & 1.038 &  0.881 &   1.043 \\

h=30
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.536 & 0.572 & 0.653 & 0.685 &  0.601 & 0.602 &  0.707 &   0.652 \\
MSE    & 0.698 & 0.690 & 0.561 & 0.476 &  0.629 & 0.577 &  0.444 &   0.490 \\
HRMSE  & 0.781 & 0.639 & 0.620 & 0.531 &  0.534 & 0.704 &  0.490 &   0.452 \\
QLIKE  & 0.937 & 0.944 & 0.899 & 0.849 &  0.884 & 0.878 &  0.843 &   0.875 \\



% BTC-D, Log， 1-day horizon

% All Jumps

h=1
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.299 & 0.264 & 0.287 & 0.204 &  0.265 & 0.289 &  0.194 &   0.241 \\
MSE    & 3.260 & 3.419 & 3.356 & 4.082 &  3.501 & 3.313 &  4.416 &   3.680 \\
HRMSE  & 0.760 & 0.893 & 0.822 & 0.969 &  0.898 & 0.807 &  1.031 &   0.937 \\
QLIKE  & 0.902 & 0.950 & 0.972 & 0.903 &  0.956 & 0.920 &  0.986 &   1.085 \\

h=7
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.327 & 0.329 & 0.297 & 0.323 &  0.404 & 0.318 &  0.305 &   0.364 \\
MSE    & 1.576 & 1.649 & 2.214 & 1.999 &  2.024 & 1.800 &  2.361 &   2.098 \\
HRMSE  & 0.881 & 1.209 & 0.926 & 1.069 &  1.093 & 1.099 &  1.047 &   0.991 \\
QLIKE  & 0.946 & 1.008 & 0.949 & 0.919 &  0.907 & 0.947 &  0.909 &   0.932 \\


h=30
{} &   HAR &   RVJ &   RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.496 & 0.533 &  0.125 & 0.583 &  0.463 & 0.550 &  0.617 &   0.503 \\
MSE    & 0.759 & 0.750 & 21.321 & 0.571 &  1.368 & 0.664 &  0.533 &   1.064 \\
HRMSE  & 0.630 & 0.498 &  1.049 & 0.693 &  0.689 & 0.548 &  0.462 &   0.485 \\
QLIKE  & 0.966 & 0.936 &  0.916 & 0.901 &  0.895 & 0.886 &  0.873 &   0.881 \\




% BTC-G, Square 1-day horizon

% All Jumps

h=1
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.213 & 0.179 & 0.182 & 0.182 &  0.190 & 0.226 &  0.144 &   0.151 \\
MSE    & 2.437 & 2.537 & 2.508 & 2.682 &  2.580 & 2.411 &  2.943 &   2.872 \\
HRMSE  & 1.976 & 2.251 & 2.080 & 2.497 &  2.385 & 2.022 &  2.762 &   2.583 \\
QLIKE  & 0.749 & 1.418 & 1.636 & 3.367 &  2.406 & 1.139 &  3.548 &   4.706 \\


h=7
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.355 & 0.347 & 0.360 & 0.405 &  0.420 & 0.423 &  0.409 &   0.425 \\
MSE    & 0.990 & 0.912 & 0.889 & 0.951 &  0.845 & 0.880 &  1.061 &   0.848 \\
HRMSE  & 1.278 & 1.434 & 1.366 & 1.252 &  1.306 & 1.050 &  1.432 &   1.626 \\
QLIKE  & 0.797 & 1.152 & 1.341 & 1.819 &  1.618 & 0.879 &  1.681 &   1.739 \\

h=30
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.623 & 0.664 & 0.681 & 0.676 &  0.680 & 0.695 &  0.777 &   0.806 \\
MSE    & 0.339 & 0.266 & 0.260 & 0.285 &  0.256 & 0.253 &  0.199 &   0.156 \\
HRMSE  & 0.699 & 0.611 & 0.554 & 0.495 &  0.489 & 0.531 &  0.462 &   0.406 \\
QLIKE  & 0.771 & 0.725 & 0.743 & 0.728 &  0.755 & 0.723 &  0.716 &   0.741 \\

% BTC-G, Log， 1-day horizon

% All Jumps

h=1
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.261 & 0.221 & 0.218 & 0.238 &  0.249 & 0.266 &  0.243 &   0.235 \\
MSE    & 2.217 & 2.329 & 2.353 & 2.284 &  2.260 & 2.209 &  2.262 &   2.298 \\
HRMSE  & 0.979 & 0.986 & 1.004 & 1.167 &  1.118 & 0.985 &  1.161 &   1.143 \\
QLIKE  & 0.906 & 0.998 & 1.017 & 1.056 &  1.074 & 0.945 &  1.112 &   1.170 \\


h=7
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.329 & 0.281 & 0.264 & 0.157 &  0.277 & 0.352 &  0.162 &   0.102 \\
MSE    & 0.949 & 1.015 & 1.049 & 2.535 &  1.360 & 0.955 &  3.445 &   4.699 \\
HRMSE  & 0.908 & 0.906 & 1.000 & 1.115 &  0.936 & 0.888 &  2.753 &   4.107 \\
QLIKE  & 0.906 & 0.909 & 1.002 & 1.004 &  1.012 & 0.929 &  0.951 &   0.981 \\

h=30
{} &   HAR &   RVJ &  RVTJ &  RVSJ &  RVSTJ &   SRV &  SRVSJ &  SRVSTJ \\
\midrule
M-Z-R2 & 0.568 & 0.593 & 0.598 & 0.510 &  0.453 & 0.609 &  0.509 &   0.504 \\
MSE    & 0.393 & 0.364 & 0.395 & 0.601 &  0.942 & 0.344 &  0.639 &   0.878 \\
HRMSE  & 0.589 & 0.523 & 0.561 & 0.524 &  0.534 & 0.516 &  0.464 &   0.467 \\
QLIKE  & 0.775 & 0.733 & 0.748 & 0.729 &  0.741 & 0.745 &  0.718 &   0.731 \\


==> DM_test.tex <==

h=1, square form

MSE:
(('HAR', 'RVJ')   , (-0.755, 0.45)) (('HAR' , 'RVJ')   , (-2.208, 0.028))
(('HAR', 'RVTJ')  , (-0.537, 0.592)) (('HAR', 'RVTJ')  , (-0.836, 0.403))
(('HAR', 'RVSJ')  , (-1.318, 0.188)) (('HAR', 'RVSJ')  , (-1.608, 0.108))
(('HAR', 'RVSTJ') , (-0.734, 0.463)) (('HAR', 'RVSTJ') , (-1.701, 0.089))
(('HAR', 'SRV')   , (0.197 , 0.844)) (('HAR', 'SRV')   , (-0.186, 0.853))
(('HAR', 'SRVSJ') , (-1.887, 0.06)) (('HAR' , 'SRVSJ') , (-2.318, 0.021))
(('HAR', 'SRVSTJ'), (-1.791, 0.074)) (('HAR', 'SRVSTJ'), (-3.15 , 0.002))

HRMSE:
(('HAR', 'RVJ')   , (-3.126, 0.002)) (('HAR', 'RVJ')   , (-2.185, 0.029))
(('HAR', 'RVTJ')  , (-0.083, 0.934)) (('HAR', 'RVTJ')  , (-1.581, 0.114))
(('HAR', 'RVSJ')  , (-2.926, 0.004)) (('HAR', 'RVSJ')  , (-2.771, 0.006))
(('HAR', 'RVSTJ') , (-2.009, 0.045)) (('HAR', 'RVSTJ') , (-2.601, 0.009))
(('HAR', 'SRV')   , (-2.366, 0.018)) (('HAR', 'SRV')   , (-0.533, 0.594))
(('HAR', 'SRVSJ') , (-2.792, 0.005)) (('HAR', 'SRVSJ') , (-3.113, 0.002))
(('HAR', 'SRVSTJ'), (-1.837, 0.067)) (('HAR', 'SRVSTJ'), (-3.369, 0.001))


QLIKE:

(('HAR', 'RVJ')   , (-3.032, 0.003)) (('HAR', 'RVJ')   , (-3.11 , 0.002))
(('HAR', 'RVTJ')  , (-3.77 , 0.0)) (('HAR'  , 'RVTJ')  , (-3.217, 0.001))
(('HAR', 'RVSJ')  , (-2.561, 0.011)) (('HAR', 'RVSJ')  , (-4.402, 0.0))
(('HAR', 'RVSTJ') , (-3.145, 0.002)) (('HAR', 'RVSTJ') , (-5.066, 0.0))
(('HAR', 'SRV')   , (-2.291, 0.022)) (('HAR', 'SRV')   , (-2.101, 0.036))
(('HAR', 'SRVSJ') , (-4.204, 0.0)) (('HAR'  , 'SRVSJ') , (-4.002, 0.0))
(('HAR', 'SRVSTJ'), (-2.742, 0.006)) (('HAR', 'SRVSTJ'), (-5.908, 0.0))








h=1, log form

MSE:
(('HAR', 'RVJ')   , (-2.2  , 0.028)) (('HAR', 'RVJ')   , (-1.918, 0.055))
(('HAR', 'RVTJ')  , (-0.376, 0.707)) (('HAR', 'RVTJ')  , (-2.088, 0.037))
(('HAR', 'RVSJ')  , (-1.813, 0.07)) (('HAR' , 'RVSJ')  , (-0.442, 0.659))
(('HAR', 'RVSTJ') , (-0.711, 0.477)) (('HAR', 'RVSTJ') , (-0.242, 0.809))
(('HAR', 'SRV')   , (-0.437, 0.662)) (('HAR', 'SRV')   , (0.108 , 0.914))
(('HAR', 'SRVSJ') , (-1.819, 0.069)) (('HAR', 'SRVSJ') , (-0.307, 0.759))
(('HAR', 'SRVSTJ'), (-1.121, 0.263)) (('HAR', 'SRVSTJ'), (-0.483, 0.63))


HRMSE:
(('HAR', 'RVJ')   , (-2.719, 0.007)) (('HAR', 'RVJ')   , (-0.256, 0.798))
(('HAR', 'RVTJ')  , (-2.001, 0.046)) (('HAR', 'RVTJ')  , (-0.982, 0.326))
(('HAR', 'RVSJ')  , (-4.193, 0.0)) (('HAR'  , 'RVSJ')  , (-1.619, 0.106))
(('HAR', 'RVSTJ') , (-2.733, 0.006)) (('HAR', 'RVSTJ') , (-1.319, 0.188))
(('HAR', 'SRV')   , (-2.254, 0.025)) (('HAR', 'SRV')   , (-0.216, 0.829))
(('HAR', 'SRVSJ') , (-4.362, 0.0)) (('HAR'  , 'SRVSJ') , (-1.802, 0.072))
(('HAR', 'SRVSTJ'), (-3.279, 0.001)) (('HAR', 'SRVSTJ'), (-1.665, 0.096))


QLIKE:
(('HAR', 'RVJ')   , (-1.69 , 0.091)) (('HAR', 'RVJ')   , (-2.939, 0.003))
(('HAR', 'RVTJ')  , (-1.776, 0.076)) (('HAR', 'RVTJ')  , (-1.944, 0.052))
(('HAR', 'RVSJ')  , (-0.012, 0.99)) (('HAR' , 'RVSJ')  , (-2.942, 0.003))
(('HAR', 'RVSTJ') , (-1.431, 0.153)) (('HAR', 'RVSTJ') , (-2.943, 0.003))
(('HAR', 'SRV')   , (-0.892, 0.373)) (('HAR', 'SRV')   , (-1.328, 0.185))
(('HAR', 'SRVSJ') , (-1.579, 0.115)) (('HAR', 'SRVSJ') , (-2.868, 0.004))
(('HAR', 'SRVSTJ'), (-2.2  , 0.028)) (('HAR', 'SRVSTJ'), (-3.128, 0.002))

(('HAR', 'RVJ'), (-1.69, 0.091))        (('HAR', 'RVJ'), (-2.939, 0.003))
(('HAR', 'RVTJ'), (-1.776, 0.076))        (('HAR', 'RVTJ'), (-1.944, 0.052))
(('HAR', 'RVSJ'), (0.004, 0.997))        (('HAR', 'RVSJ'), (-2.942, 0.003))
(('HAR', 'RVSTJ'), (-1.431, 0.153))        (('HAR', 'RVSTJ'), (-2.943, 0.003))
(('HAR', 'SRV'), (-0.892, 0.373))        (('HAR', 'SRV'), (-1.328, 0.185))
(('HAR', 'SRVSJ'), (-1.569, 0.117))        (('HAR', 'SRVSJ'), (-2.868, 0.004))
(('HAR', 'SRVSTJ'), (-2.2, 0.028))        (('HAR', 'SRVSTJ'), (-3.128, 0.002))









h=7, square form

MSE:
(('HAR', 'RVJ')   , (-2.539, 0.011)) (('HAR', 'RVJ')   , (1.618 , 0.106))
(('HAR', 'RVTJ')  , (1.836 , 0.067)) (('HAR', 'RVTJ')  , (1.717 , 0.086))
(('HAR', 'RVSJ')  , (0.739 , 0.46)) (('HAR' , 'RVSJ')  , (1.721 , 0.086))
(('HAR', 'RVSTJ') , (2.845 , 0.005)) (('HAR', 'RVSTJ') , (2.502 , 0.013))
(('HAR', 'SRV')   , (0.626 , 0.531)) (('HAR', 'SRV')   , (2.015 , 0.044))
(('HAR', 'SRVSJ') , (2.61  , 0.009)) (('HAR', 'SRVSJ') , (2.655 , 0.008))
(('HAR', 'SRVSTJ'), (2.704 , 0.007)) (('HAR', 'SRVSTJ'), (2.466 , 0.014))


HRMSE:

(('HAR', 'RVJ')   , (-2.499, 0.013)) (('HAR', 'RVJ')   , (-2.811, 0.005))
(('HAR', 'RVTJ')  , (1.354 , 0.176)) (('HAR', 'RVTJ')  , (-1.931, 0.054))
(('HAR', 'RVSJ')  , (0.003 , 0.998)) (('HAR', 'RVSJ')  , (0.564 , 0.573))
(('HAR', 'RVSTJ') , (0.752 , 0.452)) (('HAR', 'RVSTJ') , (-0.468, 0.64))
(('HAR', 'SRV')   , (-1.255, 0.21)) (('HAR' , 'SRV')   , (4.395 , 0.0))
(('HAR', 'SRVSJ') , (1.807 , 0.071)) (('HAR', 'SRVSJ') , (0.51  , 0.61))
(('HAR', 'SRVSTJ'), (0.986 , 0.324)) (('HAR', 'SRVSTJ'), (-1.752, 0.08))


QLIKE:

(('HAR', 'RVJ')   , (-2.751, 0.006)) (('HAR', 'RVJ')   , (-3.156, 0.002))
(('HAR', 'RVTJ')  , (-0.277, 0.782)) (('HAR', 'RVTJ')  , (-3.585, 0.0))
(('HAR', 'RVSJ')  , (-0.639, 0.523)) (('HAR', 'RVSJ')  , (-3.594, 0.0))
(('HAR', 'RVSTJ') , (-0.21 , 0.833)) (('HAR', 'RVSTJ') , (-5.132, 0.0))
(('HAR', 'SRV')   , (-1.407, 0.16)) (('HAR' , 'SRV')   , (-1.787, 0.074))
(('HAR', 'SRVSJ') , (2.19  , 0.029)) (('HAR', 'SRVSJ') , (-4.43 , 0.0))
(('HAR', 'SRVSTJ'), (-0.929, 0.353)) (('HAR', 'SRVSTJ'), (-5.13 , 0.0))









h=7, log form

MSE:

(('HAR', 'RVJ')   , (-1.244, 0.214)) (('HAR', 'RVJ')   , (-1.666, 0.096))
(('HAR', 'RVTJ')  , (0.505 , 0.614)) (('HAR', 'RVTJ')  , (-1.357, 0.175))
(('HAR', 'RVSJ')  , (0.366 , 0.715)) (('HAR', 'RVSJ')  , (-0.213, 0.832))
(('HAR', 'RVSTJ') , (0.819 , 0.413)) (('HAR', 'RVSTJ') , (0.432 , 0.666))
(('HAR', 'SRV')   , (-1.224, 0.221)) (('HAR', 'SRV')   , (-0.101, 0.92))
(('HAR', 'SRVSJ') , (-0.588, 0.557)) (('HAR', 'SRVSJ') , (-1.103, 0.27))
(('HAR', 'SRVSTJ'), (-0.083, 0.934)) (('HAR', 'SRVSTJ'), (0.19  , 0.85))

HRMSE:

(('HAR', 'RVJ')   , (-1.544, 0.123)) (('HAR', 'RVJ')   , (0.041 , 0.967))
(('HAR', 'RVTJ')  , (-0.476, 0.634)) (('HAR', 'RVTJ')  , (-1.902, 0.058))
(('HAR', 'RVSJ')  , (-1.261, 0.208)) (('HAR', 'RVSJ')  , (0.737 , 0.461))
(('HAR', 'RVSTJ') , (-1.046, 0.296)) (('HAR', 'RVSTJ') , (0.553 , 0.58))
(('HAR', 'SRV')   , (-2.137, 0.033)) (('HAR', 'SRV')   , (0.546 , 0.585))
(('HAR', 'SRVSJ') , (-1.081, 0.28)) (('HAR' , 'SRVSJ') , (-0.801, 0.423))
(('HAR', 'SRVSTJ'), (-1.028, 0.304)) (('HAR', 'SRVSTJ'), (-0.437, 0.662))

QLIKE:
(('HAR', 'RVJ')   , (-2.062, 0.04)) (('HAR' , 'RVJ')   , (-0.112, 0.911))
(('HAR', 'RVTJ')  , (-0.139, 0.889)) (('HAR', 'RVTJ')  , (-2.357, 0.019))
(('HAR', 'RVSJ')  , (0.814 , 0.416)) (('HAR', 'RVSJ')  , (-1.75 , 0.081))
(('HAR', 'RVSTJ') , (1.358 , 0.175)) (('HAR', 'RVSTJ') , (-2.103, 0.036))
(('HAR', 'SRV')   , (-0.047, 0.963)) (('HAR', 'SRV')   , (-0.835, 0.404))
(('HAR', 'SRVSJ') , (0.823 , 0.411)) (('HAR', 'SRVSJ') , (-0.669, 0.504))
(('HAR', 'SRVSTJ'), (0.327 , 0.743)) (('HAR', 'SRVSTJ'), (-1.195, 0.233))

(('HAR', 'RVJ')   , (-2.06 , 0.04)) (('HAR' , 'RVJ')   , (-0.111, 0.911))
(('HAR', 'RVTJ')  , (-0.029, 0.977)) (('HAR', 'RVTJ')  , (-2.345, 0.019))
(('HAR', 'RVSJ')  , (0.877 , 0.381)) (('HAR', 'RVSJ')  , (-1.686, 0.092))
(('HAR', 'RVSTJ') , (1.43  , 0.153)) (('HAR', 'RVSTJ') , (-2.052, 0.041))
(('HAR', 'SRV')   , (-0.014, 0.989)) (('HAR', 'SRV')   , (-0.835, 0.404))
(('HAR', 'SRVSJ') , (0.874 , 0.382)) (('HAR', 'SRVSJ') , (-0.592, 0.554))
(('HAR', 'SRVSTJ'), (0.369 , 0.712)) (('HAR', 'SRVSTJ'), (-1.144, 0.253))

h=30, square form

MSE:

(('HAR', 'RVJ')   , (0.785, 0.433)) (('HAR', 'RVJ')   , (2.799, 0.005))
(('HAR', 'RVTJ')  , (6.222, 0.0)) (('HAR'  , 'RVTJ')  , (3.056, 0.002))
(('HAR', 'RVSJ')  , (4.702, 0.0)) (('HAR'  , 'RVSJ')  , (3.39 , 0.001))
(('HAR', 'RVSTJ') , (2.491, 0.013)) (('HAR', 'RVSTJ') , (3.308, 0.001))
(('HAR', 'SRV')   , (4.265, 0.0)) (('HAR'  , 'SRV')   , (4.358, 0.0))
(('HAR', 'SRVSJ') , (5.624, 0.0)) (('HAR'  , 'SRVSJ') , (5.356, 0.0))
(('HAR', 'SRVSTJ'), (3.936, 0.0)) (('HAR'  , 'SRVSTJ'), (5.871, 0.0))


HRMSE:

(('HAR', 'RVJ')   , (3.491, 0.001)) (('HAR', 'RVJ')   , (3.219, 0.001))
(('HAR', 'RVTJ')  , (4.244, 0.0)) (('HAR'  , 'RVTJ')  , (3.254, 0.001))
(('HAR', 'RVSJ')  , (5.65 , 0.0)) (('HAR'  , 'RVSJ')  , (4.904, 0.0))
(('HAR', 'RVSTJ') , (5.832, 0.0)) (('HAR'  , 'RVSTJ') , (4.671, 0.0))
(('HAR', 'SRV')   , (2.432, 0.015)) (('HAR', 'SRV')   , (5.158, 0.0))
(('HAR', 'SRVSJ') , (6.297, 0.0)) (('HAR'  , 'SRVSJ') , (4.728, 0.0))
(('HAR', 'SRVSTJ'), (7.528, 0.0)) (('HAR'  , 'SRVSTJ'), (4.882, 0.0))



QLIKE:

(('HAR', 'RVJ')   , (-0.284, 0.776)) (('HAR', 'RVJ')   , (2.908, 0.004))
(('HAR', 'RVTJ')  , (2.397 , 0.017)) (('HAR', 'RVTJ')  , (1.915, 0.056))
(('HAR', 'RVSJ')  , (5.255 , 0.0)) (('HAR'  , 'RVSJ')  , (3.222, 0.001))
(('HAR', 'RVSTJ') , (2.749 , 0.006)) (('HAR', 'RVSTJ') , (0.96 , 0.337))
(('HAR', 'SRV')   , (5.615 , 0.0)) (('HAR'  , 'SRV')   , (5.41 , 0.0))
(('HAR', 'SRVSJ') , (5.942 , 0.0)) (('HAR'  , 'SRVSJ') , (3.382, 0.001))
(('HAR', 'SRVSTJ'), (2.972 , 0.003)) (('HAR', 'SRVSTJ'), (1.596, 0.111))


h=30, log form
MSE:
(('HAR', 'RVJ')   , (1.952 , 0.051)) (('HAR', 'RVJ')   , (2.791 , 0.005))
(('HAR', 'RVTJ')  , (5.152 , 0.0)) (('HAR'  , 'RVTJ')  , (2.539 , 0.011))
(('HAR', 'RVSJ')  , (2.948 , 0.003)) (('HAR', 'RVSJ')  , (2.944 , 0.003))
(('HAR', 'RVSTJ') , (2.398 , 0.017)) (('HAR', 'RVSTJ') , (3.551 , 0.0))
(('HAR', 'SRV')   , (3.537 , 0.0)) (('HAR'  , 'SRV')   , (2.266 , 0.024))
(('HAR', 'SRVSJ') , (3.531 , 0.0)) (('HAR'  , 'SRVSJ') , (4.054 , 0.0))
(('HAR', 'SRVSTJ'), (3.007 , 0.003)) (('HAR', 'SRVSTJ'), (4.971 , 0.0))

HRMSE:

(('HAR', 'RVJ')   , (5.43  , 0.0)) (('HAR'  , 'RVJ')   , (3.717, 0.0))
(('HAR', 'RVTJ')  , (5.533 , 0.0)) (('HAR'  , 'RVTJ')  , (1.958, 0.051))
(('HAR', 'RVSJ')  , (-0.692, 0.489)) (('HAR', 'RVSJ')  , (3.492, 0.001))
(('HAR', 'RVSTJ') , (-0.24 , 0.81)) (('HAR' , 'RVSTJ') , (4.483, 0.0))
(('HAR', 'SRV')   , (2.709 , 0.007)) (('HAR', 'SRV')   , (3.411, 0.001))
(('HAR', 'SRVSJ') , (4.462 , 0.0)) (('HAR'  , 'SRVSJ') , (5.601, 0.0))
(('HAR', 'SRVSTJ'), (4.679 , 0.0)) (('HAR'  , 'SRVSTJ'), (5.678, 0.0))


QLIKE:
(('HAR', 'RVJ')   , (2.039, 0.042)) (('HAR', 'RVJ')   , (3.608, 0.0))
(('HAR', 'RVTJ')  , (2.686, 0.007)) (('HAR', 'RVTJ')  , (2.285, 0.023))
(('HAR', 'RVSJ')  , (3.051, 0.002)) (('HAR', 'RVSJ')  , (3.247, 0.001))
(('HAR', 'RVSTJ') , (3.894, 0.0)) (('HAR'  , 'RVSTJ') , (2.5  , 0.013))
(('HAR', 'SRV')   , (7.849, 0.0)) (('HAR'  , 'SRV')   , (3.966, 0.0))
(('HAR', 'SRVSJ') , (4.282, 0.0)) (('HAR'  , 'SRVSJ') , (3.481, 0.001))
(('HAR', 'SRVSTJ'), (4.412, 0.0)) (('HAR'  , 'SRVSTJ'), (2.557, 0.011))

(('HAR', 'RVJ')   , (2.069, 0.039)) (('HAR', 'RVJ')   , (3.641, 0.0))
(('HAR', 'RVTJ')  , (3.036, 0.002)) (('HAR', 'RVTJ')  , (2.378, 0.018))
(('HAR', 'RVSJ')  , (3.056, 0.002)) (('HAR', 'RVSJ')  , (3.379, 0.001))
(('HAR', 'RVSTJ') , (4.14 , 0.0)) (('HAR'  , 'RVSTJ') , (2.769, 0.006))
(('HAR', 'SRV')   , (7.881, 0.0)) (('HAR'  , 'SRV')   , (3.889, 0.0))
(('HAR', 'SRVSJ') , (4.287, 0.0)) (('HAR'  , 'SRVSJ') , (3.619, 0.0))
(('HAR', 'SRVSTJ'), (4.589, 0.0)) (('HAR'  , 'SRVSTJ'), (2.829, 0.005))


RU

h=1, square form

(('HAR', 'RVJ')   , (3.019 , 0.003))
(('HAR', 'RVTJ')  , (3.32  , 0.001))
(('HAR', 'RVSJ')  , (2.075 , 0.038))
(('HAR', 'RVSTJ') , (3.357 , 0.001))
(('HAR', 'SRV')   , (2.194 , 0.029))
(('HAR', 'SRVSJ') , (3.448 , 0.001))
(('HAR', 'SRVSTJ'), (3.423 , 0.001))

(('HAR', 'RVJ')   , (3.076 , 0.002))
(('HAR', 'RVTJ')  , (3.177 , 0.002))
(('HAR', 'RVSJ')  , (4.183 , 0.0))
(('HAR', 'RVSTJ') , (4.486 , 0.0))
(('HAR', 'SRV')   , (2.573 , 0.01))
(('HAR', 'SRVSJ') , (4.453 , 0.0))
(('HAR', 'SRVSTJ'), (5.656 , 0.0))

h=1    , log form
(('HAR', 'RVJ')   , (1.43  , 0.153))
(('HAR', 'RVTJ')  , (1.723 , 0.085))
(('HAR', 'RVSJ')  , (-0.518, 0.604))
(('HAR', 'RVSTJ') , (1.145 , 0.252))
(('HAR', 'SRV')   , (0.575 , 0.566))
(('HAR', 'SRVSJ') , (1.242 , 0.215))
(('HAR', 'SRVSTJ'), (2.157 , 0.031))


(('HAR', 'RVJ')   , (2.385 , 0.017))
(('HAR', 'RVTJ')  , (2.127 , 0.034))
(('HAR', 'RVSJ')  , (2.739 , 0.006))
(('HAR', 'RVSTJ') , (3.023 , 0.003))
(('HAR', 'SRV')   , (0.92  , 0.358))
(('HAR', 'SRVSJ') , (2.928 , 0.004))
(('HAR', 'SRVSTJ'), (3.253 , 0.001))

h=7    , square form


(('HAR', 'RVJ')   , (2.543 , 0.011))
(('HAR', 'RVTJ')  , (0.174 , 0.862))
(('HAR', 'RVSJ')  , (0.707 , 0.48))
(('HAR', 'RVSTJ') , (0.285 , 0.776))
(('HAR', 'SRV')   , (1.444 , 0.149))
(('HAR', 'SRVSJ') , (-1.946, 0.052))
(('HAR', 'SRVSTJ'), (1.047 , 0.295))

(('HAR', 'RVJ')   , (3.061 , 0.002))
(('HAR', 'RVTJ')  , (3.539 , 0.0))
(('HAR', 'RVSJ')  , (3.396 , 0.001))
(('HAR', 'RVSTJ') , (4.918 , 0.0))
(('HAR', 'SRV')   , (2.163 , 0.031))
(('HAR', 'SRVSJ') , (4.234 , 0.0))
(('HAR', 'SRVSTJ'), (4.824 , 0.0))

h=7    , log form

(('HAR', 'RVJ')   , (1.876 , 0.061))
(('HAR', 'RVTJ')  , (0.163 , 0.871))
(('HAR', 'RVSJ')  , (-0.661, 0.509))
(('HAR', 'RVSTJ') , (-1.252, 0.211))
(('HAR', 'SRV')   , (-0.121, 0.904))
(('HAR', 'SRVSJ') , (-0.525, 0.6))
(('HAR', 'SRVSTJ'), (-0.055, 0.956))

(('HAR', 'RVJ')   , (-0.146, 0.884))
(('HAR', 'RVTJ')  , (2.167 , 0.031))
(('HAR', 'RVSJ')  , (1.838 , 0.066))
(('HAR', 'RVSTJ') , (2.22  , 0.027))
(('HAR', 'SRV')   , (0.991 , 0.322))
(('HAR', 'SRVSJ') , (0.568 , 0.57))
(('HAR', 'SRVSTJ'), (1.05  , 0.294))

h=30   , square form

(('HAR', 'RVJ')   , (0.788 , 0.431))
(('HAR', 'RVTJ')  , (-1.61 , 0.108))
(('HAR', 'RVSJ')  , (-4.317, 0.0))
(('HAR', 'RVSTJ') , (-1.874, 0.061))
(('HAR', 'SRV')   , (-5.085, 0.0))
(('HAR', 'SRVSJ') , (-4.874, 0.0))
(('HAR', 'SRVSTJ'), (-1.936, 0.053))

(('HAR', 'RVJ')   , (-2.495, 0.013))
(('HAR', 'RVTJ')  , (-1.42 , 0.156))
(('HAR', 'RVSJ')  , (-2.388, 0.017))
(('HAR', 'RVSTJ') , (-0.281, 0.779))
(('HAR', 'SRV')   , (-4.625, 0.0))
(('HAR', 'SRVSJ') , (-2.598, 0.01))
(('HAR', 'SRVSTJ'), (-0.772, 0.44))

h=30   , log form

(('HAR', 'RVJ')   , (-1.209, 0.227))
(('HAR', 'RVTJ')  , (-2.058, 0.04))
(('HAR', 'RVSJ')  , (-2.495, 0.013))
(('HAR', 'RVSTJ') , (-3.257, 0.001))
(('HAR', 'SRV')   , (-7.486, 0.0))
(('HAR', 'SRVSJ') , (-3.441, 0.001))
(('HAR', 'SRVSTJ'), (-3.563, 0.0))


(('HAR', 'RVJ')   , (-3.063, 0.002))
(('HAR', 'RVTJ')  , (-1.84 , 0.066))
(('HAR', 'RVSJ')  , (-2.592, 0.01))
(('HAR', 'RVSTJ') , (-1.883, 0.06))
(('HAR', 'SRV')   , (-3.359, 0.001))
(('HAR', 'SRVSJ') , (-2.649, 0.008))
(('HAR', 'SRVSTJ'), (-1.796, 0.073))


==> EconomicResults.tex <==


BTC-D
square form

{}        & HAR     & RVJ     & RVTJ    & RVSJ     & RVSTJ   & SRV     & SRVSJ    & SRVSTJ                       \\
\midrule
uow\_mean & 2.938\% & 2.403\% & 2.496\% & 2.613\%  & 2.268\% & 2.626\% & 2.356\%  & 1.421\% & 2.546\% & 4.000\%  \\
uow\_mean & 3.071\% & 2.614\% & 3.048\% & 2.935\%  & 3.024\% & 2.916\% & 3.339\%  & 2.874\% & 3.922\% & 4.000\%  \\
uow\_mean & 3.569\% & 3.522\% & 3.642\% & 3.760\%  & 3.667\% & 3.708\% & 3.769\%  & 3.678\% & 3.994\% & 4.000\%  \\

log form

{}        & HAR     & RVJ     & RVTJ    & RVSJ     & RVSTJ   & SRV     & SRVSJ    & SRVSTJ                       \\
\midrule
uow\_mean & 2.619\% & 2.486\% & 2.404\% & 2.660\%  & 2.486\% & 2.583\% & 2.403\%  & 2.146\% & 2.546\% & 4.000\%  \\
uow\_mean & 3.133\% & 2.969\% & 3.128\% & 3.196\%  & 3.234\% & 3.140\% & 3.204\%  & 3.143\% & 3.922\% & 4.000\%  \\
uow\_mean & 3.479\% & 3.527\% & 3.591\% & 3.619\%  & 3.641\% & 3.671\% & 3.676\%  & 3.665\% & 3.994\% & 4.000\%  \\



BTC-G
square form

{}        & HAR     & RVJ     & RVTJ    & RVSJ     & RVSTJ   & SRV     & SRVSJ    & SRVSTJ                       \\
\midrule
uow\_mean & 2.650\% & 1.364\% & 1.330\% & -0.244\% & 0.560\% & 2.041\% & -0.421\% & -1.843\% & 2.136\% & 4.000\% \\
uow\_mean & 3.164\% & 2.271\% & 1.862\% & 0.569\%  & 1.294\% & 2.906\% & 1.090\%  & 1.100\% & 3.896\% & 4.000\%  \\
uow\_mean & 3.585\% & 3.687\% & 3.637\% & 3.669\%  & 3.597\% & 3.689\% & 3.697\%  & 3.621\% & 3.993\% & 4.000\%  \\


log form

{}        & HAR     & RVJ     & RVTJ    & RVSJ     & RVSTJ   & SRV     & SRVSJ    & SRVSTJ                       \\
\midrule
uow\_mean & 2.098\% & 1.871\% & 1.728\% & 1.663\%  & 1.584\% & 2.019\% & 1.513\%  & 1.393\% & 2.136\% & 4.000\%  \\
uow\_mean & 2.793\% & 2.805\% & 2.549\% & 2.496\%  & 2.466\% & 2.710\% & 2.699\%  & 2.631\% & 3.896\% & 4.000\%  \\
uow\_mean & 3.576\% & 3.668\% & 3.633\% & 3.672\%  & 3.647\% & 3.635\% & 3.690\%  & 3.662\% & 3.993\% & 4.000\%  \\


==> Old_HAR_results_BeforeAdaptive.tex <==

@ Table 1: Thresholded Jump HAR

\begin{table}[!htb]
  \begin{threeparttable}
    \caption{In-Sample Fitting and Out-of-Sample Forecasting with (Un)-Thresholded Jumps}\label{tab:har_rv_tj_h1}
    \centering % centering table
    \tiny
    \begin{tabular}{lc*{11}{S[table-format=1.2,table-number-alignment = center]}}
      % >{\raggedleft\arraybackslash}p{5em}
  \toprule
  \toprule
  \multicolumn{12}{l}{\textbf{h=1}}\\
  \multicolumn{12}{l}{HAR : ${RV}_{t,t+h}
  =\alpha+\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} +\varepsilon_{t,t+1} $}\\
  %
  \multicolumn{12}{l}{RVJ : ${RV}_{t,t+h}
  =\alpha+\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} +
  \beta_{JD} {J}_{D}+\beta_{JW} {J}_{W}+\beta_{JM} {J}_{M} + \varepsilon_{t,t+1} $}\\

  \multicolumn{12}{l}{RVTJ : ${RV}_{t,t+h}
  =\alpha+\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} +
  \beta_{JD} {TJ}_{D}+\beta_{JW} {TJ}_{W}+\beta_{JM} {TJ}_{M} + \varepsilon_{t,t+1}$}\\

  \multicolumn{12}{l}{HExp-RVJ : ${RV}_{t,t+h}
  =\alpha+\beta_D {RV}_{D}^{Exp} +\beta_W {RV}_{W}^{Exp} +\beta_M {RV}_{M}^{Exp} +
  \beta_{JD} {J}_{D}+\beta_{JW} {J}_{W}+\beta_{JM} {J}_{M}  \varepsilon_{t,t+1} $}\\

  \multicolumn{12}{l}{HExp-RVTJ : ${RV}_{t,t+h}
  =\alpha+\beta_D {RV}_{D}^{Exp} +\beta_W {RV}_{W}^{Exp} +\beta_M {RV}_{M}^{Exp} +
  \beta_{JD} {TJ}_{D}+\beta_{JW} {TJ}_{W}+\beta_{JM} {TJ}_{M} + \varepsilon_{t,t+1}$}\\

  \midrule

  &\multicolumn{5}{c}{Square form}
  &\multicolumn{1}{c}{}
  &\multicolumn{5}{c}{Logarithmic form}\\
  \cline{2-6}
  \cline{8-12}\\

  \multicolumn{1}{c}{}
  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RVTJ}
  &\multicolumn{1}{c}{HExp-RVJ}
  &\multicolumn{1}{c}{HExp-RVTJ}

  &\multicolumn{1}{c}{}

  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RVTJ}
  &\multicolumn{1}{c}{HExp-RVJ}
  &\multicolumn{1}{c}{HExp-RVTJ}
  \\

  \midrule
  &\multicolumn{4}{c}{}
  &\multicolumn{3}{c}{\textbf{BTC-D}}
  &\multicolumn{4}{c}{}\\
  \cline{2-12}\\

  \multirow{2}{*}{$\alpha$}     & 0.175   & 0.335    & 0.271    & 0.335    & 0.271    & & -0.122      & -0.053       & -0.006       & -0.044       & -0.01       \\
                                & (2.46)  & (2.953)  & (1.696)  & (2.953)  & (1.696)  & & (-4.341)    & (-1.335)     & (-0.147)     & (-1.109)     & (-0.224)    \\
  \multirow{2}{*}{$\beta_{D}$}  & 0.437   & 0.430    & 0.457    & 0.430    & 0.457    & & 0.568       & 0.570        & 0.600        & 0.542        & 0.555       \\
                                & (6.284) & (6.466)  & (6.470)  & (6.466)  & (6.47)   & & (15.758)    & (15.879)     & (17.108)     & (14.952)     & (16.089)    \\
  \multirow{2}{*}{$\beta_{W}$}  & 0.100   & 0.089    & 0.089    & 0.089    & 0.089    & & 0.236       & 0.227        & 0.225        & 0.216        & 0.198       \\
                                & (2.119) & (1.862)  & (1.743)  & (1.862)  & (1.743)  & & (5.387)     & (5.002)      & (4.745)      & (5.069)      & (4.769)     \\
  \multirow{2}{*}{$\beta_{M}$}  & 0.311   & 0.292    & 0.292    & 0.292    & 0.292    & & 0.132       & 0.116        & 0.096        & 0.109        & 0.080       \\
                                & (2.722) & (2.523)  & (2.452)  & (2.523)  & (2.452)  & & (2.797)     & (2.434)      & (2.164)      & (2.368)      & (2.026)     \\
  \multirow{2}{*}{$\beta_{JD}$} &         & 0.680    & -0.476   & 1.110    & -0.020   & &             & -0.426       & -0.574       & 0.358        & 0.046       \\
                                &         & (0.781)  & (-2.303) & (1.235)  & (-0.102) & &             & (-1.094)     & (-3.053)     & (0.973)      & (0.258)     \\
  \multirow{2}{*}{$\beta_{JW}$} &         & -0.179   & -0.046   & -0.090   & 0.043    & &             & -0.595       & -0.534       & -0.385       & -0.186      \\
                                &         & (-0.195) & (-0.112) & (-0.098) & (0.110)  & &             & (-1.151)     & (-1.932)     & (-0.790)     & (-0.783)    \\
  \multirow{2}{*}{$\beta_{JM}$} &         & -4.216   & -0.538   & -3.925   & -0.246   & &             & -1.500       & -0.489       & -1.165       & 0.044       \\
                                &         & (-2.494) & (-0.489) & (-2.279) & (-0.211) & &             & (-1.789)     & (-1.350)     & (-1.459)     & (0.114)     \\
                                                                                                                                                                 \\
  MZ-$R^2$                      & 0.312   & 0.215    & 0.321    & 0.215    & 0.321    & & 0.317       & 0.329        & 0.339        & 0.335        & 0.364       \\
  MSE                           & 0.285   & 0.314    & 0.294    & 0.314    & 0.294    & & 0.209       & 0.207        & 0.205        & 0.206        & 0.203       \\
  HRMSE                         & 4.315   & 4.127    & 4.530    & 4.127    & 4.530    & & 1.156       & 1.140        & 1.106        & 1.029        & 0.853       \\
  QLIKE                         & 2.409   & 1.944    & 2.568    & 1.944    & 2.568    & & 0.140       & 0.114        & 0.107        & 0.005        & -0.121      \\
  D-M$^{\dagger}$               &         &          &          &          &          & &4.625\threeS & 3.860\threeS & 5.730\threeS & 3.854\threeS & 5.595\threeS\\
  D-M$^{\ddagger}$              &         &-1.324    & -1.091   & -1.324   & -1.091   & &             &2.452\twoS    & 1.424        & 1.973\twoS   & 1.735\oneS  \\

  \midrule
  &\multicolumn{4}{c}{}
  &\multicolumn{3}{c}{\textbf{BTC-G}}
  &\multicolumn{4}{c}{}\\
  \cline{2-12}\\

  \multirow{2}{*}{$\alpha$}     & 0.179   & 0.278    & 0.304    & 0.278    & 0.304    & & -0.183     & -0.051    & 0.002    & -0.038       & 0.019    \\
                                & (2.321) & (3.596)  & (3.958)  & (3.596)  & (3.958)  & & (-5.188)   & (-1.023)  & (0.043)  & (-0.737)     & (0.324)  \\
  \multirow{2}{*}{$\beta_{D}$}  & 0.333   & 0.379    & 0.393    & 0.379    & 0.393    & & 0.533      & 0.527     & 0.550    & 0.474        & 0.476    \\
                                & (4.552) & (5.098)  & (4.725)  & (5.098)  & (4.725)  & & (16.759)   & (16.422)  & (16.335) & (16.081)     & (15.954) \\
  \multirow{2}{*}{$\beta_{W}$}  & 0.166   & 0.177    & 0.172    & 0.177    & 0.172    & & 0.262      & 0.302     & 0.313    & 0.267        & 0.232    \\
                                & (2.973) & (2.617)  & (2.401)  & (2.617)  & (2.401)  & & (6.727)    & (7.308)   & (6.99)   & (6.828)      & (5.766)  \\
  \multirow{2}{*}{$\beta_{M}$}  & 0.322   & 0.271    & 0.258    & 0.271    & 0.258    & & 0.126      & 0.104     & 0.068    & 0.118        & 0.084    \\
                                & (2.614) & (2.226)  & (2.029)  & (2.226)  & (2.029)  & & (2.822)    & (2.391)   & (1.471)  & (2.949)      & (2.205)  \\
  \multirow{2}{*}{$\beta_{JD}$} &         & -0.493   & -0.333   & -0.114   & 0.060    & &            & -0.430    & -0.419   & 0.051        & 0.162    \\
                                &         & (-2.639) & (-2.091) & (-0.796) & (0.507)  & &            & (-2.022)  & (-2.42)  & (0.219)      & (1.037)  \\
  \multirow{2}{*}{$\beta_{JW}$} &         & -0.511   & -0.250   & -0.334   & -0.078   & &            & -0.903    & -0.685   & -0.537       & -0.199   \\
                                &         & (-1.967) & (-1.654) & (-1.496) & (-0.725) & &            & (-3.05)   & (-3.383) & (-2.083)     & (-1.155) \\
  \multirow{2}{*}{$\beta_{JM}$} &         & -0.363   & -0.274   & -0.092   & -0.016   & &            & -0.484    & -0.247   & -0.147       & -0.050   \\
                                &         & (-0.803) & (-0.901) & (-0.212) & (-0.057) & &            & (-1.353)  & (-0.891) & (-0.408)     & (-0.181) \\
                                                                                                                                                      \\
  MZ-$R^2$                      & 0.305   & 0.333    & 0.336    & 0.333    & 0.336    & & 0.313      & 0.328     & 0.310    & 0.333        & 0.334    \\
  MSE                           & 0.539   & 0.550    & 0.556    & 0.550    & 0.556    & & 0.527      & 0.508     & 0.545    & 0.503        & 0.522    \\
  HRMSE                         & 5.578   & 7.466    & 7.438    & 7.466    & 7.438    & & 1.261      & 1.353     & 1.302    & 1.569        & 1.571    \\
  QLIKE                         & 2.583   & 3.467    & 3.355    & 3.467    & 3.355    & & 0.017      & 0.112     & 0.065    & 0.295        & 0.264    \\
  D-M$^{\dagger}$               &         &          &          &          &          & &-1.879\twoS & -0.686    & -1.294   & -0.748       & -1.228   \\
  D-M$^{\ddagger}$              &         & -0.752   & -1.133   & -0.752   & -1.133   & &            &2.056\twoS & -0.666   & 2.588\threeS & 0.287    \\


    \bottomrule
    \bottomrule
    \end{tabular}
% Day-ahead Forecast Regression Results on BTC-G, $\alpha=0.9999$, $c_{\theta}=3$, 5-minutes frequency
\begin{tablenotes}
  \tiny
  \item $\alpha=99.99\%$, 5-minutes Frequency, $C_\theta=3$
  \item $^{\dagger}:$ D-M test with quadratic loss. Logarithmic form models against corresponding square form models. Significant positive statistics implies that logarithmic models perform better, vice versa.
  \item $^{\ddagger}:$ D-M test with quadratic loss. Models with jumps against HAR model. Significant positive statistics implies that HAR model perform worse, vice versa.
  \item \threeS: 1\% significance, \twoS: 5\% significance, \oneS: 10\% significance
\end{tablenotes}
\end{threeparttable}

  \end{table}

@ Table 2: Signed Jumps HAR

  \begin{table}[!htb]
    \begin{threeparttable}
      \caption{Fitting Anaylsis and Forecasting Power of Positive/Negative Jumps}\label{tab:har_signed_jtj}
      \centering % centering table
      \scriptsize
      \begin{tabular}{lc*{9}{S[table-format=3.3,table-number-alignment = center]}}
        % >{\raggedleft\arraybackslash}p{5em}
    \toprule
    \toprule
    \multicolumn{10}{l}{\textbf{h=1}}\\
    % \multicolumn{10}{l}{RV(T)J$^{+(-)}$:${RV}_{t,t+h}=\alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M}$}\\
    \multicolumn{2}{c}{RV(T)J$^{+(-)}$:}
    & \multicolumn{8}{l}{
    $\begin{array} {rcl} {RV}_{t,t+h} & = & \alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} \\
    & + & \beta_{JD} (T)J^{+(-)}_{D}+\beta_{JW} (T)J^{+(-)}_{W}+\beta_{JM} (T)J^{+(-)}_{M} +\varepsilon_{t,t+h} \end{array}$
    }\\
    \midrule
    % \multicolumn{1}{c}{}
  % \\
    \multicolumn{1}{c}{}
    &\multicolumn{4}{c}{Square form}
    &\multicolumn{1}{c}{}
    &\multicolumn{4}{c}{Logarithmic form}\\
    \cline{2-5}
    \cline{7-10}\\

    \multicolumn{1}{c}{}
    &\multicolumn{1}{c}{RVJ$^+$}
    &\multicolumn{1}{c}{RVJ$^-$}
    &\multicolumn{1}{c}{RVTJ$^+$}
    &\multicolumn{1}{c}{RVTJ$^-$}
    &\multicolumn{1}{c}{}
    &\multicolumn{1}{c}{RVJ$^+$}
    &\multicolumn{1}{c}{RVJ$^-$}
    &\multicolumn{1}{c}{RVTJ$^+$}
    &\multicolumn{1}{c}{RVTJ$^-$}\\

    \midrule
                                    &\multicolumn{3}{c}{} &\multicolumn{3}{c}{\textbf{BTC-D}} &\multicolumn{3}{c}{}                                               \\
    \cline{2-10}                                                                                                                                                  \\


    \multirow{2}{*}{$\alpha$}       & 0.291    & 0.217    & 0.338    & 0.288    & & -0.249       & -0.085       & -0.004       & 0.035                            \\
                                    & (2.629)  & (1.356)  & (3.694)  & (1.881)  & & (-2.96)      & (-1.932)     & (-0.07)      & (0.38)                           \\
    \multirow{2}{*}{$\beta_{D}$}    & 0.701    & 0.741    & 0.461    & 0.392    & & 0.751        & 0.696        & 0.551        & 0.532                            \\
                                    & (6.657)  & (6.899)  & (6.206)  & (4.408)  & & (19.362)     & (9.492)      & (14.908)     & (12.839)                         \\
    \multirow{2}{*}{$\beta_{W}$}    & 0.605    & -0.497   & 0.112    & 0.066    & & 0.242        & -0.121       & 0.258        & 0.237                            \\
                                    & (3.037)  & (-2.531) & (1.708)  & (0.987)  & & (4.277)      & (-0.968)     & (5.378)      & (4.454)                          \\
    \multirow{2}{*}{$\beta_{M}$}    & -0.463   & 0.627    & 0.375    & 0.441    & & -0.132       & 0.28         & 0.094        & 0.153                            \\
                                    & (-2.447) & (2.985)  & (2.865)  & (3.243)  & & (-3.387)     & (3.054)      & (1.906)      & (2.518)                          \\
    \multirow{2}{*}{$\beta_{JD}$}   & 1.096    & 0.02     & -1.213   & 1.257    & & 0.337        & 0.084        & -0.311       & 0.261                            \\
                                    & (1.182)  & (0.1)    & (-2.513) & (0.884)  & & (0.895)      & (0.475)      & (-1.423)     & (0.817)                          \\
    \multirow{2}{*}{$\beta_{JW}$}   & -0.347   & -0.065   & -0.955   & 0.96     & & -0.271       & -0.141       & -1.142       & -0.463                           \\
                                    & (-0.409) & (-0.153) & (-0.893) & (0.562)  & & (-0.54)      & (-0.587)     & (-2.577)     & (-0.723)                         \\
    \multirow{2}{*}{$\beta_{JM}$}   & -3.485   & 0.027    & -2.408   & -4.417   & & -0.853       & 0.211        & 0.339        & -1.364                           \\
                                    & (-2.079) & (0.024)  & (-1.801) & (-1.878) & & (-1.069)     & (0.55)       & (0.521)      & (-1.361)                         \\
                                                                                                                                                                  \\
    MZ-$R^2$                        & 0.211    & 0.295    & 0.196    & 0.267    & & 0.318        & 0.347        & 0.34         & 0.325                            \\
    MSE                             & 0.294    & 0.276    & 0.264    & 0.301    & & 0.209        & 0.207        & 0.208        & 0.21                             \\
    HRMSE                           & 3.675    & 4.074    & 3.828    & 4.514    & & 1.303        & 0.912        & 0.945        & 0.998                            \\
    QLIKE                           & 1.635    & 2.250    & 1.864    & 2.316    & & 0.157        & -0.105       & -0.051       & -0.008                           \\
    D-M$^{\dagger}$                 &          &          &          &          & & 3.721\threeS & 4.993\threeS & 2.743\threeS & 3.460\threeS                     \\
    D-M$^{\ddagger}$                &          &          &0.927     & -1.249   & &              &              &0.068         & -0.767                           \\

    \midrule
                                    &\multicolumn{3}{c}{}
                                    &\multicolumn{3}{c}{\textbf{BTC-G}}
                                    &\multicolumn{3}{c}{}                                                                                                         \\
    \cline{2-10}                                                                                                                                                  \\

    \multirow{2}{*}{$\alpha$}       & 0.247    & 0.274    & 0.482       & 0.249    & & -0.394   & -0.05       & 0.102    & -0.035                                 \\
                                    & (3.116)  & (3.509)  & (4.397)     & (3.371)  & & (-3.987) & (-0.828)    & (0.947)  & (-0.502)                               \\
    \multirow{2}{*}{$\beta_{D}$}    & 0.586    & 0.609    & 0.390       & 0.380    & & 0.691    & 0.593       & 0.481    & 0.473                                  \\
                                    & (4.66)   & (4.503)  & (4.901)     & (4.884)  & & (16.874) & (7.68)      & (16.016) & (14.100)                               \\
    \multirow{2}{*}{$\beta_{W}$}    & 0.529    & -0.269   & 0.327       & 0.168    & & 0.353    & -0.032      & 0.291    & 0.269                                  \\
                                    & (2.369)  & (-1.065) & (3.041)     & (2.458)  & & (4.616)  & (-0.209)    & (6.471)  & (6.294)                                \\
    \multirow{2}{*}{$\beta_{M}$}    & -0.264   & 0.505    & 0.371       & 0.292    & & -0.152   & 0.264       & 0.144    & 0.130                                  \\
                                    & (-1.095) & (2.188)  & (2.229)     & (2.265)  & & (-2.834) & (2.321)     & (2.617)  & (3.055)                                \\
    \multirow{2}{*}{$\beta_{JD}$}   & -0.117   & 0.059    & -0.981      & -0.050   & & -0.067   & 0.148       & -0.189   & 0.120                                  \\
                                    & (-0.905) & (0.513)  & (-1.739)    & (-0.236) & & (-0.298) & (0.97)      & (-0.693) & (0.414)                                \\
    \multirow{2}{*}{$\beta_{JW}$}   & -0.300   & -0.073   & -3.745      & -0.037   & & -0.350   & -0.156      & -1.511   & -0.377                                 \\
                                    & (-1.364) & (-0.663) & (-2.663)    & (-0.254) & & (-1.249) & (-0.794)    & (-3.296) & (-1.461)                               \\
    \multirow{2}{*}{$\beta_{JM}$}   & 0.011    & 0.064    & -2.805      & -0.169   & & 0.215    & -0.048      & -0.698   & -0.218                                 \\
                                    & (0.027)  & (0.252)  & (-1.299)    & (-0.440) & & (0.635)  & (-0.185)    & (-0.655) & (-0.551)                               \\
                                                                                                                                                                  \\
    MZ-$R^2$                 & 0.321    & 0.319    & 0.242       & 0.328    & & 0.321    & 0.326       & 0.335    & 0.330                                  \\
    MSE                             & 0.543    & 0.549    & 0.612       & 0.546    & & 0.517    & 0.534       & 0.499    & 0.510                                  \\
    HRMSE                           & 7.084    & 7.085    & 9.880       & 6.978    & & 1.733    & 1.545       & 1.420    & 1.506                                  \\
    QLIKE                           & 3.252    & 3.167    & 4.062       & 3.239    & & 0.327    & 0.175       & 0.187    & 0.244                                  \\
    D-M$^{\dagger}$                 &          &          &             &          & &-1.534    & -1.674\oneS & 1.078    & -0.914                                 \\
    D-M$^{\ddagger}$                &          &          & -2.088\twoS & 0.132    & &          &             &1.257     & 1.016                                  \\

      \bottomrule
      \bottomrule
      \end{tabular}

      \begin{tablenotes}
        \tiny
        \item $\alpha=99.99\%$, 5-minutes Frequency, $C_\theta=3$\\
        \item $^{\dagger}:$ D-M test with quadratic loss. Logarithmic form models against corresponding square form models. Significant positive statistics implies that logarithmic models perform better, vice versa.
        \item $^{\ddagger}:$ D-M test with quadratic loss. Signed-thresholded jump models against signed-unthresholded jump models. Significant negative statistics implies that unthresholded model performs better, vice versa.\\
        \item \threeS: 1\% significance, \twoS: 5\% significance, \oneS: 10\% significance
      \end{tablenotes}
      \end{threeparttable}

  % Day-ahead Forecast Regression Results on BTC-G, $\alpha=0.9999$, $c_{\theta}=3$, 5-minutes frequency
    \end{table}


@ Table 3: Signed and thresholded jump HAR

    \begin{table*}[!htb]
      \renewcommand\multirowsetup{\centering}
        \caption{In-Sample Fitting and Out-of-Sample Forecasting with Signed Jumps}\label{tab:har_signed_jtj_full}
        \centering % centering table
        \tiny
        \begin{tabular}{lc*{14}{S[table-format=1.1,table-number-alignment = center]}}
          % >{\raggedleft\arraybackslash}p{5em}
      \toprule
      \toprule
      \multicolumn{10}{l}{\textbf{h=1}}\\
      % \multicolumn{10}{l}{RV(T)J$^{+(-)}$:${RV}_{t,t+h}=\alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M}$}\\
      \multicolumn{2}{c}{RV(T)SJ:}
      & \multicolumn{13}{l}{
      $\begin{array} {rcl} {RV}_{t,t+h} & = & \alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} \\
      & + & \beta_{JD}^{+} (T)J^{+}_{D}+\beta_{JW}^{+} (T)J^{+}_{W}+\beta_{JM}^{+} (T)J^{+}_{M}\\
      & + & \beta_{JD}^{-} (T)J^{-}_{D}+\beta_{JW}^{-} (T)J^{-}_{W}+\beta_{JM}^{-} (T)J^{-}_{M} +\varepsilon_{t,t+h} \end{array}$
      }\\
    \\
      \multicolumn{1}{c}{}
      &\multicolumn{1}{c}{$\alpha$}
      &\multicolumn{1}{c}{$\beta_{D}$}
      &\multicolumn{1}{c}{$\beta_{W}$}
      &\multicolumn{1}{c}{$\beta_{M}$}
      &\multicolumn{1}{c}{$\beta_{JD}^{+}$}
      &\multicolumn{1}{c}{$\beta_{JW}^{+}$}
      &\multicolumn{1}{c}{$\beta_{JM}^{+}$}
      &\multicolumn{1}{c}{$\beta_{JD}^{-}$}
      &\multicolumn{1}{c}{$\beta_{JW}^{-}$}
      &\multicolumn{1}{c}{$\beta_{JM}^{-}$}
      &\multicolumn{1}{c}{MZ-$R^2$}
      &\multicolumn{1}{c}{MSE}
      &\multicolumn{1}{c}{HRMSE}
      &\multicolumn{1}{c}{QLIKE}\\

      \midrule
      \multicolumn{15}{l}{\textbf{BTC-D:}}\\
      \cline{1-3}
      \multicolumn{1}{l}{}&\multicolumn{10}{l}{\textbf{Square form}}\\
    \\

      \multirow{2}{*}{RVSJ}            & 0.382   & 0.431    & 0.065   & 0.521   & -1.071   & -0.647   & -3.063   & 0.800    & 1.126    & -4.111   & 0.219 & 0.275 & 3.865  & 1.855  \\
      {}                               & (2.464) & (3.785)  & (0.765) & (3.224) & (-1.958) & (-0.572) & (-2.095) & (0.515)  & (0.683)  & (-1.803) &                                 \\
      \multirow{2}{*}{RVTSJ}           & 0.305   & 0.495    & 0.089   & 0.363   & -1.357   & -0.925   & -1.547   & -0.086   & 0.798    & -0.303   & 0.140 & 0.288 & 3.648  & 1.780  \\
      {}                               & (1.994) & (5.193)  & (1.134) & (3.141) & (-3.593) & (-1.063) & (-1.21)  & (-0.138) & (1.085)  & (-0.198) &                                 \\
                                                                                                                                                                                    \\
      \cline{1-3}
      \multicolumn{1}{l}{}             &\multicolumn{10}{l}{\textbf{Logarithmic form}}                                                                                              \\
                                                                                                                                                                                    \\

      \multirow{2}{*}{RVSJ}            & 0.115   & 0.581    & 0.315   & 0.133   & -0.514   & -1.308   & 0.299    & -0.134   & -0.91    & -0.943   & 0.317 & 0.213 & 0.997  & 0.015  \\
                                       & (1.171) & (13.658) & (4.817) & (1.792) & (-2.139) & (-2.503) & (0.448)  & (-0.418) & (-1.301) & (-0.855) &       &       &        &        \\
      \multirow{2}{*}{RVTSJ}           & 0.097   & 0.605    & 0.301   & 0.103   & -0.602   & -1.245   & 0.312    & -0.223   & -0.334   & -0.455   & 0.328 & 0.209 & 1.027  & 0.045  \\
                                       & (1.195) & (13.871) & (4.841) & (1.778) & (-3.211) & (-3.225) & (0.555)  & (-0.98)  & (-0.768) & (-0.746) &       &       &        &        \\
                                                                                                                                                                                    \\
      \midrule
      \multicolumn{15}{l}{\textbf{BTC-G:}}                                                                                                                                          \\
      \cline{1-3}
      \multicolumn{1}{l}{}             &\multicolumn{10}{l}{\textbf{Square form}}                                                                                                   \\
                                                                                                                                                                                    \\
      \multirow{2}{*}{RVSJ}            & 0.512   & 0.423    & 0.352   & 0.404   & -1.357   & -4.023   & -3.105   & -0.500   & -0.461   & -0.607   & 0.234 & 0.624 & 10.735 & 4.432  \\
                                       & (4.279) & (4.2)    & (2.824) & (2.147) & (-2.309) & (-2.591) & (-1.363) & (-1.737) & (-1.869) & (-1.313) &                                 \\
      \multirow{2}{*}{RVTSJ}           & 0.522   & 0.437    & 0.31    & 0.342   & -1.221   & -2.932   & -2.295   & -0.216   & 0.168    & -0.224   & 0.18  & 0.621 & 9.506  & 3.684  \\
                                       & (5.089) & (4.323)  & (2.730) & (2.160) & (-2.831) & (-2.619) & (-1.566) & (-0.923) & (1.000)  & (-0.608) &                                 \\
                                                                                                                                                                                    \\
      \cline{1-3}
      \multicolumn{1}{l}{}             &\multicolumn{10}{l}{\textbf{Logarithmic form}}                                                                                              \\
                                                                                                                                                                                    \\

      \multirow{2}{*}{RVSJ}            & 0.247   & 0.542    & 0.382   & 0.148   & -0.601   & -1.988   & -0.732   & -0.247   & -0.863   & -0.662   & 0.326 & 0.509 & 1.192  & -0.005 \\
                                       & (1.786) & (12.9)   & (6.993) & (2.203) & (-1.793) & (-4.026) & (-0.686) & (-0.81)  & (-2.948) & (-1.526) &                                 \\
      \multirow{2}{*}{RVTSJ}           & 0.23    & 0.554    & 0.378   & 0.109   & -0.677   & -1.698   & -0.43    & -0.135   & -0.392   & -0.487   & 0.324 & 0.526 & 1.182  & -0.022 \\
                                       & (1.994) & (13.516) & (6.716) & (1.799) & (-2.624) & (-3.939) & (-0.544) & (-0.624) & (-1.568) & (-1.425) &                                 \\

        \bottomrule
        \bottomrule
        \end{tabular}
      \end{table*}



@ Table 4: Out of sample forecast, DM tests


\begin{table*}[!htb]
  \renewcommand\multirowsetup{\centering}
    \caption{Out-of-Sample Forecast Comparison with D-M test}\label{tab:dm_comparison}
    \centering % centering table
    \scriptsize
    \begin{tabular}{llc*{11}{S[table-format=1.2,table-number-alignment = center]}}
      % >{\raggedleft\arraybackslash}p{5em}
  \toprule
  \toprule
  \\
  % \multicolumn{10}{l}{RV(T)J$^{+(-)}$:${RV}_{t,t+h}=\alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M}$}\\
  % \multicolumn{2}{c}{RV(T)SJ:}
  % & \multicolumn{13}{l}{
  % $\begin{array} {rcl} {RV}_{t,t+h} & = & \alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} \\
  % & + & \beta_{JD}^{+} (T)J^{+}_{D}+\beta_{JW}^{+} (T)J^{+}_{W}+\beta_{JM}^{+} (T)J^{+}_{M}\\
  % & + & \beta_{JD}^{-} (T)J^{-}_{D}+\beta_{JW}^{-} (T)J^{-}_{W}+\beta_{JM}^{-} (T)J^{-}_{M} +\varepsilon_{t,t+h} \end{array}$
  % }\\

  \multicolumn{2}{c}{}
  &\multicolumn{2}{c}{HAR$-$RVSJ} &
  &\multicolumn{2}{c}{HAR$-$RVSTJ} &
  &\multicolumn{2}{c}{RVJ$-$RVSJ} &
  &\multicolumn{2}{c}{RVTJ$-$RVSTJ}
\\
  \cmidrule{3-4}
  \cmidrule{6-7}
  \cmidrule{9-10}
  \cmidrule{12-13}\\
  \multicolumn{2}{c}{}
  &\multicolumn{1}{c}{BTC-D}
  &\multicolumn{1}{c}{BTC-G}
  & &\multicolumn{1}{c}{BTC-D}
  &\multicolumn{1}{c}{BTC-G}
  & &\multicolumn{1}{c}{BTC-D}
  &\multicolumn{1}{c}{BTC-G}
  & &\multicolumn{1}{c}{BTC-D}
  &\multicolumn{1}{c}{BTC-G}\\

  \multicolumn{2}{l}{\textbf{Square form}}\\
  \cline{1-2}\\
  \multicolumn{2}{l}{h =1}  & 0.473         & -2.072\twoS   && -0.095        & -1.847\oneS   && 1.495         & -2.499\twoS   && 0.193         & -1.555 \\
  \multicolumn{2}{l}{h =7}  & 11.252\threeS & -3.51\threeS  && 13.074\threeS & -0.775        && 2.776\threeS  & -3.503\threeS && 14.276\threeS & -0.423 \\
  \multicolumn{2}{l}{h =30} & 5.851\threeS  & -9.755\threeS && 12.398\threeS & -4.843\threeS && -7.038\threeS & -5.791\threeS && 0.232         & -0.36  \\
                                                                                                                                                          \\

\multicolumn{2}{l}{\textbf{Logarithmic form}}                                                                                                             \\
\cline{1-2}                                                                                                                                               \\
  \multicolumn{2}{l}{h =1}  & -0.854       & 1.255  & & 0.095         & 0.086        & & -1.400       & -0.156       & & -1.692\oneS & 1.027        \\
  \multicolumn{2}{l}{h =7}  & 2.231\twoS   & -0.068 & & 3.544\threeS  & 0.757        & & -1.736       & -0.997       & & 0.195       & 0.453        \\
  \multicolumn{2}{l}{h =30} &12.743\threeS & -0.766 & & 15.021\threeS & 5.467\threeS & & 2.765\threeS & 7.415\threeS & & 1.304       & 6.747\threeS \\
\\
    \bottomrule
    \bottomrule
    \end{tabular}
  \end{table*}


@ RSV type full sample Regression

\begin{table}[!htb]
  \centering % centering table
  \begin{threeparttable}
    \caption{In-Sample Fitting and Forecasting, RSV-type HAR}\label{tab:FullSampleFit_RSV}
    \tiny
    \begin{tabular}{p{1.0cm}*{13}{S[table-format=1.1, table-number-alignment = center]}} % ,table-number-alignment = center
  \toprule
  \toprule
  &\multicolumn{6}{c}{Square form}
  &\multicolumn{1}{c}{}
  &\multicolumn{6}{c}{Logarithmic form}\\
  \cline{2-7}
  \cline{9-14}\\

  \multicolumn{1}{c}{}
  &\multicolumn{2}{c}{HAR-RSV}
  &\multicolumn{2}{c}{RSVSJ}
  &\multicolumn{2}{c}{RSVSTJ}

  &\multicolumn{1}{c}{}

  &\multicolumn{2}{c}{HAR-RSV}
  &\multicolumn{2}{c}{RSVSJ}
  &\multicolumn{2}{c}{RSVSTJ}
  \\

  \midrule

  \multicolumn{13}{l}{\textbf{h=1}, \textbf{BTC-D}}\\
  \cline{1-3}

  \rule{0pt}{4ex}$\alpha$         & 0.170  & (2.257)  & 0.407  & (2.364)  & 0.317  & (2.140)   & & 0.534 & (14.328) & 0.833  & (6.268)  & 0.786  & (7.646)  \\
  \rule{0pt}{4ex}$\beta_{D}^{+}$  & -0.161 & (-0.379) & 0.839  & (0.615)  & -1.603 & (-1.376) & & 0.202 & (2.999)  & 0.233  & (3.025)  & 0.255  & (3.299)  \\
  \rule{0pt}{4ex}$\beta_{W}^{+}$  & -0.803 & (-1.599) & -1.858 & (-1.069) & -1.049 & (-0.629) & & 0.045 & (0.434)  & 0.126  & (1.027)  & 0.212  & (1.713)  \\
  \rule{0pt}{4ex}$\beta_{M}^{+}$  & -0.217 & (-0.27)  & 0.094  & (0.023)  & 3.722  & (0.656)  & & 0.069 & (0.519)  & -0.005 & (-0.027) & -0.005 & (-0.029) \\
  \rule{0pt}{4ex}$\beta_{D}^{-}$  & 1.008  & (2.417)  & 0.023  & (0.015)  & 2.568  & (2.161)  & & 0.375 & (5.939)  & 0.349  & (4.473)  & 0.353  & (4.557)  \\
  \rule{0pt}{4ex}$\beta_{W}^{-}$  & 0.986  & (1.877)  & 1.979  & (1.084)  & 1.176  & (0.682)  & & 0.182 & (1.719)  & 0.182  & (1.379)  & 0.079  & (0.624)  \\
  \rule{0pt}{4ex}$\beta_{M}^{-}$  & 0.834  & (0.989)  & 0.948  & (0.231)  & -2.905 & (-0.52)  & & 0.057 & (0.421)  & 0.137  & (0.671)  & 0.104  & (0.54)   \\
  \rule{0pt}{4ex}$\beta_{JD}^{+}$ &        &          & -1.608 & (-0.909) & 1.095  & (0.827)  & &       &          & -0.319 & (-1.284) & -0.454 & (-2.164) \\
  \rule{0pt}{4ex}$\beta_{JW}^{+}$ &        &          & 2.091  & (0.883)  & 0.623  & (0.399)  & &       &          & -1.228 & (-2.255) & -1.367 & (-3.09)  \\
  \rule{0pt}{4ex}$\beta_{JM}^{+}$ &        &          & -2.449 & (-0.41)  & -5.764 & (-0.874) & &       &          & 0.574  & (0.728)  & 0.542  & (0.755)  \\
  \rule{0pt}{4ex}$\beta_{JD}^{-}$ &        &          & 1.381  & (0.473)  & -2.307 & (-1.657) & &       &          & -0.157 & (-0.456) & -0.264 & (-1.106) \\
  \rule{0pt}{4ex}$\beta_{JW}^{-}$ &        &          & -1.968 & (-0.471) & -0.446 & (-0.228) & &       &          & -0.989 & (-1.23)  & -0.178 & (-0.363) \\
  \rule{0pt}{4ex}$\beta_{JM}^{-}$ &        &          & -4.853 & (-0.682) & 3.128  & (0.482)  & &       &          & -1.279 & (-0.902) & -0.586 & (-0.746) \\
  \\
  Adj-$R^2$ & \multicolumn{2}{c}{0.333} & \multicolumn{2}{c}{0.340} & \multicolumn{2}{c}{0.345} & & \multicolumn{2}{c}{0.339} & \multicolumn{2}{c}{0.359} & \multicolumn{2}{c}{0.360} \\
  MSE      & \multicolumn{2}{c}{2.829} & \multicolumn{2}{c}{2.797} & \multicolumn{2}{c}{2.778} & & \multicolumn{2}{c}{2.921} & \multicolumn{2}{c}{2.894} & \multicolumn{2}{c}{2.882} \\
  HRMSE    & \multicolumn{2}{c}{1.810} & \multicolumn{2}{c}{2.122} & \multicolumn{2}{c}{1.930} & & \multicolumn{2}{c}{0.721} & \multicolumn{2}{c}{0.712} & \multicolumn{2}{c}{0.710} \\
  QLIKE    & \multicolumn{2}{c}{1.379} & \multicolumn{2}{c}{1.429} & \multicolumn{2}{c}{1.414} & & \multicolumn{2}{c}{0.609} & \multicolumn{2}{c}{0.606} & \multicolumn{2}{c}{0.605} \\
  \\
  \cline{2-7}
  \cline{9-14}\\
  \multicolumn{13}{l}{\textbf{h=1}, \textbf{BTC-G}}\\
  \cline{1-3}

  \rule{0pt}{4ex}$\alpha$         & 0.169   & (2.048)   & 0.421     & (3.819)    & 0.443      & (4.441)  & & 0.485   & (10.05)   & 1.009     & (5.733)    & 0.949      & (6.58)   \\
  \rule{0pt}{4ex}$\beta_{D}^{+}$  & 0.406   & (1.289)   & -0.862    & (-1.544)   & -0.671     & (-0.574) & & 0.238   & (4.129)   & 0.268     & (3.665)    & 0.317      & (4.115)  \\
  \rule{0pt}{4ex}$\beta_{W}^{+}$  & -0.216  & (-0.619)  & -0.883    & (-0.526)   & -3.545     & (-1.207) & & 0.103   & (1.032)   & 0.229     & (1.768)    & 0.259      & (1.883)  \\
  \rule{0pt}{4ex}$\beta_{M}^{+}$  & 0.382   & (0.719)   & -2.210    & (-0.83)    & -7.760     & (-1.058) & & 0.235   & (2.205)   & 0.218     & (1.101)    & 0.150      & (0.715)  \\
  \rule{0pt}{4ex}$\beta_{D}^{-}$  & 0.267   & (0.856)   & 1.633     & (3.089)    & 1.511      & (1.289)  & & 0.303   & (5.47)    & 0.279     & (3.848)    & 0.247      & (3.271)  \\
  \rule{0pt}{4ex}$\beta_{W}^{-}$  & 0.501   & (1.45)    & 1.512     & (0.934)    & 4.076      & (1.359)  & & 0.146   & (1.566)   & 0.132     & (1.163)    & 0.100      & (0.84)   \\
  \rule{0pt}{4ex}$\beta_{M}^{-}$  & 0.302   & (0.621)   & 3.027     & (1.155)    & 8.361      & (1.123)  & & -0.109  & (-0.98)   & -0.063    & (-0.324)   & -0.044     & (-0.213) \\
  \rule{0pt}{4ex}$\beta_{JD}^{+}$ &         &           & 0.640     & (0.634)    & 0.085      & (0.058)  & &         &           & -0.490    & (-1.413)   & -0.689     & (-2.241) \\
  \rule{0pt}{4ex}$\beta_{JW}^{+}$ &         &           & -2.097    & (-0.752)   & 1.586      & (0.541)  & &         &           & -1.969    & (-3.457)   & -1.799     & (-3.397) \\
  \rule{0pt}{4ex}$\beta_{JM}^{+}$ &         &           & 0.582     & (0.136)    & 7.011      & (0.861)  & &         &           & -1.422    & (-1.124)   & -0.710     & (-0.689) \\
  \rule{0pt}{4ex}$\beta_{JD}^{-}$ &         &           & -1.761    & (-2.949)   & -1.329     & (-1.044) & &         &           & -0.210    & (-0.698)   & -0.060     & (-0.258) \\
  \rule{0pt}{4ex}$\beta_{JW}^{-}$ &         &           & -1.750    & (-1.035)   & -3.779     & (-1.251) & &         &           & -0.648    & (-2.16)    & -0.152     & (-0.557) \\
  \rule{0pt}{4ex}$\beta_{JM}^{-}$ &         &           & -3.478    & (-1.254)   & -8.551     & (-1.109) & &         &           & -0.362    & (-0.594)   & -0.228     & (-0.385) \\
  \\
  Adj-$R^2$ & \multicolumn{2}{c}{0.231} & \multicolumn{2}{c}{0.268} & \multicolumn{2}{c}{0.268} & & \multicolumn{2}{c}{0.259} & \multicolumn{2}{c}{0.290} & \multicolumn{2}{c}{0.299} \\
  MSE       & \multicolumn{2}{c}{2.319} & \multicolumn{2}{c}{2.210} & \multicolumn{2}{c}{2.208} & & \multicolumn{2}{c}{2.338} & \multicolumn{2}{c}{2.280} & \multicolumn{2}{c}{2.256} \\
  HRMSE     & \multicolumn{2}{c}{3.564} & \multicolumn{2}{c}{4.770} & \multicolumn{2}{c}{5.125} & & \multicolumn{2}{c}{1.074} & \multicolumn{2}{c}{1.058} & \multicolumn{2}{c}{1.056} \\
  QLIKE     & \multicolumn{2}{c}{1.843} & \multicolumn{2}{c}{2.078} & \multicolumn{2}{c}{2.167} & & \multicolumn{2}{c}{0.420} & \multicolumn{2}{c}{0.413} & \multicolumn{2}{c}{0.411} \\

    \bottomrule
    \bottomrule
    \end{tabular}
% Day-ahead Forecast Regression Results on BTC-G, $\alpha=0.9999$, $c_{\theta}=3$, 5-minutes frequency
\begin{tablenotes}
  \tiny
  \item $\alpha=99.99\%$, 5-minutes Frequency, $C_\theta=3$
  \item $^{\dagger}:$ D-M test with quadratic loss. Logarithmic form models against corresponding square form models. Significant positive statistics implies that logarithmic models perform better, vice versa.
  \item $^{\ddagger}:$ D-M test with quadratic loss. Models with jumps against HAR model. Significant positive statistics implies that HAR model perform worse, vice versa.
  \item \threeS: 1\% significance, \twoS: 5\% significance, \oneS: 10\% significance
\end{tablenotes}
\end{threeparttable}

  \end{table}


==> RSVtype_FullSampleFit.tex <==

% BTC-D, square form

{} & SRV\_idxv   & SRV\_v & SRV\_idxt           & SRV\_t   & SRV\_idxm & SRV\_m & SRVSJ\_idxv    & SRVSJ\_v & SRVSJ\_idxt            & SRVSJ\_t & SRVSJ\_idxm & SRVSJ\_m & SRVSTJ\_idxv    & SRVSTJ\_v & SRVSTJ\_idxt            & SRVSTJ\_t & SRVSTJ\_idxm & SRVSTJ\_m \\
\midrule
0  & Intercept   & 0.170  & Intercept\_tvalue   & (2.257)  & M-Z-R2    & 0.333  & Intercept      & 0.407    & Intercept\_tvalue      & (2.364)  & M-Z-R2      & 0.340    & Intercept       & 0.317     & Intercept\_tvalue       & (2.14)    & M-Z-R2       & 0.345     \\
1  & RSVP\_day   & -0.161 & RSVP\_day\_tvalue   & (-0.379) & MSE       & 2.829  & RSVP\_day      & 0.839    & RSVP\_day\_tvalue      & (0.615)  & MSE         & 2.797    & RSVP\_day       & -1.603    & RSVP\_day\_tvalue       & (-1.376)  & MSE          & 2.778     \\
2  & RSVP\_week  & -0.803 & RSVP\_week\_tvalue  & (-1.599) & HRMSE     & 1.810  & RSVP\_week     & -1.858   & RSVP\_week\_tvalue     & (-1.069) & HRMSE       & 2.122    & RSVP\_week      & -1.049    & RSVP\_week\_tvalue      & (-0.629)  & HRMSE        & 1.930     \\
3  & RSVP\_month & -0.217 & RSVP\_month\_tvalue & (-0.27)  & QLIKE     & 1.379  & RSVP\_month    & 0.094    & RSVP\_month\_tvalue    & (0.023)  & QLIKE       & 1.429    & RSVP\_month     & 3.722     & RSVP\_month\_tvalue     & (0.656)   & QLIKE        & 1.414     \\
4  & RSVN\_day   & 1.008  & RSVN\_day\_tvalue   & (2.417)  & NaN       & NaN    & RSVN\_day      & 0.023    & RSVN\_day\_tvalue      & (0.015)  & NaN         & NaN      & RSVN\_day       & 2.568     & RSVN\_day\_tvalue       & (2.161)   & NaN          & NaN       \\
5  & RSVN\_week  & 0.986  & RSVN\_week\_tvalue  & (1.877)  & NaN       & NaN    & RSVN\_week     & 1.979    & RSVN\_week\_tvalue     & (1.084)  & NaN         & NaN      & RSVN\_week      & 1.176     & RSVN\_week\_tvalue      & (0.682)   & NaN          & NaN       \\
6  & RSVN\_month & 0.834  & RSVN\_month\_tvalue & (0.989)  & NaN       & NaN    & RSVN\_month    & 0.948    & RSVN\_month\_tvalue    & (0.231)  & NaN         & NaN      & RSVN\_month     & -2.905    & RSVN\_month\_tvalue     & (-0.52)   & NaN          & NaN       \\
7  & NaN         & NaN    & NaN                 & NaN      & NaN       & NaN    & Jump\_p\_day   & -1.608   & Jump\_p\_day\_tvalue   & (-0.909) & NaN         & NaN      & TJump\_p\_day   & 1.095     & TJump\_p\_day\_tvalue   & (0.827)   & NaN          & NaN       \\
8  & NaN         & NaN    & NaN                 & NaN      & NaN       & NaN    & Jump\_p\_week  & 2.091    & Jump\_p\_week\_tvalue  & (0.883)  & NaN         & NaN      & TJump\_p\_week  & 0.623     & TJump\_p\_week\_tvalue  & (0.399)   & NaN          & NaN       \\
9  & NaN         & NaN    & NaN                 & NaN      & NaN       & NaN    & Jump\_p\_month & -2.449   & Jump\_p\_month\_tvalue & (-0.41)  & NaN         & NaN      & TJump\_p\_month & -5.764    & TJump\_p\_month\_tvalue & (-0.874)  & NaN          & NaN       \\
10 & NaN         & NaN    & NaN                 & NaN      & NaN       & NaN    & Jump\_n\_day   & 1.381    & Jump\_n\_day\_tvalue   & (0.473)  & NaN         & NaN      & TJump\_n\_day   & -2.307    & TJump\_n\_day\_tvalue   & (-1.657)  & NaN          & NaN       \\
11 & NaN         & NaN    & NaN                 & NaN      & NaN       & NaN    & Jump\_n\_week  & -1.968   & Jump\_n\_week\_tvalue  & (-0.471) & NaN         & NaN      & TJump\_n\_week  & -0.446    & TJump\_n\_week\_tvalue  & (-0.228)  & NaN          & NaN       \\
12 & NaN         & NaN    & NaN                 & NaN      & NaN       & NaN    & Jump\_n\_month & -4.853   & Jump\_n\_month\_tvalue & (-0.682) & NaN         & NaN      & TJump\_n\_month & 3.128     & TJump\_n\_month\_tvalue & (0.482)   & NaN          & NaN       \\


{}           & 0                 & 1                 & 2                  & 3                   & 4                 & 5                  & 6                   & 7                     & 8                      & 9                       & 10                    & 11                     & 12                      \\
\midrule
SRV\_idxv    & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_v       & 0.17              & -0.161            & -0.803             & -0.217              & 1.008             & 0.986              & 0.834               & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_idxt    & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_t       & (2.257)           & (-0.379)          & (-1.599)           & (-0.27)             & (2.417)           & (1.877)            & (0.989)             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_idxm    & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_m       & 0.333             & 2.829             & 1.81               & 1.379               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSJ\_idxv  & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
SRVSJ\_v     & 0.407             & 0.839             & -1.858             & 0.094               & 0.023             & 1.979              & 0.948               & -1.608                & 2.091                  & -2.449                  & 1.381                 & -1.968                 & -4.853                  \\
SRVSJ\_idxt  & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
SRVSJ\_t     & (2.364)           & (0.615)           & (-1.069)           & (0.023)             & (0.015)           & (1.084)            & (0.231)             & (-0.909)              & (0.883)                & (-0.41)                 & (0.473)               & (-0.471)               & (-0.682)                \\
SRVSJ\_idxm  & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSJ\_m     & 0.34              & 2.797             & 2.122              & 1.429               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSTJ\_idxv & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
SRVSTJ\_v    & 0.317             & -1.603            & -1.049             & 3.722               & 2.568             & 1.176              & -2.905              & 1.095                 & 0.623                  & -5.764                  & -2.307                & -0.446                 & 3.128                   \\
SRVSTJ\_idxt & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
SRVSTJ\_t    & (2.14)            & (-1.376)          & (-0.629)           & (0.656)             & (2.161)           & (0.682)            & (-0.52)             & (0.827)               & (0.399)                & (-0.874)                & (-1.657)              & (-0.228)               & (0.482)                 \\
SRVSTJ\_idxm & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSTJ\_m    & 0.345             & 2.778             & 1.93               & 1.414               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\



% BTC-D, logarithmic form

{} &    SRV\_idxv &  SRV\_v &           SRV\_idxt &     SRV\_t & SRV\_idxm &  SRV\_m &    SRVSJ\_idxv &  SRVSJ\_v &           SRVSJ\_idxt &   SRVSJ\_t & SRVSJ\_idxm &  SRVSJ\_m &    SRVSTJ\_idxv &  SRVSTJ\_v &           SRVSTJ\_idxt &  SRVSTJ\_t & SRVSTJ\_idxm &  SRVSTJ\_m \\
\midrule
0  &   Intercept &  0.534 &   Intercept\_tvalue &  (14.328) &   M-Z-R2 &  0.339 &     Intercept &    0.833 &     Intercept\_tvalue &   (6.268) &     M-Z-R2 &    0.359 &      Intercept &     0.786 &      Intercept\_tvalue &   (7.646) &      M-Z-R2 &     0.360 \\
1  &    RSVP\_day &  0.202 &    RSVP\_day\_tvalue &   (2.999) &      MSE &  2.921 &      RSVP\_day &    0.233 &      RSVP\_day\_tvalue &   (3.025) &        MSE &    2.894 &       RSVP\_day &     0.255 &       RSVP\_day\_tvalue &   (3.299) &         MSE &     2.882 \\
2  &   RSVP\_week &  0.045 &   RSVP\_week\_tvalue &   (0.434) &    HRMSE &  0.721 &     RSVP\_week &    0.126 &     RSVP\_week\_tvalue &   (1.027) &      HRMSE &    0.712 &      RSVP\_week &     0.212 &      RSVP\_week\_tvalue &   (1.713) &       HRMSE &     0.710 \\
3  &  RSVP\_month &  0.069 &  RSVP\_month\_tvalue &   (0.519) &    QLIKE &  0.609 &    RSVP\_month &   -0.005 &    RSVP\_month\_tvalue &  (-0.027) &      QLIKE &    0.606 &     RSVP\_month &    -0.005 &     RSVP\_month\_tvalue &  (-0.029) &       QLIKE &     0.605 \\
4  &    RSVN\_day &  0.375 &    RSVN\_day\_tvalue &   (5.939) &      NaN &    NaN &      RSVN\_day &    0.349 &      RSVN\_day\_tvalue &   (4.473) &        NaN &      NaN &       RSVN\_day &     0.353 &       RSVN\_day\_tvalue &   (4.557) &         NaN &       NaN \\
5  &   RSVN\_week &  0.182 &   RSVN\_week\_tvalue &   (1.719) &      NaN &    NaN &     RSVN\_week &    0.182 &     RSVN\_week\_tvalue &   (1.379) &        NaN &      NaN &      RSVN\_week &     0.079 &      RSVN\_week\_tvalue &   (0.624) &         NaN &       NaN \\
6  &  RSVN\_month &  0.057 &  RSVN\_month\_tvalue &   (0.421) &      NaN &    NaN &    RSVN\_month &    0.137 &    RSVN\_month\_tvalue &   (0.671) &        NaN &      NaN &     RSVN\_month &     0.104 &     RSVN\_month\_tvalue &    (0.54) &         NaN &       NaN \\
7  &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &    Jump\_p\_day &   -0.319 &    Jump\_p\_day\_tvalue &  (-1.284) &        NaN &      NaN &    TJump\_p\_day &    -0.454 &    TJump\_p\_day\_tvalue &  (-2.164) &         NaN &       NaN \\
8  &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &   Jump\_p\_week &   -1.228 &   Jump\_p\_week\_tvalue &  (-2.255) &        NaN &      NaN &   TJump\_p\_week &    -1.367 &   TJump\_p\_week\_tvalue &   (-3.09) &         NaN &       NaN \\
9  &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &  Jump\_p\_month &    0.574 &  Jump\_p\_month\_tvalue &   (0.728) &        NaN &      NaN &  TJump\_p\_month &     0.542 &  TJump\_p\_month\_tvalue &   (0.755) &         NaN &       NaN \\
10 &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &    Jump\_n\_day &   -0.157 &    Jump\_n\_day\_tvalue &  (-0.456) &        NaN &      NaN &    TJump\_n\_day &    -0.264 &    TJump\_n\_day\_tvalue &  (-1.106) &         NaN &       NaN \\
11 &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &   Jump\_n\_week &   -0.989 &   Jump\_n\_week\_tvalue &   (-1.23) &        NaN &      NaN &   TJump\_n\_week &    -0.178 &   TJump\_n\_week\_tvalue &  (-0.363) &         NaN &       NaN \\
12 &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &  Jump\_n\_month &   -1.279 &  Jump\_n\_month\_tvalue &  (-0.902) &        NaN &      NaN &  TJump\_n\_month &    -0.586 &  TJump\_n\_month\_tvalue &  (-0.746) &         NaN &       NaN \\


{}           & 0                 & 1                 & 2                  & 3                   & 4                 & 5                  & 6                   & 7                     & 8                      & 9                       & 10                    & 11                     & 12                      \\
\midrule
SRV\_idxv    & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_v       & 0.534             & 0.202             & 0.045              & 0.069               & 0.375             & 0.182              & 0.057               & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_idxt    & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_t       & (14.328)          & (2.999)           & (0.434)            & (0.519)             & (5.939)           & (1.719)            & (0.421)             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_idxm    & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_m       & 0.339             & 2.921             & 0.721              & 0.609               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSJ\_idxv  & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
SRVSJ\_v     & 0.833             & 0.233             & 0.126              & -0.005              & 0.349             & 0.182              & 0.137               & -0.319                & -1.228                 & 0.574                   & -0.157                & -0.989                 & -1.279                  \\
SRVSJ\_idxt  & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
SRVSJ\_t     & (6.268)           & (3.025)           & (1.027)            & (-0.027)            & (4.473)           & (1.379)            & (0.671)             & (-1.284)              & (-2.255)               & (0.728)                 & (-0.456)              & (-1.23)                & (-0.902)                \\
SRVSJ\_idxm  & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSJ\_m     & 0.359             & 2.894             & 0.712              & 0.606               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSTJ\_idxv & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
SRVSTJ\_v    & 0.786             & 0.255             & 0.212              & -0.005              & 0.353             & 0.079              & 0.104               & -0.454                & -1.367                 & 0.542                   & -0.264                & -0.178                 & -0.586                  \\
SRVSTJ\_idxt & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
SRVSTJ\_t    & (7.646)           & (3.299)           & (1.713)            & (-0.029)            & (4.557)           & (0.624)            & (0.54)              & (-2.164)              & (-3.09)                & (0.755)                 & (-1.106)              & (-0.363)               & (-0.746)                \\
SRVSTJ\_idxm & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSTJ\_m    & 0.36              & 2.882             & 0.71               & 0.605               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\



% BTC-G, square form



{} &    SRV\_idxv &  SRV\_v &           SRV\_idxt &     SRV\_t & SRV\_idxm &  SRV\_m &    SRVSJ\_idxv &  SRVSJ\_v &           SRVSJ\_idxt &   SRVSJ\_t & SRVSJ\_idxm &  SRVSJ\_m &    SRVSTJ\_idxv &  SRVSTJ\_v &           SRVSTJ\_idxt &  SRVSTJ\_t & SRVSTJ\_idxm &  SRVSTJ\_m \\
\midrule
0  &   Intercept &  0.169 &   Intercept\_tvalue &   (2.048) &   M-Z-R2 &  0.231 &     Intercept &    0.421 &     Intercept\_tvalue &   (3.819) &     M-Z-R2 &    0.268 &      Intercept &     0.443 &      Intercept\_tvalue &   (4.441) &      M-Z-R2 &     0.268 \\
1  &    RSVP\_day &  0.406 &    RSVP\_day\_tvalue &   (1.289) &      MSE &  2.319 &      RSVP\_day &   -0.862 &      RSVP\_day\_tvalue &  (-1.544) &        MSE &    2.210 &       RSVP\_day &    -0.671 &       RSVP\_day\_tvalue &  (-0.574) &         MSE &     2.208 \\
2  &   RSVP\_week & -0.216 &   RSVP\_week\_tvalue &  (-0.619) &    HRMSE &  3.564 &     RSVP\_week &   -0.883 &     RSVP\_week\_tvalue &  (-0.526) &      HRMSE &    4.770 &      RSVP\_week &    -3.545 &      RSVP\_week\_tvalue &  (-1.207) &       HRMSE &     5.125 \\
3  &  RSVP\_month &  0.382 &  RSVP\_month\_tvalue &   (0.719) &    QLIKE &  1.843 &    RSVP\_month &   -2.210 &    RSVP\_month\_tvalue &   (-0.83) &      QLIKE &    2.078 &     RSVP\_month &    -7.760 &     RSVP\_month\_tvalue &  (-1.058) &       QLIKE &     2.167 \\
4  &    RSVN\_day &  0.267 &    RSVN\_day\_tvalue &   (0.856) &      NaN &    NaN &      RSVN\_day &    1.633 &      RSVN\_day\_tvalue &   (3.089) &        NaN &      NaN &       RSVN\_day &     1.511 &       RSVN\_day\_tvalue &   (1.289) &         NaN &       NaN \\
5  &   RSVN\_week &  0.501 &   RSVN\_week\_tvalue &    (1.45) &      NaN &    NaN &     RSVN\_week &    1.512 &     RSVN\_week\_tvalue &   (0.934) &        NaN &      NaN &      RSVN\_week &     4.076 &      RSVN\_week\_tvalue &   (1.359) &         NaN &       NaN \\
6  &  RSVN\_month &  0.302 &  RSVN\_month\_tvalue &   (0.621) &      NaN &    NaN &    RSVN\_month &    3.027 &    RSVN\_month\_tvalue &   (1.155) &        NaN &      NaN &     RSVN\_month &     8.361 &     RSVN\_month\_tvalue &   (1.123) &         NaN &       NaN \\
7  &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &    Jump\_p\_day &    0.640 &    Jump\_p\_day\_tvalue &   (0.634) &        NaN &      NaN &    TJump\_p\_day &     0.085 &    TJump\_p\_day\_tvalue &   (0.058) &         NaN &       NaN \\
8  &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &   Jump\_p\_week &   -2.097 &   Jump\_p\_week\_tvalue &  (-0.752) &        NaN &      NaN &   TJump\_p\_week &     1.586 &   TJump\_p\_week\_tvalue &   (0.541) &         NaN &       NaN \\
9  &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &  Jump\_p\_month &    0.582 &  Jump\_p\_month\_tvalue &   (0.136) &        NaN &      NaN &  TJump\_p\_month &     7.011 &  TJump\_p\_month\_tvalue &   (0.861) &         NaN &       NaN \\
10 &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &    Jump\_n\_day &   -1.761 &    Jump\_n\_day\_tvalue &  (-2.949) &        NaN &      NaN &    TJump\_n\_day &    -1.329 &    TJump\_n\_day\_tvalue &  (-1.044) &         NaN &       NaN \\
11 &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &   Jump\_n\_week &   -1.750 &   Jump\_n\_week\_tvalue &  (-1.035) &        NaN &      NaN &   TJump\_n\_week &    -3.779 &   TJump\_n\_week\_tvalue &  (-1.251) &         NaN &       NaN \\
12 &         NaN &    NaN &                NaN &       NaN &      NaN &    NaN &  Jump\_n\_month &   -3.478 &  Jump\_n\_month\_tvalue &  (-1.254) &        NaN &      NaN &  TJump\_n\_month &    -8.551 &  TJump\_n\_month\_tvalue &  (-1.109) &         NaN &       NaN \\


{}           & 0                 & 1                 & 2                  & 3                   & 4                 & 5                  & 6                   & 7                     & 8                      & 9                       & 10                    & 11                     & 12                      \\
\midrule
SRV\_idxv    & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_v       & 0.169             & 0.406             & -0.216             & 0.382               & 0.267             & 0.501              & 0.302               & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_idxt    & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_t       & (2.048)           & (1.289)           & (-0.619)           & (0.719)             & (0.856)           & (1.45)             & (0.621)             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_idxm    & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_m       & 0.231             & 2.319             & 3.564              & 1.843               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSJ\_idxv  & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
SRVSJ\_v     & 0.421             & -0.862            & -0.883             & -2.21               & 1.633             & 1.512              & 3.027               & 0.64                  & -2.097                 & 0.582                   & -1.761                & -1.75                  & -3.478                  \\
SRVSJ\_idxt  & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
SRVSJ\_t     & (3.819)           & (-1.544)          & (-0.526)           & (-0.83)             & (3.089)           & (0.934)            & (1.155)             & (0.634)               & (-0.752)               & (0.136)                 & (-2.949)              & (-1.035)               & (-1.254)                \\
SRVSJ\_idxm  & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSJ\_m     & 0.268             & 2.21              & 4.77               & 2.078               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSTJ\_idxv & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
SRVSTJ\_v    & 0.443             & -0.671            & -3.545             & -7.76               & 1.511             & 4.076              & 8.361               & 0.085                 & 1.586                  & 7.011                   & -1.329                & -3.779                 & -8.551                  \\
SRVSTJ\_idxt & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
SRVSTJ\_t    & (4.441)           & (-0.574)          & (-1.207)           & (-1.058)            & (1.289)           & (1.359)            & (1.123)             & (0.058)               & (0.541)                & (0.861)                 & (-1.044)              & (-1.251)               & (-1.109)                \\
SRVSTJ\_idxm & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSTJ\_m    & 0.268             & 2.208             & 5.125              & 2.167               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\






% BTC-G, logarithmic form

{} &    SRV\_idxv &  SRV\_v &           SRV\_idxt &    SRV\_t & SRV\_idxm &  SRV\_m &    SRVSJ\_idxv &  SRVSJ\_v &           SRVSJ\_idxt &   SRVSJ\_t & SRVSJ\_idxm &  SRVSJ\_m &    SRVSTJ\_idxv &  SRVSTJ\_v &           SRVSTJ\_idxt &  SRVSTJ\_t & SRVSTJ\_idxm &  SRVSTJ\_m \\
\midrule
0  &   Intercept &  0.485 &   Intercept\_tvalue &  (10.05) &   M-Z-R2 &  0.259 &     Intercept &    1.009 &     Intercept\_tvalue &   (5.733) &     M-Z-R2 &    0.290 &      Intercept &     0.949 &      Intercept\_tvalue &    (6.58) &      M-Z-R2 &     0.299 \\
1  &    RSVP\_day &  0.238 &    RSVP\_day\_tvalue &  (4.129) &      MSE &  2.338 &      RSVP\_day &    0.268 &      RSVP\_day\_tvalue &   (3.665) &        MSE &    2.280 &       RSVP\_day &     0.317 &       RSVP\_day\_tvalue &   (4.115) &         MSE &     2.256 \\
2  &   RSVP\_week &  0.103 &   RSVP\_week\_tvalue &  (1.032) &    HRMSE &  1.074 &     RSVP\_week &    0.229 &     RSVP\_week\_tvalue &   (1.768) &      HRMSE &    1.058 &      RSVP\_week &     0.259 &      RSVP\_week\_tvalue &   (1.883) &       HRMSE &     1.056 \\
3  &  RSVP\_month &  0.235 &  RSVP\_month\_tvalue &  (2.205) &    QLIKE &  0.420 &    RSVP\_month &    0.218 &    RSVP\_month\_tvalue &   (1.101) &      QLIKE &    0.413 &     RSVP\_month &     0.150 &     RSVP\_month\_tvalue &   (0.715) &       QLIKE &     0.411 \\
4  &    RSVN\_day &  0.303 &    RSVN\_day\_tvalue &   (5.47) &      NaN &    NaN &      RSVN\_day &    0.279 &      RSVN\_day\_tvalue &   (3.848) &        NaN &      NaN &       RSVN\_day &     0.247 &       RSVN\_day\_tvalue &   (3.271) &         NaN &       NaN \\
5  &   RSVN\_week &  0.146 &   RSVN\_week\_tvalue &  (1.566) &      NaN &    NaN &     RSVN\_week &    0.132 &     RSVN\_week\_tvalue &   (1.163) &        NaN &      NaN &      RSVN\_week &     0.100 &      RSVN\_week\_tvalue &    (0.84) &         NaN &       NaN \\
6  &  RSVN\_month & -0.109 &  RSVN\_month\_tvalue &  (-0.98) &      NaN &    NaN &    RSVN\_month &   -0.063 &    RSVN\_month\_tvalue &  (-0.324) &        NaN &      NaN &     RSVN\_month &    -0.044 &     RSVN\_month\_tvalue &  (-0.213) &         NaN &       NaN \\
7  &         NaN &    NaN &                NaN &      NaN &      NaN &    NaN &    Jump\_p\_day &   -0.490 &    Jump\_p\_day\_tvalue &  (-1.413) &        NaN &      NaN &    TJump\_p\_day &    -0.689 &    TJump\_p\_day\_tvalue &  (-2.241) &         NaN &       NaN \\
8  &         NaN &    NaN &                NaN &      NaN &      NaN &    NaN &   Jump\_p\_week &   -1.969 &   Jump\_p\_week\_tvalue &  (-3.457) &        NaN &      NaN &   TJump\_p\_week &    -1.799 &   TJump\_p\_week\_tvalue &  (-3.397) &         NaN &       NaN \\
9  &         NaN &    NaN &                NaN &      NaN &      NaN &    NaN &  Jump\_p\_month &   -1.422 &  Jump\_p\_month\_tvalue &  (-1.124) &        NaN &      NaN &  TJump\_p\_month &    -0.710 &  TJump\_p\_month\_tvalue &  (-0.689) &         NaN &       NaN \\
10 &         NaN &    NaN &                NaN &      NaN &      NaN &    NaN &    Jump\_n\_day &   -0.210 &    Jump\_n\_day\_tvalue &  (-0.698) &        NaN &      NaN &    TJump\_n\_day &    -0.060 &    TJump\_n\_day\_tvalue &  (-0.258) &         NaN &       NaN \\
11 &         NaN &    NaN &                NaN &      NaN &      NaN &    NaN &   Jump\_n\_week &   -0.648 &   Jump\_n\_week\_tvalue &   (-2.16) &        NaN &      NaN &   TJump\_n\_week &    -0.152 &   TJump\_n\_week\_tvalue &  (-0.557) &         NaN &       NaN \\
12 &         NaN &    NaN &                NaN &      NaN &      NaN &    NaN &  Jump\_n\_month &   -0.362 &  Jump\_n\_month\_tvalue &  (-0.594) &        NaN &      NaN &  TJump\_n\_month &    -0.228 &  TJump\_n\_month\_tvalue &  (-0.385) &         NaN &       NaN \\


{}           & 0                 & 1                 & 2                  & 3                   & 4                 & 5                  & 6                   & 7                     & 8                      & 9                       & 10                    & 11                     & 12                      \\
\midrule
SRV\_idxv    & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_v       & 0.485             & 0.238             & 0.103              & 0.235               & 0.303             & 0.146              & -0.109              & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_idxt    & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_t       & (10.05)           & (4.129)           & (1.032)            & (2.205)             & (5.47)            & (1.566)            & (-0.98)             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_idxm    & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRV\_m       & 0.259             & 2.338             & 1.074              & 0.42                & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSJ\_idxv  & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
SRVSJ\_v     & 1.009             & 0.268             & 0.229              & 0.218               & 0.279             & 0.132              & -0.063              & -0.49                 & -1.969                 & -1.422                  & -0.21                 & -0.648                 & -0.362                  \\
SRVSJ\_idxt  & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
SRVSJ\_t     & (5.733)           & (3.665)           & (1.768)            & (1.101)             & (3.848)           & (1.163)            & (-0.324)            & (-1.413)              & (-3.457)               & (-1.124)                & (-0.698)              & (-2.16)                & (-0.594)                \\
SRVSJ\_idxm  & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSJ\_m     & 0.29              & 2.28              & 1.058              & 0.413               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSTJ\_idxv & Intercept         & RSVP\_day         & RSVP\_week         & RSVP\_month         & RSVN\_day         & RSVN\_week         & RSVN\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
SRVSTJ\_v    & 0.949             & 0.317             & 0.259              & 0.15                & 0.247             & 0.1                & -0.044              & -0.689                & -1.799                 & -0.71                   & -0.06                 & -0.152                 & -0.228                  \\
SRVSTJ\_idxt & Intercept\_tvalue & RSVP\_day\_tvalue & RSVP\_week\_tvalue & RSVP\_month\_tvalue & RSVN\_day\_tvalue & RSVN\_week\_tvalue & RSVN\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
SRVSTJ\_t    & (6.58)            & (4.115)           & (1.883)            & (0.715)             & (3.271)           & (0.84)             & (-0.213)            & (-2.241)              & (-3.397)               & (-0.689)                & (-0.258)              & (-0.557)               & (-0.385)                \\
SRVSTJ\_idxm & M-Z-R2            & MSE               & HRMSE              & QLIKE               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
SRVSTJ\_m    & 0.299             & 2.256             & 1.056              & 0.411               & NaN               & NaN                & NaN                 & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\


==> RVtype_fullsample_fit_results.tex <==



% BTC-D, Square, 1-day horizon,
% All jumps

{}               & HAR     & HAR\_RVJs & HAR\_RVTJs & HAR\_Exp\_RV\_Js & HAR\_Exp\_RV\_TJs & HAR\_CJPs & HAR\_CJNs & HAR\_RVJPs & HAR\_RVJNs & HAR\_RVTJPs & HAR\_RVTJNs \\
\midrule
alpha            & 0.175   & 0.335     & 0.271      & 0.335            & 0.271             & 0.289     & 0.211     & 0.291      & 0.217      & 0.338       & 0.288       \\
alpha\_tvalue    & (2.46)  & (2.953)   & (1.696)    & (2.953)          & (1.696)           & (2.591)   & (1.304)   & (2.629)    & (1.356)    & (3.694)     & (1.881)     \\
beta\_D          & 0.437   & 0.43      & 0.457      & 0.43             & 0.457             & 0.7       & 0.733     & 0.701      & 0.741      & 0.461       & 0.392       \\
beta\_D\_tvalue  & (6.284) & (6.466)   & (6.47)     & (6.466)          & (6.47)            & (6.672)   & (6.873)   & (6.657)    & (6.899)    & (6.206)     & (4.408)     \\
beta\_W          & 0.1     & 0.089     & 0.089      & 0.089            & 0.089             & -0.46     & -0.482    & 0.605      & -0.497     & 0.112       & 0.066       \\
beta\_W\_tvalue  & (2.119) & (1.862)   & (1.743)    & (1.862)          & (1.743)           & (-2.431)  & (-2.438)  & (3.037)    & (-2.531)   & (1.708)     & (0.987)     \\
beta\_M          & 0.311   & 0.292     & 0.292      & 0.292            & 0.292             & 0.604     & 0.62      & -0.463     & 0.627      & 0.375       & 0.441       \\
beta\_M\_tvalue  & (2.722) & (2.523)   & (2.452)    & (2.523)          & (2.452)           & (3.017)   & (2.945)   & (-2.447)   & (2.985)    & (2.865)     & (3.243)     \\
beta\_JD         & NaN     & 0.68      & -0.476     & 1.11             & -0.02             & 0.682     & -0.402    & 1.096      & 0.02       & -1.213      & 1.257       \\
beta\_JD\_tvalue & NaN     & (0.781)   & (-2.303)   & (1.235)          & (-0.102)          & (0.756)   & (-2.006)  & (1.182)    & (0.1)      & (-2.513)    & (0.884)     \\
beta\_JW         & NaN     & -0.179    & -0.046     & -0.09            & 0.043             & -0.48     & -0.211    & -0.347     & -0.065     & -0.955      & 0.96        \\
beta\_JW\_tvalue & NaN     & (-0.195)  & (-0.112)   & (-0.098)         & (0.11)            & (-0.571)  & (-0.466)  & (-0.409)   & (-0.153)   & (-0.893)    & (0.562)     \\
beta\_JM         & NaN     & -4.216    & -0.538     & -3.925           & -0.246            & -3.717    & -0.213    & -3.485     & 0.027      & -2.408      & -4.417      \\
beta\_JM\_tvalue & NaN     & (-2.494)  & (-0.489)   & (-2.279)         & (-0.211)          & (-2.255)  & (-0.198)  & (-2.079)   & (0.024)    & (-1.801)    & (-1.878)    \\


{}          & 0                 & 1               & 2                & 3                 & 4                     & 5                      & 6                       & 7                     & 8                      & 9                       \\
\midrule
HAR\_idxv   & Intercept         & RV\_day         & RV\_week         & RV\_month         & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_v      & 0.175             & 0.437           & 0.1              & 0.311             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_idxt   & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_t      & (2.46)            & (6.284)         & (2.119)          & (2.722)           & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_idxm   & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_m      & 0.322             & 2.877           & 1.886            & 1.429             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVJ\_idxv   & Intercept         & RV\_day         & RV\_week         & RV\_month         & Jump\_day             & Jump\_week             & Jump\_month             & NaN                   & NaN                    & NaN                     \\
RVJ\_v      & 0.335             & 0.43            & 0.089            & 0.292             & 0.68                  & -0.179                 & -4.216                  & NaN                   & NaN                    & NaN                     \\
RVJ\_idxt   & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & Jump\_day\_tvalue     & Jump\_week\_tvalue     & Jump\_month\_tvalue     & NaN                   & NaN                    & NaN                     \\
RVJ\_t      & (2.953)           & (6.466)         & (1.862)          & (2.523)           & (0.781)               & (-0.195)               & (-2.494)                & NaN                   & NaN                    & NaN                     \\
RVJ\_idxm   & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVJ\_m      & 0.326             & 2.859           & 2.181            & 1.425             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxv  & Intercept         & RV\_day         & RV\_week         & RV\_month         & TJump\_day            & TJump\_week            & TJump\_month            & NaN                   & NaN                    & NaN                     \\
RVTJ\_v     & 0.271             & 0.457           & 0.089            & 0.292             & -0.476                & -0.046                 & -0.538                  & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxt  & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & TJump\_day\_tvalue    & TJump\_week\_tvalue    & TJump\_month\_tvalue    & NaN                   & NaN                    & NaN                     \\
RVTJ\_t     & (1.696)           & (6.47)          & (1.743)          & (2.452)           & (-2.303)              & (-0.112)               & (-0.489)                & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxm  & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVTJ\_m     & 0.326             & 2.86            & 1.997            & 1.464             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSJ\_idxv  & Intercept         & RV\_day         & RV\_week         & RV\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
RVSJ\_v     & 0.382             & 0.431           & 0.065            & 0.521             & -1.071                & -0.647                 & -3.063                  & 0.8                   & 1.126                  & -4.111                  \\
RVSJ\_idxt  & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
RVSJ\_t     & (2.464)           & (3.785)         & (0.765)          & (3.224)           & (-1.958)              & (-0.572)               & (-2.095)                & (0.515)               & (0.683)                & (-1.803)                \\
RVSJ\_idxm  & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSJ\_m     & 0.339             & 2.802           & 2.078            & 1.414             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSTJ\_idxv & Intercept         & RV\_day         & RV\_week         & RV\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
RVSTJ\_v    & 0.305             & 0.495           & 0.089            & 0.363             & -1.357                & -0.925                 & -1.547                  & -0.086                & 0.798                  & -0.303                  \\
RVSTJ\_idxt & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
RVSTJ\_t    & (1.994)           & (5.193)         & (1.134)          & (3.141)           & (-3.593)              & (-1.063)               & (-1.21)                 & (-0.138)              & (1.085)                & (-0.198)                \\
RVSTJ\_idxm & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSTJ\_m    & 0.338             & 2.806           & 1.992            & 1.43              & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\

% Conditional on Jumps

{}               & HAR       & HAR\_RVJs & HAR\_RVTJs & HAR\_Exp\_RV\_Js & HAR\_Exp\_RV\_TJs & HAR\_CJPs & HAR\_CJNs & HAR\_RVJPs & HAR\_RVJNs & HAR\_RVTJPs & HAR\_RVTJNs \\
\midrule
alpha            & -0.004    & 0.242     & 0.316      & 0.242            & 0.316             & 0.27      & 0.306     & 0.261      & 0.304      & 0.385       & 0.199 \\
alpha\_tvalue    & (-0.045)  & (2.177)   & (1.557)    & (2.177)          & (1.557)           & (2.049)   & (1.605)   & (2.012)    & (1.616)    & (4.586)     & (1.175) \\
beta\_D          & 0.929     & 1.697     & 0.465      & 1.697            & 0.465             & 0.187     & 0.376     & 0.197      & 0.406      & 0.233       & 0.33 \\
beta\_D\_tvalue  & (2.745)   & (2.555)   & (3.838)    & (2.555)          & (3.838)           & (0.272)   & (1.639)   & (0.271)    & (1.722)    & (4.951)     & (3.323) \\
beta\_W          & 0.376     & 0.324     & 0.361      & 0.324            & 0.361             & 1.508     & 0.519     & -0.648     & 0.479      & 0.309       & 0.013 \\
beta\_W\_tvalue  & (3.447)   & (2.895)   & (3.067)    & (2.895)          & (3.067)           & (1.583)   & (2.285)   & (-1.12)    & (2.236)    & (3.438)     & (0.149) \\
beta\_M          & -0.139    & -0.095    & -0.021     & -0.095           & -0.021            & -0.655    & -0.11     & 1.503      & -0.093     & 0.258       & 0.566 \\
beta\_M\_tvalue  & (-0.721)  & (-0.445)  & (-0.286)   & (-0.445)         & (-0.286)          & (-1.12)   & (-0.869)  & (1.554)    & (-0.762)   & (1.99)      & (3.103) \\
beta\_JD         & NaN       & -3.067    & -0.418     & -1.37            & 0.047             & 0.796     & -0.189    & 1.226      & 0.157      & 0.194       & 1.667 \\
beta\_JD\_tvalue & NaN       & (-2.077)  & (-0.95)    & (-1.611)         & (0.142)           & (0.563)   & (-0.376)  & (1.025)    & (0.399)    & (0.626)     & (1.08) \\
beta\_JW         & NaN       & -3.782    & -1.046     & -3.458           & -0.686            & -3.725    & -1.016    & -2.912     & -0.623     & -2.371      & 1.26 \\
beta\_JW\_tvalue & NaN       & (-2.173)  & (-2.859)   & (-1.972)         & (-1.954)          & (-2.551)  & (-2.464)  & (-2.156)   & (-1.609)   & (-2.465)    & (0.7) \\
beta\_JM         & NaN       & -1.486    & -0.527     & -1.581           & -0.548            & -2.676    & -0.654    & -2.765     & -0.613     & -2.106      & -4.148 \\
beta\_JM\_tvalue & NaN       & (-1.181)  & (-0.355)   & (-1.309)         & (-0.378)          & (-1.939)  & (-0.563)  & (-1.879)   & (-0.518)   & (-1.333)    & (-1.651) \\


% BTC-D, Square-root, 1-day horizon,
% All jumps

% Conditional on Jumps


% BTC-D, Log, 1-day horizon,
% All jumps

{}               & HAR      & HAR\_RVJs & HAR\_RVTJs & HAR\_Exp\_RV\_Js & HAR\_Exp\_RV\_TJs & HAR\_CJPs & HAR\_CJNs & HAR\_RVJPs & HAR\_RVJNs & HAR\_RVTJPs & HAR\_RVTJNs \\
\midrule
alpha            & -0.122   & -0.053    & -0.006     & -0.044           & -0.01             & -0.14     & -0.098    & -0.249     & -0.085     & -0.004      & 0.035       \\
alpha\_tvalue    & (-4.341) & (-1.335)  & (-0.147)   & (-1.109)         & (-0.224)          & (-3.231)  & (-2.09)   & (-2.96)    & (-1.932)   & (-0.07)     & (0.38)      \\
beta\_D          & 0.568    & 0.57      & 0.6        & 0.542            & 0.555             & 0.713     & 0.733     & 0.751      & 0.696      & 0.551       & 0.532       \\
beta\_D\_tvalue  & (15.758) & (15.879)  & (17.108)   & (14.952)         & (16.089)          & (8.931)   & (9.377)   & (19.362)   & (9.492)    & (14.908)    & (12.839)    \\
beta\_W          & 0.236    & 0.227     & 0.225      & 0.216            & 0.198             & -0.158    & -0.117    & 0.242      & -0.121     & 0.258       & 0.237       \\
beta\_W\_tvalue  & (5.387)  & (5.002)   & (4.745)    & (5.069)          & (4.769)           & (-1.035)  & (-0.791)  & (4.277)    & (-0.968)   & (5.378)     & (4.454)     \\
beta\_M          & 0.132    & 0.116     & 0.096      & 0.109            & 0.08              & 0.392     & 0.335     & -0.132     & 0.28       & 0.094       & 0.153       \\
beta\_M\_tvalue  & (2.797)  & (2.434)   & (2.164)    & (2.368)          & (2.026)           & (3.266)   & (3.013)   & (-3.387)   & (3.054)    & (1.906)     & (2.518)     \\
beta\_JD         & NaN      & -0.426    & -0.574     & 0.358            & 0.046             & -0.231    & -0.486    & 0.337      & 0.084      & -0.311      & 0.261       \\
beta\_JD\_tvalue & NaN      & (-1.094)  & (-3.053)   & (0.973)          & (0.258)           & (-0.598)  & (-2.711)  & (0.895)    & (0.475)    & (-1.423)    & (0.817)     \\
beta\_JW         & NaN      & -0.595    & -0.534     & -0.385           & -0.186            & -0.584    & -0.525    & -0.271     & -0.141     & -1.142      & -0.463      \\
beta\_JW\_tvalue & NaN      & (-1.151)  & (-1.932)   & (-0.79)          & (-0.783)          & (-1.124)  & (-1.816)  & (-0.54)    & (-0.587)   & (-2.577)    & (-0.723)    \\
beta\_JM         & NaN      & -1.5      & -0.489     & -1.165           & 0.044             & -1.246    & -0.325    & -0.853     & 0.211      & 0.339       & -1.364      \\
beta\_JM\_tvalue & NaN      & (-1.789)  & (-1.35)    & (-1.459)         & (0.114)           & (-1.464)  & (-0.888)  & (-1.069)   & (0.55)     & (0.521)     & (-1.361)    \\

{}          & 0                 & 1                    & 2                     & 3                      & 4                     & 5                      & 6                       & 7                     & 8                      & 9                       \\
\midrule
HAR\_idxv   & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_v      & -0.122            & 0.568                & 0.236                 & 0.132                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_idxt   & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_t      & (-4.341)          & (15.758)             & (5.387)               & (2.797)                & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_idxm   & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_m      & 0.333             & 2.95                 & 0.736                 & 0.614                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVJ\_idxv   & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & Jump\_day             & Jump\_week             & Jump\_month             & NaN                   & NaN                    & NaN                     \\
RVJ\_v      & -0.053            & 0.57                 & 0.227                 & 0.116                  & -0.426                & -0.595                 & -1.5                    & NaN                   & NaN                    & NaN                     \\
RVJ\_idxt   & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & Jump\_day\_tvalue     & Jump\_week\_tvalue     & Jump\_month\_tvalue     & NaN                   & NaN                    & NaN                     \\
RVJ\_t      & (-1.335)          & (15.879)             & (5.002)               & (2.434)                & (-1.094)              & (-1.151)               & (-1.789)                & NaN                   & NaN                    & NaN                     \\
RVJ\_idxm   & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVJ\_m      & 0.333             & 2.936                & 0.74                  & 0.613                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxv  & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & TJump\_day            & TJump\_week            & TJump\_month            & NaN                   & NaN                    & NaN                     \\
RVTJ\_v     & -0.006            & 0.6                  & 0.225                 & 0.096                  & -0.574                & -0.534                 & -0.489                  & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxt  & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & TJump\_day\_tvalue    & TJump\_week\_tvalue    & TJump\_month\_tvalue    & NaN                   & NaN                    & NaN                     \\
RVTJ\_t     & (-0.147)          & (17.108)             & (4.745)               & (2.164)                & (-3.053)              & (-1.932)               & (-1.35)                 & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxm  & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVTJ\_m     & 0.33              & 2.934                & 0.722                 & 0.609                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSJ\_idxv  & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
RVSJ\_v     & 0.115             & 0.581                & 0.315                 & 0.133                  & -0.514                & -1.308                 & 0.299                   & -0.134                & -0.91                  & -0.943                  \\
RVSJ\_idxt  & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
RVSJ\_t     & (1.171)           & (13.658)             & (4.817)               & (1.792)                & (-2.139)              & (-2.503)               & (0.448)                 & (-0.418)              & (-1.301)               & (-0.855)                \\
RVSJ\_idxm  & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSJ\_m     & 0.361             & 2.896                & 0.722                 & 0.609                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSTJ\_idxv & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
RVSTJ\_v    & 0.097             & 0.605                & 0.301                 & 0.103                  & -0.602                & -1.245                 & 0.312                   & -0.223                & -0.334                 & -0.455                  \\
RVSTJ\_idxt & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
RVSTJ\_t    & (1.195)           & (13.871)             & (4.841)               & (1.778)                & (-3.211)              & (-3.225)               & (0.555)                 & (-0.98)               & (-0.768)               & (-0.746)                \\
RVSTJ\_idxm & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSTJ\_m    & 0.363             & 2.885                & 0.72                  & 0.608                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\


% Conditional on Jumps

{}               & HAR       & HAR\_RVJs & HAR\_RVTJs & HAR\_Exp\_RV\_Js & HAR\_Exp\_RV\_TJs & HAR\_CJPs & HAR\_CJNs & HAR\_RVJPs & HAR\_RVJNs & HAR\_RVTJPs & HAR\_RVTJNs \\
\midrule
alpha            & -0.23     & 0.33      & -0         & 0.238            & -0.06             & 0.109     & -0.072    & -0.364     & -0.134     & 0.03        & -0.008 \\
alpha\_tvalue    & (-3.409)  & (1.415)   & (-0.0)     & (1.095)          & (-0.412)          & (0.509)   & (-0.488)  & (-1.3)     & (-0.977)   & (0.416)     & (-0.07) \\
beta\_D          & 0.629     & 0.772     & 0.544      & 0.664            & 0.478             & 0.947     & 0.549     & 0.726      & 0.513      & 0.555       & 0.556 \\
beta\_D\_tvalue  & (8.889)   & (6.79)    & (5.235)    & (6.949)          & (5.123)           & (4.319)   & (2.766)   & (7.63)     & (2.88)     & (10.051)    & (11.43) \\
beta\_W          & 0.17      & 0.139     & 0.38       & 0.119            & 0.312             & -0.386    & 0.187     & 0.319      & 0.114      & 0.27        & 0.189 \\
beta\_W\_tvalue  & (1.865)   & (1.36)    & (4.144)    & (1.347)          & (3.944)           & (-1.037)  & (0.628)   & (1.001)    & (0.464)    & (4.451)     & (2.832) \\
beta\_M          & 0.105     & 0.164     & 0.034      & 0.166            & 0.051             & 0.514     & 0.271     & -0.104     & 0.244      & 0.063       & 0.144 \\
beta\_M\_tvalue  & (1.653)   & (2.08)    & (0.431)    & (2.35)           & (0.718)           & (2.116)   & (1.27)    & (-0.256)   & (1.467)    & (1.037)     & (1.873) \\
beta\_JD         & NaN       & -1.522    & -0.275     & -0.398           & 0.218             & -0.715    & -0.244    & 0.472      & 0.26       & -0.327      & 0.096 \\
beta\_JD\_tvalue & NaN       & (-1.456)  & (-0.685)   & (-0.463)         & (0.677)           & (-0.784)  & (-0.724)  & (0.619)    & (0.93)     & (-1.306)    & (0.26) \\
beta\_JW         & NaN       & -0.889    & -1.855     & -0.716           & -0.929            & -1.309    & -1.621    & -0.75      & -0.857     & -1.36       & -0.25 \\
beta\_JW\_tvalue & NaN       & (-1.054)  & (-3.233)   & (-0.843)         & (-1.71)           & (-1.486)  & (-3.079)  & (-0.827)   & (-1.666)   & (-2.722)    & (-0.324) \\
beta\_JM         & NaN       & -3.426    & 0.049      & -2.248           & 0.916             & -2.729    & -0.181    & -0.51      & 0.868      & 0.104       & -0.536 \\
beta\_JM\_tvalue & NaN       & (-2.529)  & (0.062)    & (-1.688)         & (1.151)           & (-1.944)  & (-0.24)   & (-0.342)   & (1.144)    & (0.138)     & (-0.441) \\




% BTC-G, square, 1-day horizon,
% All jumps

{}               & HAR     & HAR\_RVJs & HAR\_RVTJs & HAR\_Exp\_RV\_Js & HAR\_Exp\_RV\_TJs & HAR\_CJPs & HAR\_CJNs & HAR\_RVJPs & HAR\_RVJNs & HAR\_RVTJPs & HAR\_RVTJNs \\
\midrule
alpha            & 0.179   & 0.278     & 0.304      & 0.278            & 0.304             & 0.239     & 0.26      & 0.247      & 0.274      & 0.482       & 0.249       \\
alpha\_tvalue    & (2.321) & (3.596)   & (3.958)    & (3.596)          & (3.958)           & (2.914)   & (3.104)   & (3.116)    & (3.509)    & (4.397)     & (3.371)     \\
beta\_D          & 0.333   & 0.379     & 0.393      & 0.379            & 0.393             & 0.577     & 0.589     & 0.586      & 0.609      & 0.39        & 0.38        \\
beta\_D\_tvalue  & (4.552) & (5.098)   & (4.725)    & (5.098)          & (4.725)           & (4.611)   & (4.477)   & (4.66)     & (4.503)    & (4.901)     & (4.884)     \\
beta\_W          & 0.166   & 0.177     & 0.172      & 0.177            & 0.172             & -0.261    & -0.255    & 0.529      & -0.269     & 0.327       & 0.168       \\
beta\_W\_tvalue  & (2.973) & (2.617)   & (2.401)    & (2.617)          & (2.401)           & (-1.086)  & (-1.017)  & (2.369)    & (-1.065)   & (3.041)     & (2.458)     \\
beta\_M          & 0.322   & 0.271     & 0.258      & 0.271            & 0.258             & 0.538     & 0.513     & -0.264     & 0.505      & 0.371       & 0.292       \\
beta\_M\_tvalue  & (2.614) & (2.226)   & (2.029)    & (2.226)          & (2.029)           & (2.42)    & (2.247)   & (-1.095)   & (2.188)    & (2.229)     & (2.265)     \\
beta\_JD         & NaN     & -0.493    & -0.333     & -0.114           & 0.06              & -0.477    & -0.308    & -0.117     & 0.059      & -0.981      & -0.05       \\
beta\_JD\_tvalue & NaN     & (-2.639)  & (-2.091)   & (-0.796)         & (0.507)           & (-3.194)  & (-2.349)  & (-0.905)   & (0.513)    & (-1.739)    & (-0.236)    \\
beta\_JW         & NaN     & -0.511    & -0.25      & -0.334           & -0.078            & -0.496    & -0.27     & -0.3       & -0.073     & -3.745      & -0.037      \\
beta\_JW\_tvalue & NaN     & (-1.967)  & (-1.654)   & (-1.496)         & (-0.725)          & (-1.74)   & (-1.525)  & (-1.364)   & (-0.663)   & (-2.663)    & (-0.254)    \\
beta\_JM         & NaN     & -0.363    & -0.274     & -0.092           & -0.016            & -0.213    & -0.14     & 0.011      & 0.064      & -2.805      & -0.169      \\
beta\_JM\_tvalue & NaN     & (-0.803)  & (-0.901)   & (-0.212)         & (-0.057)          & (-0.532)  & (-0.534)  & (0.027)    & (0.252)    & (-1.299)    & (-0.44)     \\


{}          & 0                 & 1               & 2                & 3                 & 4                     & 5                      & 6                       & 7                     & 8                      & 9                       \\
\midrule
HAR\_idxv   & Intercept         & RV\_day         & RV\_week         & RV\_month         & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_v      & 0.178             & 0.333           & 0.163            & 0.326             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_idxt   & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_t      & (2.315)           & (4.56)          & (3.016)          & (2.654)           & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_idxm   & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_m      & 0.229             & 2.325           & 3.541            & 1.849             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVJ\_idxv   & Intercept         & RV\_day         & RV\_week         & RV\_month         & Jump\_day             & Jump\_week             & Jump\_month             & NaN                   & NaN                    & NaN                     \\
RVJ\_v      & 0.278             & 0.379           & 0.175            & 0.273             & -0.493                & -0.5                   & -0.372                  & NaN                   & NaN                    & NaN                     \\
RVJ\_idxt   & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & Jump\_day\_tvalue     & Jump\_week\_tvalue     & Jump\_month\_tvalue     & NaN                   & NaN                    & NaN                     \\
RVJ\_t      & (3.591)           & (5.11)          & (2.677)          & (2.251)           & (-2.676)              & (-1.977)               & (-0.824)                & NaN                   & NaN                    & NaN                     \\
RVJ\_idxm   & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVJ\_m      & 0.244             & 2.282           & 3.962            & 1.933             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxv  & Intercept         & RV\_day         & RV\_week         & RV\_month         & TJump\_day            & TJump\_week            & TJump\_month            & NaN                   & NaN                    & NaN                     \\
RVTJ\_v     & 0.302             & 0.393           & 0.171            & 0.259             & -0.333                & -0.241                 & -0.266                  & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxt  & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & TJump\_day\_tvalue    & TJump\_week\_tvalue    & TJump\_month\_tvalue    & NaN                   & NaN                    & NaN                     \\
RVTJ\_t     & (3.94)            & (4.732)         & (2.446)          & (2.045)           & (-2.106)              & (-1.596)               & (-0.877)                & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxm  & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVTJ\_m     & 0.241             & 2.289           & 4.154            & 1.995             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSJ\_idxv  & Intercept         & RV\_day         & RV\_week         & RV\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
RVSJ\_v     & 0.513             & 0.424           & 0.343            & 0.414             & -1.347                & -3.877                 & -3.297                  & -0.502                & -0.434                 & -0.605                  \\
RVSJ\_idxt  & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
RVSJ\_t     & (4.279)           & (4.243)         & (2.858)          & (2.21)            & (-2.356)              & (-2.565)               & (-1.467)                & (-1.769)              & (-1.771)               & (-1.3)                  \\
RVSJ\_idxm  & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSJ\_m     & 0.261             & 2.23            & 5.284            & 2.223             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSTJ\_idxv & Intercept         & RV\_day         & RV\_week         & RV\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
RVSTJ\_v    & 0.519             & 0.437           & 0.304            & 0.348             & -1.211                & -2.857                 & -2.372                  & -0.219                & 0.173                  & -0.194                  \\
RVSTJ\_idxt & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
RVSTJ\_t    & (5.051)           & (4.347)         & (2.745)          & (2.199)           & (-2.857)              & (-2.593)               & (-1.631)                & (-0.941)              & (1.022)                & (-0.526)                \\
RVSTJ\_idxm & M-Z-R2            & MSE             & HRMSE            & QLIKE             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSTJ\_m    & 0.262             & 2.226           & 5.419            & 2.248             & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\


% Conditional on jumps

{}               & HAR       & HAR\_RVJs & HAR\_RVTJs & HAR\_Exp\_RV\_Js & HAR\_Exp\_RV\_TJs & HAR\_CJPs & HAR\_CJNs & HAR\_RVJPs & HAR\_RVJNs & HAR\_RVTJPs & HAR\_RVTJNs \\
\midrule
alpha            & 0.227     & 0.215     & 0.289      & 0.215            & 0.289             & 0.251     & 0.276     & 0.253      & 0.277      & 0.515       & 0.184 \\
alpha\_tvalue    & (1.832)   & (2.205)   & (3.978)    & (2.205)          & (3.978)           & (2.159)   & (3.052)   & (2.335)    & (3.522)    & (4.351)     & (2.267) \\
beta\_D          & 0.211     & 1.073     & 0.818      & 1.073            & 0.818             & 0.866     & 0.917     & 1.084      & 1.109      & 0.313       & 0.727 \\
beta\_D\_tvalue  & (1.399)   & (5.92)    & (7.081)    & (5.92)           & (7.081)           & (2.954)   & (5.061)   & (4.826)    & (5.719)    & (2.928)     & (6.903) \\
beta\_W          & 0.257     & 0.189     & 0.197      & 0.189            & 0.197             & -0.154    & -0.228    & 0.164      & -0.397     & 0.274       & 0.087 \\
beta\_W\_tvalue  & (2.959)   & (2.319)   & (2.366)    & (2.319)          & (2.366)           & (-0.499)  & (-0.887)  & (0.839)    & (-1.635)   & (2.425)     & (1.355) \\
beta\_M          & 0.107     & 0.002     & -0.041     & 0.002            & -0.041            & 0.181     & 0.171     & -0.291     & 0.188      & 0.413       & 0.271 \\
beta\_M\_tvalue  & (1.327)   & (0.02)    & (-0.49)    & (0.02)           & (-0.49)           & (0.923)   & (0.891)   & (-1.13)    & (1.007)    & (2.179)     & (2.114) \\
beta\_JD         & NaN       & -1.775    & -0.944     & -0.702           & -0.126            & -0.836    & -0.596    & -0.38      & -0.064     & -0.344      & -0.487 \\
beta\_JD\_tvalue & NaN       & (-5.729)  & (-6.27)    & (-5.408)         & (-2.48)           & (-4.204)  & (-5.767)  & (-4.131)   & (-0.874)   & (-0.525)    & (-4.263) \\
beta\_JW         & NaN       & -0.365    & -0.368     & -0.176           & -0.171            & -0.5      & -0.326    & -0.183     & -0.069     & -3.507      & -0.078 \\
beta\_JW\_tvalue & NaN       & (-2.41)   & (-2.158)   & (-2.083)         & (-1.464)          & (-1.81)   & (-1.564)  & (-1.235)   & (-0.679)   & (-2.096)    & (-0.588) \\
beta\_JM         & NaN       & 0.081     & 0.098      & 0.083            & 0.058             & -0.064    & 0.001     & 0.014      & 0.043      & -3.666      & -0.187 \\
beta\_JM\_tvalue & NaN       & (0.244)   & (0.385)    & (0.266)          & (0.272)           & (-0.212)  & (0.007)   & (0.048)    & (0.226)    & (-1.571)    & (-0.605) \\



% BTC-G, square-root, 1-day horizon,
% All jumps

% Conditional on Jumps


% BTC-G, Log, 1-day horizon,

% All jumps

{}               & HAR      & HAR\_RVJs & HAR\_RVTJs & HAR\_Exp\_RV\_Js & HAR\_Exp\_RV\_TJs & HAR\_CJPs & HAR\_CJNs & HAR\_RVJPs & HAR\_RVJNs & HAR\_RVTJPs & HAR\_RVTJNs \\
\midrule
alpha            & -0.183   & -0.051    & 0.002      & -0.038           & 0.019             & -0.116    & -0.062    & -0.394     & -0.05      & 0.102       & -0.035      \\
alpha\_tvalue    & (-5.188) & (-1.023)  & (0.043)    & (-0.737)         & (0.324)           & (-2.289)  & (-1.038)  & (-3.987)   & (-0.828)   & (0.947)     & (-0.502)    \\
beta\_D          & 0.533    & 0.527     & 0.55       & 0.474            & 0.476             & 0.556     & 0.566     & 0.691      & 0.593      & 0.481       & 0.473       \\
beta\_D\_tvalue  & (16.759) & (16.422)  & (16.335)   & (16.081)         & (15.954)          & (7.285)   & (7.011)   & (16.874)   & (7.68)     & (16.016)    & (14.1)      \\
beta\_W          & 0.262    & 0.302     & 0.313      & 0.267            & 0.232             & 0.163     & 0.228     & 0.353      & -0.032     & 0.291       & 0.269       \\
beta\_W\_tvalue  & (6.727)  & (7.308)   & (6.99)     & (6.828)          & (5.766)           & (1.08)    & (1.399)   & (4.616)    & (-0.209)   & (6.471)     & (6.294)     \\
beta\_M          & 0.126    & 0.104     & 0.068      & 0.118            & 0.084             & 0.254     & 0.169     & -0.152     & 0.264      & 0.144       & 0.13        \\
beta\_M\_tvalue  & (2.822)  & (2.391)   & (1.471)    & (2.949)          & (2.205)           & (2.069)   & (1.288)   & (-2.834)   & (2.321)    & (2.617)     & (3.055)     \\
beta\_JD         & NaN      & -0.43     & -0.419     & 0.051            & 0.162             & -0.534    & -0.432    & -0.067     & 0.148      & -0.189      & 0.12        \\
beta\_JD\_tvalue & NaN      & (-2.022)  & (-2.42)    & (0.219)          & (1.037)           & (-2.546)  & (-2.553)  & (-0.298)   & (0.97)     & (-0.693)    & (0.414)     \\
beta\_JW         & NaN      & -0.903    & -0.685     & -0.537           & -0.199            & -1.153    & -0.846    & -0.35      & -0.156     & -1.511      & -0.377      \\
beta\_JW\_tvalue & NaN      & (-3.05)   & (-3.383)   & (-2.083)         & (-1.155)          & (-3.452)  & (-3.431)  & (-1.249)   & (-0.794)   & (-3.296)    & (-1.461)    \\
beta\_JM         & NaN      & -0.484    & -0.247     & -0.147           & -0.05             & -0.529    & -0.286    & 0.215      & -0.048     & -0.698      & -0.218      \\
beta\_JM\_tvalue & NaN      & (-1.353)  & (-0.891)   & (-0.408)         & (-0.181)          & (-1.566)  & (-1.12)   & (0.635)    & (-0.185)   & (-0.655)    & (-0.551)    \\



{}          & 0                 & 1                    & 2                     & 3                      & 4                     & 5                      & 6                       & 7                     & 8                      & 9                       \\
\midrule
HAR\_idxv   & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_v      & -0.182            & 0.532                & 0.262                 & 0.127                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_idxt   & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_t      & (-5.267)          & (16.773)             & (6.793)               & (2.856)                & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_idxm   & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
HAR\_m      & 0.255             & 2.356                & 1.089                 & 0.427                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVJ\_idxv   & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & Jump\_day             & Jump\_week             & Jump\_month             & NaN                   & NaN                    & NaN                     \\
RVJ\_v      & -0.048            & 0.528                & 0.301                 & 0.107                  & -0.436                & -0.863                 & -0.51                   & NaN                   & NaN                    & NaN                     \\
RVJ\_idxt   & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & Jump\_day\_tvalue     & Jump\_week\_tvalue     & Jump\_month\_tvalue     & NaN                   & NaN                    & NaN                     \\
RVJ\_t      & (-0.981)          & (16.499)             & (7.329)               & (2.462)                & (-2.17)               & (-3.112)               & (-1.425)                & NaN                   & NaN                    & NaN                     \\
RVJ\_idxm   & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVJ\_m      & 0.257             & 2.329                & 1.057                 & 0.416                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxv  & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & TJump\_day            & TJump\_week            & TJump\_month            & NaN                   & NaN                    & NaN                     \\
RVTJ\_v     & -0.002            & 0.55                 & 0.313                 & 0.071                  & -0.412                & -0.643                 & -0.232                  & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxt  & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & TJump\_day\_tvalue    & TJump\_week\_tvalue    & TJump\_month\_tvalue    & NaN                   & NaN                    & NaN                     \\
RVTJ\_t     & (-0.032)          & (16.423)             & (7.01)                & (1.525)                & (-2.452)              & (-3.275)               & (-0.835)                & NaN                   & NaN                    & NaN                     \\
RVTJ\_idxm  & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVTJ\_m     & 0.248             & 2.347                & 1.048                 & 0.415                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSJ\_idxv  & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
RVSJ\_v     & 0.254             & 0.543                & 0.376                 & 0.158                  & -0.584                & -1.875                 & -0.954                  & -0.252                & -0.805                 & -0.673                  \\
RVSJ\_idxt  & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
RVSJ\_t     & (1.828)           & (13.176)             & (6.949)               & (2.351)                & (-1.828)              & (-3.856)               & (-0.896)                & (-0.872)              & (-2.862)               & (-1.553)                \\
RVSJ\_idxm  & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSJ\_m     & 0.29              & 2.292                & 1.071                 & 0.418                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSTJ\_idxv & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
RVSTJ\_v    & 0.226             & 0.555                & 0.373                 & 0.113                  & -0.658                & -1.64                  & -0.52                   & -0.141                & -0.349                 & -0.445                  \\
RVSTJ\_idxt & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
RVSTJ\_t    & (1.968)           & (13.653)             & (6.69)                & (1.873)                & (-2.615)              & (-3.839)               & (-0.661)                & (-0.673)              & (-1.473)               & (-1.303)                \\
RVSTJ\_idxm & M-Z-R2            & MSE                  & HRMSE                 & QLIKE                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\
RVSTJ\_m    & 0.296             & 2.272                & 1.073                 & 0.417                  & NaN                   & NaN                    & NaN                     & NaN                   & NaN                    & NaN                     \\


% Condition on Jump

{}               & HAR       & HAR\_RVJs & HAR\_RVTJs & HAR\_Exp\_RV\_Js & HAR\_Exp\_RV\_TJs & HAR\_CJPs & HAR\_CJNs & HAR\_RVJPs & HAR\_RVJNs & HAR\_RVTJPs & HAR\_RVTJNs \\
\midrule
alpha            & -0.281    & -0.075    & 0.014      & -0.024           & 0.013             & -0.115    & -0.011    & -0.48      & -0.059     & 0.045       & 0.016 \\
alpha\_tvalue    & (-4.409)  & (-0.607)  & (0.129)    & (-0.182)         & (0.121)           & (-0.91)   & (-0.089)  & (-2.628)   & (-0.53)    & (0.373)     & (0.203) \\
beta\_D          & 0.496     & 0.501     & 0.513      & 0.448            & 0.453             & 0.471     & 0.464     & 0.669      & 0.537      & 0.495       & 0.48 \\
beta\_D\_tvalue  & (10.068)  & (7.734)   & (8.604)    & (8.078)          & (9.656)           & (3.595)   & (3.847)   & (11.097)   & (4.896)    & (12.716)    & (12.677) \\
beta\_W          & 0.271     & 0.333     & 0.386      & 0.286            & 0.262             & 0.31      & 0.423     & 0.526      & 0.057      & 0.245       & 0.262 \\
beta\_W\_tvalue  & (4.686)   & (4.987)   & (6.526)    & (4.676)          & (4.859)           & (1.322)   & (2.0)     & (3.022)    & (0.285)    & (4.672)     & (5.806) \\
beta\_M          & 0.146     & 0.131     & 0.059      & 0.134            & 0.065             & 0.24      & 0.12      & -0.193     & 0.22       & 0.117       & 0.14 \\
beta\_M\_tvalue  & (2.427)   & (2.14)    & (1.112)    & (2.45)           & (1.553)           & (1.332)   & (0.75)    & (-1.7)     & (1.591)    & (1.91)      & (2.99) \\
beta\_JD         & NaN       & -0.286    & -0.295     & 0.041            & 0.181             & -0.428    & -0.368    & -0.094     & 0.191      & -0.181      & -0.024 \\
beta\_JD\_tvalue & NaN       & (-0.776)  & (-1.053)   & (0.111)          & (0.779)           & (-1.172)  & (-1.368)  & (-0.283)   & (0.842)    & (-0.646)    & (-0.084) \\
beta\_JW         & NaN       & -1.003    & -1.011     & -0.62            & -0.363            & -1.57     & -1.271    & -0.5       & -0.318     & -1.286      & -0.34 \\
beta\_JW\_tvalue & NaN       & (-3.317)  & (-4.37)    & (-2.538)         & (-1.976)          & (-5.023)  & (-4.965)  & (-1.684)   & (-1.422)   & (-2.286)    & (-1.181) \\
beta\_JM         & NaN       & -0.404    & -0.166     & -0.08            & 0.041             & -0.423    & -0.28     & 0.236      & -0.006     & -0.449      & -0.274 \\
beta\_JM\_tvalue & NaN       & (-0.746)  & (-0.507)   & (-0.148)         & (0.128)           & (-0.858)  & (-0.911)  & (0.486)    & (-0.019)   & (-0.383)    & (-0.679) \\


==> rsv_results.tex <==
\\BTC-D, Square form, 1-day
\\insample

\midrule
HAR\_RVSJ\_idxv  & Intercept         & RV\_day         & RV\_week         & RV\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
HAR\_RVSJ\_idxt  & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
HAR\_RVSTJ\_idxv & Intercept         & RV\_day         & RV\_week         & RV\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
HAR\_RVSTJ\_idxt & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
HAR\_RVSJ\_v     & 0.382             & 0.431           & 0.065            & 0.521             & -1.071                & -0.647                 & -3.063                  & 0.8                   & 1.126                  & -4.111                  \\
HAR\_RVSJ\_t     & (2.464)           & (3.785)         & (0.765)          & (3.224)           & (-1.958)              & (-0.572)               & (-2.095)                & (0.515)               & (0.683)                & (-1.803)                \\
HAR\_RVSTJ\_v    & 0.305             & 0.495           & 0.089            & 0.363             & -1.357                & -0.925                 & -1.547                  & -0.086                & 0.798                  & -0.303                  \\
HAR\_RVSTJ\_t    & (1.994)           & (5.193)         & (1.134)          & (3.141)           & (-3.593)              & (-1.063)               & (-1.21)                 & (-0.138)              & (1.085)                & (-0.198)                \\


\\out sample

\midrule
HAR\_RVSJ\_idxm  & M-Z-R2 & MSE   & HRMSE & QLIKE & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSTJ\_idxm & M-Z-R2 & MSE   & HRMSE & QLIKE & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSJ\_m     & 0.221  & 3.445 & 1.891 & 1.362 & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSTJ\_m    & 0.216  & 3.511 & 1.677 & 1.339 & NaN & NaN & NaN & NaN & NaN & NaN \\


\\BTC-D, log form, 1-day
\\insample

\midrule
HAR\_RVSJ\_idxv  & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
HAR\_RVSJ\_idxt  & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
HAR\_RVSTJ\_idxv & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
HAR\_RVSTJ\_idxt & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
HAR\_RVSJ\_v     & 0.115             & 0.581                & 0.315                 & 0.133                  & -0.514                & -1.308                 & 0.299                   & -0.134                & -0.91                  & -0.943                  \\
HAR\_RVSJ\_t     & (1.171)           & (13.658)             & (4.817)               & (1.792)                & (-2.139)              & (-2.503)               & (0.448)                 & (-0.418)              & (-1.301)               & (-0.855)                \\
HAR\_RVSTJ\_v    & 0.097             & 0.605                & 0.301                 & 0.103                  & -0.602                & -1.245                 & 0.312                   & -0.223                & -0.334                 & -0.455                  \\
HAR\_RVSTJ\_t    & (1.195)           & (13.871)             & (4.841)               & (1.778)                & (-3.211)              & (-3.225)               & (0.555)                 & (-0.98)               & (-0.768)               & (-0.746)                \\

\\out sample

HAR\_RVSJ\_idxm  & M-Z-R2 & MSE   & HRMSE & QLIKE & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSTJ\_idxm & M-Z-R2 & MSE   & HRMSE & QLIKE & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSJ\_m     & 0.238  & 3.308 & 0.728 & 0.647 & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSTJ\_m    & 0.243  & 3.289 & 0.716 & 0.641 & NaN & NaN & NaN & NaN & NaN & NaN \\



\\BTC-G, Square form, 1-day
\\in sample


\midrule
HAR\_RVSJ\_idxv  & Intercept         & RV\_day         & RV\_week         & RV\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
HAR\_RVSJ\_idxt  & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
HAR\_RVSTJ\_idxv & Intercept         & RV\_day         & RV\_week         & RV\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
HAR\_RVSTJ\_idxt & Intercept\_tvalue & RV\_day\_tvalue & RV\_week\_tvalue & RV\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
HAR\_RVSJ\_v     & 0.512             & 0.423           & 0.352            & 0.404             & -1.357                & -4.023                 & -3.105                  & -0.5                  & -0.461                 & -0.607                  \\
HAR\_RVSJ\_t     & (4.279)           & (4.2)           & (2.824)          & (2.147)           & (-2.309)              & (-2.591)               & (-1.363)                & (-1.737)              & (-1.869)               & (-1.313)                \\
HAR\_RVSTJ\_v    & 0.522             & 0.437           & 0.31             & 0.342             & -1.221                & -2.932                 & -2.295                  & -0.216                & 0.168                  & -0.224                  \\
HAR\_RVSTJ\_t    & (5.089)           & (4.323)         & (2.73)           & (2.16)            & (-2.831)              & (-2.619)               & (-1.566)                & (-0.923)              & (1.0)                  & (-0.608)                \\


\\ out sample

\midrule

HAR\_RVSJ\_idxm  & M-Z-R2 & MSE   & HRMSE & QLIKE & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSTJ\_idxm & M-Z-R2 & MSE   & HRMSE & QLIKE & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSJ\_m     & 0.238  & 2.196 & 5.744 & 2.371 & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSTJ\_m    & 0.255  & 2.137 & 5.549 & 2.351 & NaN & NaN & NaN & NaN & NaN & NaN \\




log form, 1-day
\\ in sample
\midrule
HAR\_RVSJ\_idxv  & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & Jump\_p\_day          & Jump\_p\_week          & Jump\_p\_month          & Jump\_n\_day          & Jump\_n\_week          & Jump\_n\_month          \\
HAR\_RVSJ\_idxt  & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & Jump\_p\_day\_tvalue  & Jump\_p\_week\_tvalue  & Jump\_p\_month\_tvalue  & Jump\_n\_day\_tvalue  & Jump\_n\_week\_tvalue  & Jump\_n\_month\_tvalue  \\
HAR\_RVSTJ\_idxv & Intercept         & Log\_RV\_day         & Log\_RV\_week         & Log\_RV\_month         & TJump\_p\_day         & TJump\_p\_week         & TJump\_p\_month         & TJump\_n\_day         & TJump\_n\_week         & TJump\_n\_month         \\
HAR\_RVSTJ\_idxt & Intercept\_tvalue & Log\_RV\_day\_tvalue & Log\_RV\_week\_tvalue & Log\_RV\_month\_tvalue & TJump\_p\_day\_tvalue & TJump\_p\_week\_tvalue & TJump\_p\_month\_tvalue & TJump\_n\_day\_tvalue & TJump\_n\_week\_tvalue & TJump\_n\_month\_tvalue \\
HAR\_RVSJ\_v     & 0.247             & 0.542                & 0.382                 & 0.148                  & -0.601                & -1.988                 & -0.732                  & -0.247                & -0.863                 & -0.662                  \\
HAR\_RVSJ\_t     & (1.786)           & (12.9)               & (6.993)               & (2.203)                & (-1.793)              & (-4.026)               & (-0.686)                & (-0.81)               & (-2.948)               & (-1.526)                \\
HAR\_RVSTJ\_v    & 0.23              & 0.554                & 0.378                 & 0.109                  & -0.677                & -1.698                 & -0.43                   & -0.135                & -0.392                 & -0.487                  \\
HAR\_RVSTJ\_t    & (1.994)           & (13.516)             & (6.716)               & (1.799)                & (-2.624)              & (-3.939)               & (-0.544)                & (-0.624)              & (-1.568)               & (-1.425)                \\

\\out sample

HAR\_RVSJ\_idxm  & M-Z-R2 & MSE   & HRMSE & QLIKE & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSTJ\_idxm & M-Z-R2 & MSE   & HRMSE & QLIKE & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSJ\_m     & 0.258  & 2.263 & 1.037 & 0.41  & NaN & NaN & NaN & NaN & NaN & NaN \\
HAR\_RVSTJ\_m    & 0.281  & 2.216 & 1.032 & 0.41  & NaN & NaN & NaN & NaN & NaN & NaN \\


==> sections/subsections/AdaptiveForecast.tex <==
% !TEX root = ../../RCVJ.tex

\subsection{Out-of-Sample Forecasts Evaluation}

In this subsection, we further discuss the out-of-sample forecasting results aiming for comparing different models.
All the out-of-sample forecasts are computed using 90-days rolling-window HAR regressions as described in the previous sections.
Parameters are re-estimated on a daily basis.
Here the "insanity filter" is applied in which we ensure that any forecast is no smaller (larger) than the minimum (maximum) realization of the past (\cite{patton2015good}, \cite{swanson1997forecasting} and \cite{bollerslev2018risk}).

\subsubsection{Forecasting Accuracy}

The out-of-sample performance evaluations are based on the squared form, i.e results from the log-log forecasting models are transformed back to squared form for a fair comparison
\footnote{The squared form of HAR models are also common in previous literature, and usually underperforms the logarithmic form. We also report the squared form forecasting accuracy in  Appendix \ref{tab:OutSampleForecasts_squareform}, the conclusions are consistent with logarithmic form}.
We employ four metrics for the forecasting performance comparison.
The first one is $R^2$ from Mincer-Zarnowitz forecasting regression, named MZ-$R^2$.
The following three metrics named MSE, HRMSE, and QLIKE are computed from corresponding loss functions,

\begin{align}
  \operatorname{L^{MSE}}&=\left(RV_{t,t+h}-\widehat{RV}_{t,t+h}\right)^2\\
  \operatorname{L^{HRMSE}}&=\left(\frac{RV_{t,t+h}-\widehat{RV}_{t,t+h}}{RV_{t,t+h}}\right)^2\\
  \operatorname{L^{QLIKE}}&=\log\widehat{RV}_{t,t+h}+\frac{{RV_{t,t+h}}}{\widehat{RV}_{t,t+h}},
\end{align}

where $\widehat{RV}_{t,t+h}$ is the forecast average realized variance over time period $[t,t+h]$, and $RV_{t,t+h}$ is the corresponding true value.
And then the D-M test (\cite{diebold2002comparing}) is used to test the significance of comparison results by embedding the three loss functions.
The mean squared error (MSE) is the mean value of quadratic loss function $\operatorname{L^{MSE}}$ which measures the Euclidean distance between the ex-post realized variance and forecast result.
The heteroscedasticity adjusted root mean squared error (HRMSE) defined as the squared root mean of $\operatorname{L^{HRMSE}}$ (\cite{bollerslev1996periodic}) is a more robust metric to the scale changing of realized variance.
The third metric QLIKE is the mean of a gaussian quasi-likelihood loss function $L^{QLIKE}$ (\cite{patton2011volatility}) which gives consistent evaluation on different imperfect volatility proxies.

\input{tabs/Tab_OutOfSampleForecasts_logform.tex}

The out-of-sample forecasting evaluation reported in Tab.\ref{tab:OutSampleForecasts_logform} shows clearly that the forecasting performance depends on the forecasting horizon.
This conclusion has a twofold meaning.
First of all, it is obvious that each of the models performs better in the long forecasting horizon under most of the metrics, such as the MZ-$R^2$ is higher and MSE is much lower in $h=30$.
Secondly, it partially reveals the necessity of modeling jumps or decomposition into signed estimators.
In the short forecasting horizon, $h=1$, those models that do not put jump components as explanatory variables separately, HAR and RSV models, tend to outperform any other models.
For example, MZ-$R^2$ is 0.299 in HAR while it is 0.241 in RSVSJ which accounts for the decomposed estimators $SRV$ and $J^{+/-}$.
As shown in the first panel of Tab.\ref{tab:OutSampleForecasts_logform}, the D-M test shows the better accuracy of HAR at 5\% significant level.
However, in the long forecasting horizon case, $h=30$, modeling the jumps and signed estimators does improve the forecasting performance.
As shown in the last panel of Tab.\ref{tab:OutSampleForecasts_logform}, the models accounting jumps or signed estimators including RVJ, RSV, and RSVSJ, outperform HAR model by all the metrics.
And the significance is confirmed by the D-M test at the 5\% significant level.
Contrary to \cite{andersen2007roughing}, we find evidence that modeling separated jumps or signed estimators do not necessarily improve the BTC $RV$ forecasting accuracy and forecasting horizon matters.
However, the theoretical explanation of that is not answered as far as we know.


==> sections/subsections/Datasource.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Data Source}\label{sec:data}

There are 254\footnote{Until July 2019, https://coin.market/exchanges-info.php} online exchanges trading various types of cryptocurrencies and each of the coins is traded in different exchanges globally.
Among all crypto markets, the Bitcoin market is dominant with more than 70\% market share.
In this article, we focus only on the Bitcoin market, two price processes constructed from two different data sources are studied.
One process is provided by a private data company DYOS\footnote{Dyos solutions GmbH, Berlin, Germany},
hereafter \textbf{BTC-D}.
And the other one is obtained from an online free provider\footnote{https://www.cryptodatadownload.com/}, hereafter \textbf{BTC-G}.
BTC-D price is equal-weighted prices from three actively trading exchanges, Poloniex, Bittrex, and Bitfinex\footnote{Poloniex and Bittrex are U.S based companies, and Bitfinex located in Hongkong}.
Such construction can be viewed as the price of a portfolio, which allows investors to diversify idiosyncratic risk from exchanges.
% a portfolio-type price that allows investors to avoid idiosyncratic risk from exchanges.
In contrast, BTC-G price comes from only one exchange, Gemini\footnote{https://gemini.com/about/}, which is one of the largest digital exchanges regulated by NYDFS\footnote{New York State Department of Financial Services}.

Although the full dataset can be dated back to 2014, the trading was not active until 2017.
We thus construct our data from January 2017.
In particular, the sample period of BTC-D price is from January 2017 to May 2019, while that of BTC-G price starts from January 2017 to July 2019.
The Bitcoin market is trading all-day and all-year globally akin to the foreign exchange market which prompts the issue of removing the illiquidity periods, such as weekends/holidays, and inactive trading hours.
In this article, we do not remove any trading days because many of the non-institutional investors who can trade during non-business days in the cryptocurrency market.
Moreover, as the trading records come from U.S based and Asia based online exchanges, we define the day as 0:00 GMT to 23:55 GMT and keep the whole 24-hour data samples.
After cleaning and removing the trading days that have an incomplete number of samples, the dataset has an 864-day sample for BTC-D and an 883-day sample for BTC-G.
Note that due to the data missing problem from BTC-G datasource, we remove samples from 15th Nov. 2018 to 6th Dec. 2018.
Both two data sources are sampled every 5-min, thus every day has 288 samples.


==> sections/subsections/DynamicsJump.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Dynamics of Jumps Processes}

Recall that we construct three jump estimators, the corrected thresholded jump $J$, and positive(negative) thresholded jump $J^{+(-)}$ in Section \ref{sec:RV_Decomp_Model}.
We first explain the descriptive statistics of the three jump estimators and then show the detected jump processes.
Only the non-zero detected jumps are reported in Tab.\ref{tab:summary_des_jumps} and estimator $J(\alpha)$ is evaluated at 99.99\% confidence level.

% More jumps in the Cryptocurrency market
Jumps appear far more frequently in the Bitcoin market than in any other developed markets comparing our results with the those documented in pervious researches using similar approaches.
From our empirical results in Tab.\ref{tab:summary_des_jumps}, 39\% and 68\% of days are detected with jumps for BTC-D and BTC-G, respectively.
\cite{corsi2010threshold} show that for the most liquid six stocks of S\&P500, 8.3\% of the 1256 sample days are entangled with jumps by the corrected thresholded jump estimator $J(\alpha=99.9\%)$.
\cite{andersen2007roughing} examine on various financial assets including DM/\$, S\&P 500 and U.S T-Bond, the result shows that up to 8.3\% of all the sample days are detected with jumps in DM/\$ exchange rate market.

% More jumps in BTC-G than in BTC-D
Nevertheless, we find that a simple equal-weighted portfolio, BTC-D, reduces the size and quantity of jumps significantly, i.e the jump risk of BTC can be diversified.
Comparing the two panels in Tab.\ref{tab:summary_des_jumps}, given the same time period and the same jump detection estimator, BTC-D has much fewer sample days contained with price jumps, e.g by $J(\alpha)$ estimator, 39\% of days in BTC-D while 68\% of days in BTC-G are found with jumps.
The price process of BTC-D is constructed by weighting prices from multiple exchanges equally, thus idiosyncratic jumps from one exchange detected by high-frequency data can be canceled out from such construction.
BTC-G is more positive skewed and leptokurtic than BTC-D in terms of all jump estimators which indicates that more extreme jumps appear in BTC-G, for example, $skewness(\text{BTC-D},J)=7.28$ versus $skewness(\text{BTC-G}, J)=14.40$ and $kurtosis(\text{BTC-D}, J)=73.22$ versus $kurtosis(\text{BTC-G}, J)=259.24$.

\begin{table}[!htb]
  \centering % centering table
\begin{threeparttable}
\caption{Summary Statistics For BTC Jump Components}\label{tab:summary_des_jumps}
\footnotesize
\begin{tabular}{l *{3}{S[table-format=3.3,table-number-alignment = center]}l *{3}{S[table-format=3.3,table-number-alignment = center]}}
\toprule\toprule
\multicolumn{1}{r}{}&\multicolumn{3}{c}{\textbf{Panel A: BTC-D}} &\multicolumn{1}{r}{}& \multicolumn{3}{c}{\textbf{Panel B: BTC-G}}\\
% \cline{2-11}\\
% \midrule
\multicolumn{1}{c}{}
& \multicolumn{1}{c}{$J(\alpha)$}
& \multicolumn{1}{c}{$J^+$}
& \multicolumn{1}{c}{$J^-$}
& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{$J(\alpha)$}
& \multicolumn{1}{c}{$J^+$}
& \multicolumn{1}{c}{$J^-$}\\

\cmidrule{2-4}
\cmidrule{6-8}

prop.$^{\dagger}$ & 0.39  & 0.76  & 0.79   & & 0.68   & 0.83  & 0.87   \\
mean              & 0.20  & 0.09  & 0.11   & & 0.24   & 0.11  & 0.15   \\
std               & 0.40  & 0.21  & 0.25   & & 0.76   & 0.23  & 0.56   \\
skewness          & 7.28  & 5.80  & 9.46   & & 14.40  & 6.77  & 17.33  \\
kurtosis          & 73.22 & 43.31 & 131.43 & & 259.24 & 62.06 & 368.50 \\
min(\%)           & 0.92  & 0.02  & 0.03   & & 0.34   & 0.00  & 0.02   \\
50\%              & 0.09  & 0.03  & 0.04   & & 0.11   & 0.04  & 0.05   \\
max               & 5.09  & 2.36  & 4.39   & & 15.14  & 2.86  & 12.87  \\

\bottomrule\bottomrule
\end{tabular}
\begin{tablenotes}
  \scriptsize
  \item Panel A and panel B document the descriptive statistics of three jump estimators of BTC-D and BTC-G.
  Columns from left to right are the corrected thresholded jump estimator $J(\alpha)$ at $\alpha=99.99\%$ confidence level, the thresholded positive jump estimator $J^+$, and the thresholded negative jump estimator $J^-$.
  The threshold constant coefficient $c_{\theta}=3$.
  The first row reports the proportion of non-zero jumps.
  The last first rows contain the sample mean, sample deviation, sample minimum, 50\% quantile, and sample maximum.
\end{tablenotes}
\end{threeparttable}
\end{table}


The detected jumps processes are shown in Fig. \ref{fig:jump_process}.
On one hand, from the second figure in each panel of positive and negative jump processes, one can see that the jumps appear more frequently comparing the first figure of such panel, e.g for BTC-D 76\% of the sample days are detected with positive jumps, however, only 39\% of them are categorized as jump days (See Tab.\ref{tab:summary_des_jumps}).
On the other hand, the decomposition of $J(\alpha)$ into signed jump estimators is clean in terms of jump intensity.
The average intensity of jump components decomposition is approximate $J(\alpha) \approx J^+ + J^-$.
This conflict is partially caused by the lack of significance test on signed jumps $J^{+/-}$.
Also, The size and quantity of negative jumps $J^-$ are almost equal to that of positive jump $J^+$ which implies that a jump is not necessary a crash event in the sample period used in this article.

Jumps are usually considered as results from exogenous shocks, for example, the news shocks on the financial market.
To check the sanity of the detected jumps, we try to link the news and reports to the detected jumps by exemplifying some of the large jumps.
We choose four of the days detected with large price jumps marked in the first figure of the upper panel in Fig. \ref{fig:jump_process}.
The largest detected jump happened in our sample period is 10th March 2017, in which the Bitcoin ETF from Winklevoss twins was denied by the Securities Exchange Commission (SEC).\footnote{"Breaking: ETF Denied, Bitcoin Price Drops From \$1350 to \$980 Within Hours" from https://cointelegraph.com/}
On 29th November 2017, BTC reached \$10,000 where many analysts suspected that the market would be more volatile caused by the profit-taking investors. \footnote{Source by: https://www.fintechfutures.com/}
A mysterious bull run appeared on 12th April 2018 and the BTC price hit \$8,011 from \$6,780 in a short time. \footnote{https://www.investopedia.com/news/why-did-bitcoin-jump-1k-april-12/}
Drastic fluctuation happened on 15th October 2018.
The BTC price first surged from \$6,376 to \$7,083 and then fell back to \$6,821. \footnote{https://medium.com/@bitcurate/}


\begin{figure}[!htb]
  \begin{subfigure}{\linewidth}
    \centering
    \caption{Jump Process of BTC-D, $\sqrt{J(\alpha)}$, $\sqrt{J^+}$, and $-\sqrt{J^-}$}\label{fig:jump_dynamic_btcd}
    \includegraphics[width=6.5in]{figures/btcd_jumps_compare.png}
    \end{subfigure}\\%[1ex]

    \begin{subfigure}{\linewidth}
      \centering
      \caption{Jump Process of BTC-G, $\sqrt{J(\alpha)}$, $\sqrt{J^+}$, and $-\sqrt{J^-}$}\label{fig:jump_dynamic_btcg}
      \includegraphics[width=6.5in]{figures/btcg_jumps_compare.png}
    \end{subfigure}
    \caption{The detected jump estimators of BTC-D (top panel) and BTC-G (bottom panel) evolve over time.
    The first figure of each panel is the square root form of $J(\alpha)$ at $\alpha=99.99\%$ confidence level.
    The second figure of each panel contains the square root of the positive jump \textcolor{blue}{$J^+$} and the negative jump \textcolor{red}{$J^-$}.
    \href{https://github.com/QuantLet/RCVJ_Forecasting}{\textcolor{babyblue}{RiskBTC}}}\label{fig:jump_process}
\end{figure}

% Threshold well performed
% By the threshold smoothing method $TBPV$, much more jumps can be detected from $TJ(\alpha)$ estimator, or in other words, the threshold method has a stronger detection ability on the jumps in Bitcoin market.
% In BTC-D, 39\% of all days with jumps by $TJ$ comparing 25\% by $J$, and the statistics are 68\% against 51\% in BTC-G.
% Also, $TJ$ component is more intensive than $J$ component.
% Especially, we can see $TJ$ has much larger value at 95-percentile and maximum, this may suggest that some of the large size jumps or consecutive jumps are missed in $J$.


==> sections/subsections/DynamicsRV.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Realized Volatility in Bitcoin Market}\label{sec:rv_btc}

% This subsection discusses the dynamics of variance estimates in three aspects including descriptive statistics, empirical distribution, and series autocorrelation.

The extremely high risk of BTC comparing with tradition asset stands out immediately by the sample mean of $RV$ shown in Tab.\ref{tab:summary_des_rvs}.
For example, the sample mean of annualized daily realized variance of BTC-D is 1.16.
In contrast, one of the most volatile equity market indices, SSEC, has annualized daily realized variance 0.23. \footnote{Datasource from Realized Library, Oxford-Man Institute of Quantitative Finance. The trading hour bias is corrected by accounting the overnight price change (\cite{bollerslev2018risk}) to allow the two $RV$ estimators to be comparable.}
More comparisons are detailed in Appendix \ref{app_rvcompare_btc_indices}.

The descriptive statistics of continuous component $C$ in Tab.\ref{tab:summary_des_rvs} suggest that the discontinuities do not contribute to the risk too much.
As definition in section \ref{sec:tj}, $C$ is the difference between $RV$ and $J$ which implies closer the distance between $C$ and $RV$, lower the contribution from $J$.
On average, jumps contribute to risk up to 6.8\% \footnote{The average annualized daily $RV$ is around 1.16, and the average annualized daily jump intensity $J$ is around 0.08, hence the contribution from jump to risk is around $0.08/1.16=6.8\%$, likewise for BTC-G.} for BTC-D, and up to 17.2\% for BTC-G.
% Percentile statistics give consistent results.
And ADF unit root test suggests that most estimators do not contain unit root at 5\% significant level.

\begin{table}[!htb]
  \centering % centering table
\begin{threeparttable}
% \captionsetup{font=scriptsize}
\caption{Summary Statistics For Bitcoin Annualized Daily (Semi-)Realized Variance}\label{tab:summary_des_rvs}
\footnotesize
\begin{tabular}{l *{7}{S[table-format=-1.2,table-number-alignment = center]}}
\toprule\toprule

\multicolumn{8}{l}{\textbf{Panel A: BTC-D}}\\
% \cline{2-11}\\
% \midrule
\multicolumn{1}{c}{}
& \multicolumn{1}{c}{$RV$}
& \multicolumn{1}{c}{$RSV^+$}
& \multicolumn{1}{c}{$RSV^-$}
& \multicolumn{1}{c}{$\log(RV)$}
& \multicolumn{1}{c}{$\log(RSV^+)$}
& \multicolumn{1}{c}{$\log(RSV^-)$}
& \multicolumn{1}{c}{$C$}\\
% & \multicolumn{1}{c}{$TC$}\\
% & \multicolumn{1}{c}{$\log(C)$}
% & \multicolumn{1}{c}{$\log(TC)$}\\
\cmidrule{2-8}

mean     & 1.16       & 0.57       & 0.59       & -0.60        & -1.32        & -1.30         & 1.08       \\   %& 1.12
std      & 2.05       & 1.02       & 1.05       & 1.20         & 1.22         & 1.23          & 2.01       \\   %& 2.06
min      & 0.02       & 0.01       & 0.01       & -3.98        & -4.88        & -4.51         & 0.01       \\   %& 0.01
% 5\%      & 0.08       & 0.04       & 0.04       & -2.54        & -3.29        & -3.27         & 0.05       \\   %& 0.06
% 50\%     & 0.56       & 0.27       & 0.26       & -0.58        & -1.31        & -1.33         & 0.47       \\   %& 0.51
% 95\%     & 3.70       & 1.81       & 2.06       & 1.31         & 0.59         & 0.72          & 3.69       \\   %& 3.70
max      & 26.07      & 13.28      & 12.80      & 3.26         & 2.59         & 2.55          & 26.07      \\   %& 26.07
skewness & 5.59       & 5.78       & 5.41       & 0.06         & 0.04         & 0.10          & 5.73       \\   %& 5.60
kurtosis & 43.38      & 46.24      & 40.12      & -0.04        & -0.03        & -0.15         & 45.86      \\   %& 43.40
acf(1)   & 0.53       & 0.51       & 0.52       & 0.79         & 0.78         & 0.77          & 0.56       \\   %& 0.53
acf(7)   & 0.17       & 0.16       & 0.17       & 0.58         & 0.58         & 0.57          & 0.18       \\   %& 0.17
acf(30)  & 0.11       & 0.10       & 0.11       & 0.38         & 0.37         & 0.38          & 0.13       \\   %& 0.12
acf(100) & 0.06       & 0.06       & 0.06       & 0.23         & 0.23         & 0.23          & 0.07       \\   %& 0.06
ADF      & -3.16\twoS & -3.22\twoS & -3.12\twoS & -4.36\threeS & -4.34\threeS & -4.42\threeS  & -3.10\twoS \\   %& -3.12\twoS

\multicolumn{8}{l}{\textbf{Panel B: BTC-G}}\\
\multicolumn{1}{c}{}
& \multicolumn{1}{c}{$RV$}
& \multicolumn{1}{c}{$RSV^+$}
& \multicolumn{1}{c}{$RSV^-$}
& \multicolumn{1}{c}{$\log(RV)$}
& \multicolumn{1}{c}{$\log(RSV^+)$}
& \multicolumn{1}{c}{$\log(RSV^-)$}
& \multicolumn{1}{c}{$C$}\\
% & \multicolumn{1}{c}{$TC$}\\
% & \multicolumn{1}{c}{$\log(C)$}
% & \multicolumn{1}{c}{$\log(TC)$}\\
\cmidrule{2-8}

mean     & 0.93       & 0.45       & 0.49         & -0.92        & -1.66        & -1.64         & 0.77        \\    %& 0.85
std      & 1.76       & 0.84       & 0.98         & 1.32         & 1.32         & 1.37          & 1.55        \\    %& 1.64
min      & 0.01       & 0.00       & 0.00         & -4.88        & -5.51        & -5.63         & 0.00        \\    %& 0.00
% 5\%      & 0.04       & 0.02       & 0.02         & -3.15        & -3.90        & -4.00         & 0.02        \\    %& 0.03
% 50\%     & 0.40       & 0.19       & 0.19         & -0.91        & -1.65        & -1.64         & 0.28        \\    %& 0.33
% 95\%     & 3.17       & 1.53       & 1.73         & 1.15         & 0.42         & 0.55          & 2.95        \\    %& 3.09
max      & 21.99      & 11.78      & 14.52        & 3.09         & 2.47         & 2.68          & 21.99       \\    %& 21.99
skewness & 5.86       & 6.32       & 6.85         & -0.04        & -0.04        & -0.01         & 6.21        \\    %& 5.73
kurtosis & 47.28      & 59.42      & 68.92        & -0.10        & -0.14        & -0.19         & 57.88       \\    %& 48.03
acf(1)   & 0.42       & 0.45       & 0.35         & 0.74         & 0.73         & 0.71          & 0.50        \\    %& 0.47
acf(7)   & 0.13       & 0.14       & 0.11         & 0.49         & 0.51         & 0.47          & 0.19        \\    %& 0.16
acf(30)  & 0.09       & 0.09       & 0.07         & 0.26         & 0.26         & 0.25          & 0.14        \\    %& 0.12
acf(100) & 0.03       & 0.04       & 0.02         & 0.11         & 0.11         & 0.11          & 0.04        \\    %& 0.03
ADF      & -3.03\twoS & -3.12\twoS & -4.89\threeS & -5.06\threeS & -3.61\threeS & -5.27\threeS  & -2.77\oneS  \\    %& -2.95\twoS

\bottomrule\bottomrule
\end{tabular}
\begin{tablenotes}
  \scriptsize
  \item Panel A and panel B are the descriptive statistics of BTC-D and BTC-G.
  The left three columns are realized variance, positive realized semi-variance, negative realized semi-variance, followed by the logarithmic form of those three estimators.
  The right column is the continuous component defined as the difference between realized variance and significant jump.
  The first six rows for each panel contain the sample mean, standard deviation, sample minimum, maximum, skewness, and excess kurtosis, followed by four autocorrelation with 1-day, 7-day, 30-day, and 100-day lags. the last row reports the Augmented Dickey-Fuller test with three significance levels. \threeS: 1\% significance, \twoS: 5\% significance, \oneS: 10\% significance.
\end{tablenotes}
\end{threeparttable}
\end{table}

\begin{figure}[!htb]
  \begin{subfigure}{\linewidth}
    \centering
    \caption{Kernel Density Estimation of $RV$ estimators on BTC-D}\label{fig:kde_rvs_btcd}
    \includegraphics[width=6.5in]{figures/btcd_rvs_comparison.png}
    \end{subfigure}\\%[1ex]

    \begin{subfigure}{\linewidth}
      \centering
      \caption{Kernel Density Estimation of $RV$ estimators on BTC-G}\label{fig:kde_rvs_btcg}
      \includegraphics[width=6.5in]{figures/btcg_rvs_comparison.png}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
      \centering
      \caption{ACF of $\log(RV)$ for BTC-D (left column) and BTC-G (right column)}\label{fig:acf_btc}
      \includegraphics[width=6.5in]{figures/btcd_btcg_acf_compare.png}
      \end{subfigure}\\%[1ex]
    \caption{The top two panels are the kernel density estimation on annualized unconditional daily logarithmic estimators for BTC-D (a) and BTC-G (b).
    Logarithmic estimators in each panel include \textcolor{green}{$RV$}, \textcolor{black}{$RSV^+$}, \textcolor{red}{$RSV^-$}, and \textcolor{blue}{$C$}.
    The last panel is the \textcolor{blue}{autocorrelation function} of BTC with 95\% confidence band.
    \href{https://github.com/QuantLet/RCVJ_Forecasting}{\textcolor{babyblue}{RiskBTC}}}\label{fig:btc_rv_properties}
\end{figure}

Fig. \ref{fig:btc_rv_properties} shows two of the most important properties for $RV$, the log-normal distribution and strong temporal dependency.
We use Epanechnikov kernel with bandwidth=1.5 to estimate the density of logarithmic form of $RV$, $RSV^{+(-)}$, and $C$.
Consistent with the results that skewness and excess kurtosis of those estimators in logarithmic forms in Tab.\ref{tab:summary_des_rvs}, we can see that the $RV$ can be well approximated by a log-normal distribution.
The strong and persistent temporal dependency of $\log(RV)$ process which can be well described as a long-memory process documented in \cite{andersen2001distribution} motivates our forecasting model construction.
The ACF statistics in Tab.\ref{tab:summary_des_rvs} in line with the bottom panel in Fig. \ref{fig:btc_rv_properties} show that the $\log(RV)$ processes of both BTC-D and BTC-G have strong temporal dependency.
However, the decay of such dependency is much slower in BTC-D than in BTC-G which suggests that one could possibly improve the forecasts by diversifying the BTC investment into different online exchanges.


==> sections/subsections/EconomicValue.tex <==
%!TEX root = ../../RCVJ.tex

\subsubsection{Economic Value}\label{sec:utility}

It is a stylized fact that the model performance evaluation is heavily influenced by the choice of metrics.
For example, in the case of BTC-G $h=1$ shown in Tab.\ref{tab:OutSampleForecasts_logform}, the HAR model underperforms RSV by MZ-R$^2$, however, one can find that HAR has smaller forecasting errors than that of RSV by both HRMSE and QLIKE.

As the validity of forecasting realized variance is to be tested by the market, we employ the approach of \cite{bollerslev2018risk}.
The advantages of this approach relative to the framework of \cite{fleming2001economic} are twofold.
This so-called RU-framework evaluates utility without requiring forecasts on asset returns.
Then, it mimics a trading strategy when an investor targets at a constant Sharp ratio and adjust his/her risky asset positions according to the $RV$ forecasts.
A first-order expansion on expected utility yields (for $h=1$)

\begin{equation}
  \operatorname{E}\left[u(W_{t+1})\right] = \operatorname{E}(W_{t+1}) - \frac{1}{2}\gamma^{A}\operatorname{V}(W_{t+1}),
\end{equation}

where $\gamma^{A}$ is the absolute Pratt-Arrow risk aversion.
The Realized Utility $RU_{t+1}^{(m)}$ at time $t+1$ by model $m$ defined as utility per wealth with optimal weights $\operatorname{RU}^{(m)}_{t+1} = \operatorname{EU}(\omega_t^{(m)})/W_t$ is given by (See Appendix \ref{app_economic_value} for more details of realized utility):

\begin{equation}
  \operatorname{RU}_{t+1}^{(m)} = \frac{SR^2}{\gamma}\left(\sqrt{\frac{RV_{t+1}}{\widehat{RV}_{t+1}^{(m)}}}-\frac{1}{2}\frac{RV_{t+1}}{\widehat{RV}_{t+1}^{(m)}}\right),
\end{equation}

where $RV_{t+1}$ and $\widehat{RV}_{t+1}$ are the ex-post and forecast realized variance of $t+1$.
Sharp ratio $SR=0.4$ and relative risk aversion $\gamma=2$ are given as constant.
If one has perfect forecast, i.e $\widehat{RV}_{t+1}^{(m)}=RV_{t+1}$, then $\operatorname{RU}_{t+1}^{(m)} = \frac{SR^2}{2\gamma} = 4\%$.

As the optimal weight is given by \eqref{eq:optimal_omega} in Appendix \ref{app_economic_value}, for an investor given constant $SR/\gamma$, lower risk the investor expects for the next day, higher the proportion of wealth should be allocated to risky asset.
And in the case that $\sqrt{\widehat{RV}_{t+1}^{(m)}}<SR/\gamma$, then $\omega_t^{(m)}>1$ implies a leverage investment.
However, we restrict the weight as $\omega_t\in[0,1]$.
Consequently, when $\omega_t^{(m)}>1$, the realized utility $\operatorname{RU}^{(m)}_{t} = SR\cdot\sqrt{RV_{t+1}} - \frac{\gamma}{2}RV_{t+1}$ which is the case when $\omega_t^{(m)}=1$.

\begin{equation}\label{eq:ru}
  \operatorname{RU}^{(m)}_{t+1} =\begin{cases}
    \frac{SR^2}{\gamma}\left(\sqrt{\frac{RV_{t+1}}{\widehat{RV}_{t+1}^{(m)}}}-\frac{1}{2}\frac{RV_{t+1}}{\widehat{RV}_{t+1}^{(m)}}\right), & \text{$\frac{SR}{\gamma}\leq \sqrt{\widehat{RV}_{t+1}^{(m)}}$}\\
    SR\cdot\sqrt{RV_{t+1}} - \frac{\gamma}{2}RV_{t+1}, & \text{otherwise}
\end{cases}
\end{equation}

Clearly, the comparison almost solely depends on the forecasts $\widehat{RV}_{t+1}^{(m)}$ illustrated in \eqref{eq:ru}.
Note that each of the forecasting models is in logarithmic form, the realized utility is calculated after transforming the logarithmic forecast to squared form.
We also report the realized utility by squared form forecasting models in Appendix \ref{app_economicvalue_squareform}.

By averaging the $RU^{(m)}_{t+h}$ over time $t\in[1,T]$, one can have the realized utility $RU^{(m)}$ for each model $m$ on forecasting horizon $h$.
The realized utility provides another metric to compare forecasts from different models.
As explained above, better the forecast is, closer the $RU_{t+h}^{(m)}$ to $4\%$.

\begin{equation}
  RU^{(m)}_h = \frac{1}{T} \sum_{t=1}^{T} RU^{(m)}_{t+h}
\end{equation}

\input{tabs/Tab_EconomicValue_logform.tex}

The economic value reported in Tab.\ref{tab:economic_evaluation_logform} confirms the conclusion from the out-of-sample forecasting.
Firstly, an investor can gain higher utility regardless of the choice of the model if one forecasts in the long horizon risk.
For example, the RSVSJ model gives around 227 basis points more utility in the case of $h=30$ than that of $h=1$ for BTC-D.
Secondly, in the short horizon forecasting, $h=1$, the HAR model provides much more utility than the other models do, for example, HAR outperforms RVJ by up to around 22 basis points which suggest that modeling realized variance with the jump in the short horizon risk forecasting case would not add economic values.
However, in the longer horizon forecasting case, $h=30$, accounting either jumps or signed estimators do provide extra utility, such as RVJ model outperforms HAR model by 11 basis points utility, and RSV outperforms HAR by around 19 basis points utility for BTC-D.
This finding sheds light on realized variance forecasting models selection for BTC investors.
BTC Investors who target at a certain risk level should select the forecasting model based on their investment horizons.
Last but not least, the investors can gain more utility by investing in BTC-D than on BTC-G in the short horizon forecasting case.
BTC-D is a simple equal-weighted price portfolio which diversifies exchange idiosyncratic discontinuities changes risk (jumps) on price.
While BTC-G suffers from the extra risk inherent in some specific exchanges.


% The wealth function $W$ is explicitly given by \eqref{eq:wealth} for allocating $\omega_t$ proportion of whole wealth on the risky asset, and $r_{t+1}-r_f$ is the unknown excess return.

% \begin{align}
%   \begin{split}
%     W_{t+1} &= W_t\{1 + (1-\omega_t) r_f + \omega_t r_{t+1}\}\\
%             &= W_t\{1+r_f+ \omega_t(r_{t+1}-r_f)\}
%     \label{eq:wealth}
%   \end{split}
% \end{align}
%
% Assuming that the risk-free interest rate $r_f$ is constant, $W_t$ and $\omega_t$ are known, the expect value and variance of $W_{t+1}$ is:
%
% \begin{align}
%   \begin{split}
%     \operatorname{E}(W_{t+1})&= W_t(1+r_f) + W_t\omega_t\operatorname(r_{t+1}-r_f)\\
%     \operatorname{V}(W_{t+1})&= W_t^2\omega_t^2\cdot\operatorname{V}(r_{t+1}-r_f)
%   \end{split}
%   \label{eq:exp_var_w}
% \end{align}
%
% Given a target Sharp ratio $SR=\frac{\operatorname{E}(r_{t+1})}{\sqrt{\operatorname{V}(r_{t+1})}}$, \eqref{eq:exp_var_w} and \eqref{eq:expect_utility} give the following expression of expected utility $EU(\omega_t)$  $\operatorname{EU}(\omega_t)$ with replacing $\operatorname{V}(r_{t+1})$ by $RV_{t+1}$
%
% \begin{align}
% \operatorname{EU}(\omega_t) &= W_t\left[\omega_t\operatorname{E}(r_{t+1}) - \frac{\gamma}{2}\omega_t^2\operatorname{V}(r_{t+1})\right]\nonumber\\
%     &= W_t\left[\omega_t\operatorname{E}(r_{t+1}) - \frac{\gamma}{2}\omega_t^2RV_{t+1}\right]\nonumber\\
%     &= W_t\left[\omega_t\cdot SR\cdot\sqrt{RV_{t+1}} - \frac{\gamma}{2}\omega_t^2 RV_{t+1}\right]\label{eq:eu_final}
% \end{align}
%
% Here the $\gamma = \gamma^{A} W_{t}$ represents the relative risk aversion.
% Based on the out-of-sample forecasts $\widehat{RV}_{t+1}^{(m)}$ from model $m$, one can derive the optimal weight $\omega_t^{(m)}$ targeting $SR/\gamma$.
%
% \begin{equation}
%   \omega_t^{(m)} = \frac{SR/\gamma}{\sqrt{\widehat{RV}_{t+1}^{(m)}}}
%   \label{eq:optimal_omega}
% \end{equation}
%

% uow\_mean & 2.938\% & 2.642\% & 2.648\% & 2.606\% & 1.917\% & 2.193\% & 1.775\% & 1.517\%  & 2.546\% & 4.000\% \\
% uow\_mean & 2.928\% & 2.838\% & 2.969\% & 1.760\% & 2.953\% & 3.030\% & 3.081\% & 2.775\%  & 3.922\% & 4.000\% \\
% uow\_mean & 3.328\% & 3.439\% & 3.204\% & 3.740\% & 3.653\% & 3.681\% & 3.685\% & 3.698\%  & 3.994\% & 4.000\% \\

% uow\_mean & 2.619\% & 2.486\% & 2.311\% & 2.659\% & 2.472\% & 2.583\% & 2.402\% & 2.119\%  & 2.546\% & 4.000\% \\
% uow\_mean & 3.133\% & 2.968\% & 3.081\% & 3.157\% & 3.131\% & 3.113\% & 3.177\% & 3.058\%  & 3.922\% & 4.000\% \\
% uow\_mean & 3.470\% & 3.455\% & 3.460\% & 3.592\% & 3.166\% & 3.664\% & 3.589\% & 3.168\%  & 3.994\% & 4.000\% \\
%

% {}       & HAR & RVJ    & RVTJ   & RVSJ   & RVSTJ  & SRV    & SRVSJ  & SRVSTJ & naive  & ru\_true \\
% dm\_test & NaN & -1.535 & -1.877 & -0.813 & -1.148 & -1.060 & -1.208 & -1.948 & -1.623 & 2.517    \\
% dm\_test & NaN & 0.445  & 0.685  & -0.994 & -0.026 & 0.839  & 0.195  & -0.300 & 1.234  & 1.245    \\
% dm\_test & NaN & 0.838  & -1.328 & 1.038  & 0.968  & 1.053  & 0.988  & 0.977  & 1.072  & 1.072    \\
%
% {}       & HAR & RVJ    & RVTJ   & RVSJ   & RVSTJ  & SRV    & SRVSJ  & SRVSTJ & naive  & ru\_true \\
% p\_value & NaN & 0.125  & 0.061  & 0.417  & 0.251  & 0.290  & 0.227  & 0.052  & 0.105  & 0.012    \\
% p\_value & NaN & 0.656  & 0.494  & 0.320  & 0.979  & 0.402  & 0.846  & 0.764  & 0.218  & 0.213    \\
% p\_value & NaN & 0.402  & 0.185  & 0.300  & 0.333  & 0.293  & 0.323  & 0.329  & 0.284  & 0.284    \\
%
%
% {}       & HAR & RVJ    & RVTJ   & RVSJ   & RVSTJ  & SRV    & SRVSJ  & SRVSTJ & naive  & ru\_true \\
% dm\_test & NaN & -1.190 & -1.651 & 0.662  & -0.707 & 0.705  & -0.993 & -1.476 & -0.796 & 2.174    \\
% dm\_test & NaN & -1.107 & -1.157 & -0.681 & -0.859 & -0.982 & -0.782 & -1.198 & 2.394  & 2.444    \\
% dm\_test & NaN & -1.083 & -0.963 & -1.007 & -1.007 & 1.362  & -1.026 & -1.006 & 1.521  & 1.522    \\
%
% {}       & HAR & RVJ    & RVTJ   & RVSJ   & RVSTJ  & SRV    & SRVSJ  & SRVSTJ & naive  & ru\_true \\
% p\_value & NaN & 0.235  & 0.099  & 0.508  & 0.480  & 0.481  & 0.321  & 0.140  & 0.426  & 0.030    \\
% p\_value & NaN & 0.269  & 0.247  & 0.496  & 0.391  & 0.326  & 0.434  & 0.231  & 0.017  & 0.015    \\
% p\_value & NaN & 0.279  & 0.336  & 0.314  & 0.314  & 0.174  & 0.305  & 0.315  & 0.129  & 0.128    \\



% uow\_mean & 2.650\% & 2.342\% & 1.704\% & 1.081\% & 1.577\% & 2.099\% & 1.488\% & -0.427\% & 2.136\% & 4.000\% \\
% uow\_mean & 3.159\% & 2.361\% & 2.655\% & 1.701\% & 2.836\% & 2.822\% & 3.013\% & 3.006\%  & 3.896\% & 4.000\% \\
% uow\_mean & 3.462\% & 3.453\% & 3.540\% & 3.415\% & 3.344\% & 3.433\% & 3.663\% & 3.672\%  & 3.993\% & 4.000\% \\
%
% uow\_mean & 2.098\% & 1.871\% & 1.728\% & 1.663\% & 1.584\% & 2.019\% & 1.511\% & 1.390\%  & 2.136\% & 4.000\% \\
% uow\_mean & 2.793\% & 2.782\% & 2.548\% & 2.480\% & 2.455\% & 2.685\% & 2.638\% & 2.601\%  & 3.896\% & 4.000\% \\
% uow\_mean & 3.570\% & 3.617\% & 3.596\% & 2.993\% & 3.557\% & 3.625\% & 3.149\% & 3.609\%  & 3.993\% & 4.000\% \\



% \begin{table}
%   \begin{center}
%     \scriptsize
%     \begin{tabular}{ll }
%     \toprule\toprule
%
% \multicolumn{2}{c}{}
% &\multicolumn{1}{c}{HAR}
% &\multicolumn{1}{c}{RVJ}
% &\multicolumn{1}{c}{RVTJ}
% &\multicolumn{1}{c}{RVSJ}
% &\multicolumn{1}{c}{RVSTJ}
% &\multicolumn{1}{c}{RSV}
% &\multicolumn{1}{c}{RSVSJ}
% &\multicolumn{1}{c}{RSVSTJ}
%
% \\
%     \midrule
% \multirow{3}{*}{$h\mbox{=}1$}  & $RV$         & 3.547\% & 3.535\%                   & 3.534\%                  & 3.536\%                   & 3.535\%                   \\
%                                & $(RV)^{1/2}$ & 3.418\% & \textcolor{red}{3.493\%}  &\textcolor{red}{3.499\%}  & \textcolor{red}{3.485\%}  & \textcolor{red}{3.493\%}  \\
%                                & $\log(RV)$   & 3.137\% & \textcolor{red}{3.343\%}  &\textcolor{red}{3.303\%}  &3.364\%                    & 3.265\%                   \\
%
%      \midrule
% \multirow{3}{*}{$h\mbox{ =}7$} & $RV$         & 3.758\% & 3.728\%                   & 3.747\%                  & 3.704\%                   & 3.715\%                   \\
%                                & $(RV)^{1/2}$ & 3.718\% & 3.776\%                   & 3.783\%                  & 3.776\%                   & 3.780\%                   \\
%                                & $\log(RV)$   & 3.568\% & \textcolor{red}{3.733\%}  & \textcolor{red}{3.640\%} & 3.749\%                   & \textcolor{red}{3.664\%}  \\
%
%      \midrule
% \multirow{3}{*}{$h\mbox{=}30$} & $RV$         & 3.835\% & \textcolor{blue}{3.751\%} & 3.792\%                  & \textcolor{blue}{3.707\%} & \textcolor{blue}{3.733\%} \\
%                                & $(RV)^{1/2}$ & 3.842\% & 3.787\%                   & 3.825\%                  & 3.765\%                   & 3.775\%                   \\
%                                & $\log(RV)$   & 3.780\% & 3.769\%                   & 3.723\%                  & 3.675\%                   & 3.732\%                   \\
%
%     \bottomrule\bottomrule
%     \end{tabular}
%   \end{center}
%   \caption{BTC out-of-sample realized utility evaluated at the maximum value equals to $RU(RV_{t+h})=\frac{1}{2}SR^2/\gamma$=4\%. D-M t-test shows \textcolor{red}{Better}/\textcolor{blue}{Worse} comparing with HAR model at 5\% Significant level}\label{tab:ru_compare}
% \end{table}


==> sections/subsections/EstimatorsConstruction.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Realized Variance and Jump Estimators Construction}\label{subsec:estimator_construct}

In section \ref{sec:RV_Decomp_Model}, we illustrate the estimators used in this article including the realized (semi-)variance $RV$, $RSV^{+(-)}$ and three of the jump estimators $J^{+(-)}$.
Here we would like to clarify the notation of each estimator in different forms and over different periods.

For simplicity, any of the estimators over a longer period is computed by averaging its daily estimate over the period.
The averaging method not only has incorporated information included in different periods but also ensure estimates over different periods having the same scale.
Given a daily estimator $\hat{Y}_{\tau}$, its corresponding average estimator is defined as:

\begin{equation}\label{eq:rv_long_horizon}
  \hat{Y}_{\tau_1,\tau_2}=\frac{1}{\tau_2-\tau_1}\sum_{\tau=\tau_1+1}^{\tau_2}\hat{Y}_{\tau}
\end{equation}

Take $RV$ for example, all the empirical results are based on the annualized unconditional daily realized variance $RV_{t+1}$ in \eqref{eq:def_rv}.
The longer horizon estimator, $RV_{t,t+7}$, is average of annualized daily estimates $RV_{t,t+7}= \frac{1}{6} \sum_{\tau=t+1}^{t+7} RV_{\tau}$.

We specially denote the daily lagged, weekly lagged and monthly lagged estimators for further use as follows.

\begin{align}\label{eq:day_week_month_lag_estimate}
  \text{Daily estimator}&, \hat{Y}_{D}\overset{def}{=}\hat{Y}_{t-1,t}\nonumber\\
  \text{Weekly estimator}&, \hat{Y}_{W}\overset{def}{=}\hat{Y}_{t-7,t-1}\\
  \text{monthly estimator}&, \hat{Y}_{M}\overset{def}{=}\hat{Y}_{t-30,t-7}\nonumber
\end{align}

Those three stepwise estimators will be employed in the latter HAR model which captures the footprint of $RV's$ long memory property.

To incorporate nonlineararity, we also use estimators in logarithmic form $\log(\hat{Y})$, for example $\log(RV)$, $\log(J+1)$.
Economically, the squared form $RV$ (realized variance) is of our interest, thus any forecasting result computed from the logarithmic form is transformed back to squared form for comparison purpose.

% Smoothing estimators

% Estimators ($RV_D, RV_W, and RV_M$) above involve stepwise change as giving the same weights to a certain length of past estimates which ignore the truth that information slowly decay as going back further. We also implement exponential weighted moving average smoothing estimators on the past $RV$ and continuous components $(T)C$. Here we take the definition of $RV_{t-h,t}^{Exp}$ for example and likewise for $(T)C_{t-h,t}^{Exp}$. $RV_{t-h,t}^{Exp}$ considers an approximate exponentially decay weights for the past $h-periods$ $RV$, here we specify $h={1,7,30}$ which represents daily, weekly, and monthly, respectively.

% \begin{equation}
%   RV_{t-h,t}=\frac{\sum^{t}_{k=0}(1-\alpha)^{k}\cdot RV_{t-k}}{\sum^{h}_{k=0}(1-\alpha)^{k}}
% \end{equation}

% \begin{align}
%   \label{eq:def_exp_rv}
%   \begin{split}
%     RV_{t-h,t}^{Exp} &\overset{def}{=} \alpha RV_{t} + (1-\alpha) RV^{Exp}_{t-1}\\
%                      &=\frac{\sum^{h}_{k=0}(1-\alpha)^{k}\cdot RV_{t-k}}{\sum^{h}_{k=0}(1-\alpha)^{k}}\\
%                      &= \frac{\sum^{h}_{k=0}(1-\frac{1}{1+CoM(t-h,t)})^{k}\cdot RV_{t-k}}{\sum^{h}_{k=0}(1-\frac{1}{1+CoM(t-h,t)})^{k}}
%   \end{split}
% \end{align}
%
% Where $\alpha$ is the smoothing factor by which is defined as $\alpha = \frac{1}{1+CoM(t-h,t)}$. For each given $CoM(t-h,t)=h/2$ which is Center-of-Mass for ewma, we compute corresponding $\alpha$ and yield exponential smoothed $RV^{Exp}_{t-h,t}$. Likewise, we also have the exponentially smoothed version of continuous components, $C_{t-h,t}^{Exp}$ and $TC_{t-h,t}^{Exp}$.


==> sections/subsections/HAR.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Realized Variance Forecasting Models}\label{subsec:har_model}

In section \ref{sec:RV_Decomp_Model}, we illustrate the estimators used in this article including the realized (semi-)variance $RV$, $RSV^{+/-}$ and three of the jump estimators $J^{+/-}$.
Before proceeding to the forecasting models, we first clarify the notation of each estimator.

Following the existed literature, \textit{any of the estimators} used here, for example, the estimated realized variance $RV_{\tau_1, \tau_2}$, is computed by averaging its daily estimate over time period $[\tau_1, \tau_2]$.
Let the estimated annualized daily realized variance be $RV_{\tau}$, its corresponding average estimator is defined as:

\begin{equation}\label{eq:rv_long_horizon}
  RV_{\tau_1,\tau_2}=\frac{1}{\tau_2-\tau_1}\sum_{\tau=\tau_1+1}^{\tau_2}RV_{\tau}
\end{equation}

The averaging method not only has incorporated information over the period but also ensure estimates having the same scale.
We specially denote the daily lagged, weekly lagged and monthly lagged estimators for further use in \eqref{eq:day_week_month_lag_estimate}.
As BTC is a 24-hour/7-day trading asset, we use 7 days and 30 days for weekly and monthly estimators instead of 5 days and 20 days.
Those three stepwise estimators will then be employed in the latter HAR model which captures the footprint of $RV's$ long memory property.
% The one-week horizon estimator, $RV_{t,t+7}$, is the average of annualized daily estimates $RV_{t,t+7}= \frac{1}{6} \sum_{\tau=t+1}^{t+7} RV_{\tau}$.

\begin{align}\label{eq:day_week_month_lag_estimate}
  \text{Daily lagged estimator}&, RV_{D}\overset{def}{=}RV_{t-1,t}\nonumber\\
  \text{Weekly lagged estimator}&, RV_{W}\overset{def}{=}RV_{t-7,t-1}\\
  \text{monthly lagged estimator}&, RV_{M}\overset{def}{=}RV_{t-30,t-7}\nonumber
\end{align}

Furthermore, as shown in \ref{sec:rv_btc}, the logarithmic form of realized variance has a stronger temporal dependency and is approximately normal distributed,
we transform the estimators into logarithmic form $\log(RV)$ to incorporate nonlinearity while still keep the model simple.
As the square form, $RV$ is of our interest, any of the forecasting results computed from the logarithmic form is transformed back to square form for comparison purposes.

In the above text, we take the realized variance estimator $RV$ as an example, the realized semi-variance $RSV$ and jump $J^{+/-}$ estimators also follow the notations.

The temporal dependence structure of the realized variance process is crucial in forecasting.
Many of the studies use different ARCH, ARMA, and stochastic volatility models to capture the temporal dependency or long-memory effect.
Other than those complicated models, a simple linear model named the Heterogenous AutoRegression model, HAR, is proposed in \cite{corsi2009simple}.
The advantages of HAR can be illustrated threefold.
First, it is a parameter parsimonious volatility regression model that can be constructed easily with different lagged regressors.
Second, it captures the strong temporal dependency and shows good forecasting performance comparing with those complicated models.
Finally, HAR can be extended by using any other relevant estimators, for example, the jump components.
Such extensibility allows one to investigate a wide range of effects on $RV$.

% Here we would study the improvement of forecast accuracy from different models instead of absolute forecast accuracy,
% hence follow many of the literature on realized volatility forecasting, HAR-RV, and its extensive models are used.

The basic \textbf{HAR} model is formulated in \eqref{eq:har_def}.
As we use the logarithmic form of all estimators, we are essentially estimating the log-log HAR model.
The dependent variable $\log\left(RV_{t,t+h}\right)$ is estimated over three different horizons, $h=1,3,7$.

\begin{equation}\label{eq:har_def}
  \log\left(RV_{t,t+h}\right)=\alpha+ \log\left(X_{RV}^{\top}\right)\beta_{RV} +\varepsilon_{t,t+h}\quad t=1,2,\ldots,T,
  % \log(RV_{t,t+h})=\alpha+ \log\left(X_{RV}^{\top}\right)\beta_{RV}+ \log\left(X_{J}^{\top}\right)\beta_{J} +\varepsilon_{t,t+h},
\end{equation}

where the explanatory variables vector is defined as
\begin{equation}
  \log\left(X_{RV}^{\top}\right)=\left(\log(RV_{D}), \log(RV_{W}), \log(RV_{M})\right), \nonumber
\end{equation}
which contains the multi-period lagged realized variance estimators defined previously.
And the corresponding parameters vector is $\beta_{RV}=\left(\beta_{D},\beta_{W},\beta_{M}\right)^{\top}$.
Based on the HAR model, one could construct a model that accounts jump components by simply adding the thresholded jump estimators which are discussed in section \ref{sec:RV_Decomp_Model}, thus we have

\begin{equation}\label{eq:rvj_def}
  \log\left(RV_{t,t+h}\right)=\alpha+ \log\left(X_{RV}^{\top}\right)\beta_{RV}+ \log\left(X_{J}^{\top}\right)\beta_{J}+\varepsilon_{t,t+h}\quad t=1,2,\ldots,T,
\end{equation}

where the added jumps variables vector is
\begin{equation}
  \log\left(X_{J}^{\top}\right)=\left(\log(J_{D}+1), \log(J_{W}+1), \log(J_{M}+1)\right).\nonumber
\end{equation}

Note that here the logarithmic transform ensures that the jump estimators to be positive.
And the corresponding parameters vector is $\beta_{J}= \left(\beta_{JD},\beta_{JW},\beta_{JM}\right)^{\top}$.
We abbreviate this model as \textbf{RVJ}.
Furthermore, the HAR model can be decomposed with realized semi-variance estimators $RSV^+$ and $RSV^-$ which we name it as \textbf{RSV} model.
Such that,

\begin{equation}\label{eq:rsv_def}
  \log\left(RV_{t,t+h}\right) = \alpha + \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \varepsilon_{t,t+h}\quad t=1,2,\ldots,T,
\end{equation}

where the variables vector included positive/negative lagged regressors is defined as

\begin{equation}
  \log\left(X_{RSV}^{\top}\right)=\left(\log(RSV_{D}^+), \log(RSV_{W}^+), \log(RSV_{M}^+), \log(RSV_{D}^-), \log(RSV_{W}^-), \log(RSV_{M}^-)\right).\nonumber
\end{equation}

Correspondingly, the parameters vector is $\beta_{RSV}=\left(\beta_{D}^{+},\beta_{W}^{+},\beta_{M}^{+}, \beta_{D}^{-},\beta_{W}^{-},\beta_{M}^{-}\right)^{\top}$.
With analogous arguments, we can formulate the \textbf{RSVSJ} model by extending the RSV with positive/negative jumps, i.e

\begin{equation}\label{eq:rsvj_def}
  \log\left(RV_{t,t+h}\right) = \alpha+ \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \log\left(X_{J^{+/-}}^{\top}\right)\beta_{J^{+/-}} + \varepsilon_{t,t+h}\quad t=1,2,\ldots,T,
\end{equation}

where the jump variables vector is
\begin{equation}
  \log(X_{J^{+/-}}^{\top})=\left(\log(J_{D}^{+}+1), \log(J_{W}^{+}+1), \log(J_{M}^{+}+1), \log(J_{D}^{-}+1), \log(J_{W}^{-}+1), \log(J_{M}^{-}+1)\right),\nonumber
\end{equation}
and the jumps coefficients vector is $\beta_{J^{+/-}}=\left(\beta_{JD}^{+},\beta_{JW}^{+},\beta_{JM}^{+}, \beta_{JD}^{-},\beta_{JW}^{-},\beta_{JM}^{-}\right)^{\top}$.

All coefficients, $\beta_{RV}$, $\beta_{J}$, $\beta_{RSV}$, and $\beta_{J^{+/-}}$ are estimated by OLS.
To adjust the possible serial correlation and heteroskedasticity of the error term, we use the Newey-West covariance matrix estimator with 7, 14 and 60 lags for daily, weekly and monthly forecast horizon, respectively.
Note that all the jump estimators are based on $\alpha=0.9999$ and $c_{\theta}=3$.
To summarize it up, we construct 4 forecasting models in equations from \eqref{eq:har_def}-\eqref{eq:rsvj_def} abbreviated as \textbf{HAR, RVJ, RSV, RSVSJ}.


% On the other hand, one can also decompose the realized variance estimators. The Realized SemiVariance model \textbf{RSV} is constructed by decomposing $RV$ in HAR model with $RSV$, i.e .
% one can construct the Realized Variance Signed Jump model \textbf{RVSJ} and the Realized Variance Signed Thresholded Jump model \textbf{RVSTJ} by decomposing the jump components in RVJ and RVTJ model into signed jump components.
% To be more specifically, RVSJ can be formulated as $RV_{t,t+h}=\alpha+ X_{RV}^{\top}\beta_{RV}+ X_{J^+}^{\top}\beta_{J^+}+ X_{J^-}^{\top}\beta_{J^-}+\varepsilon_{t,t+h}$.
% And RVSTJ is $RV_{t,t+h}=\alpha+ X_{RV}^{\top}\beta_{RV}+ X_{TJ^+}^{\top}\beta_{TJ^+}+ X_{TJ^-}^{\top}\beta_{TJ^-}+\varepsilon_{t,t+h}$.
% Those two models are finer calibrated and allow different impacts of positive and negative jumps on future realized variance.
% As the explanatory variables in HAR model are only average values across certain periods, i.e equally weighted estimators.
% Here we extend HAR model with the ewma estimators described in Sec.\ref{subsec:estimator_construct} in which variables are constructed with decay coefficients (\cite{bollerslev2018risk}).
% With the ewma estimators, we can investigate if exponentially smoothing the continuous components can enhance the forecast.
% Model in \eqref{eq:har_def} replaced with un-thresholded continuous components estimators, $RV=RV^{Exp}$ and $J=J$, i.e $RV_{t,t+h}=\alpha+ X_{RV^{Exp}}^{\top}\beta_{RV^{Exp}}+ X_{J}^{\top}\beta_{J}+\varepsilon_{t,t+h}$, is named \textbf{HExp-RVJ}.
% And its thresholded version with $RV=RV{Exp}$, $J=TJ$ is then the \textbf{HExp-RVTJ} expressed as $RV_{t,t+h}=\alpha+ X_{RV^{Exp}}^{\top}\beta_{RV^{Exp}}+ X_{TJ}^{\top}\beta_{TJ}+\varepsilon_{t,t+h}$.

% As stated in Sec.\ref{subsec:estimator_construct}, those estimators can be transformed into logarithmic form and then used to construct logarithmic HAR-type models which capture the nonlinearity.

% Also, the logarithmic forecasting model ensures forecasts values $RV$ to be positive.
% Here we simply define the logarithmic HAR-type models by replacing all estimators with the logarithmic form.

% \begin{align}\label{eq:log_sqr_har_def}
%   \begin{split}
%     \log\left(y_{t,t+h}\right) &= \alpha+ \log\left(X_{RV}\right)^{\top}\beta_{RV}+ \log\left(X_{J}\right)^{\top}\beta_{J} +\varepsilon_{t,t+h},\\
%     % y_{t,t+h}^{1/2} &= \alpha + \left(X_{RV}^{1/2}\right)^{\top}\beta_{RV}+ \left(X_{J}^{1/2}\right)^{\top}\beta_{J} +\varepsilon_{t,t+h},\nonumber\\
%   \end{split}
% \end{align}

% Where, for example, $\log\left(X_{RV}\right)^{\top}=\left(\log(RV_{D}), \log(RV_{W}), \log(RV_{M})\right)$.


==> sections/subsections/InSampleFit.tex <==
% !TEX root = ../../RCVJ.tex

\subsection{In-Sample Forecasting Analysis}

To analyze how each explanatory variable affects future $RV$, we fit each of the forecasting models with full sample, i.e from the start of 2017 until the Middle of 2019\footnote{The sample date lasts until July 2019 for BTC-D and May 2019 for BTC-G}, named as full-sample forecasting.

\afterpage{\input{tabs/Tab_InSampleFit_RVtype_BTCDG.tex}}
\afterpage{\input{tabs/Tab_InSampleFit_SRVtype_BTCDG.tex}}

Tab.\ref{tab:InSampleReg_RVtype_BTCDG} reports the regression results of HAR and RVJ models in which estimators are not decomposed into positive and negative.
The in-sample forecasting results show consistently that the lagged $RV$ has a strong and persistent positive relationship with future $RV$ in all of the three forecasting horizons.
For example, the coefficient of 1-day lagged $\log(RV)$ can be up to 0.600.
The significance of autocorrelation decays as the estimator lagged more, e.g $\beta_D=0.568$ and $\beta_W=0.236$ for HAR model in $h=1$ case as shown in BTC-D part of tab.\ref{tab:InSampleReg_RVtype_BTCDG}.
And this effect decays with longer forecasting horizon, e.g $\beta_D=0.568$ in $h=1$ case, and $\beta_D=0.202$ in $h=30$ case.
Also, the 1-day lagged detected jumps induce significant lower future realized variances in both BTC-D and BTC-G across all of the three forecasting horizons.
This suggests that higher jump shocks, on average, actually reduce future risk.
Further more, the Adj-$R^2$ raises along with the forecasting horizon, e.g in BTC-D from 0.333 in $h=1$ case to 0.397 in $h=30$ case.

Tab.\ref{tab:InSampleReg_SRVtype_BTCDG} contains the in-sample forecasting results of RSV and RSVSJ model which account for the positive and negative effect from past realized variances or jumps.
It shows that future realized variances of BTC is strongly impacted by the positive jumps, and such impact is significant and persistent.
One can see that there is a significant negative relationship between the positive jumps and future realized variances in those three forecasting horizons.
While the relationships in most cases between negative jumps and future realized variances are insignificant.
This finding slightly differs from the result in \cite{patton2015good} in which negative jumps lead to significant higher future volatility.
Also, one can see that both the positive and negative realized variances lead to significant higher future realized variances.

One of the assumptions of the full-sample forecasting is the stability of coefficients, namely the market is not changing too volatile.
However, such an assumption is too strong for the Bitcoin market in which a lot of speculations have been happening.
When the market changes intensively, any model could be biased if it is calibrated only in a certain period.
Hence, such a fitted model would underperform in the out-of-sample forecasting as the forecasting period could deviate from the fitting period substantially.
We implement the rolling window method to allow the parameters changing over time, then the more reasonable comparisons can be obtained.

% The fast-changing market is not only characterized by high volatility but also observed with market changes.
% Despite the parameter estimations changing over time using a rolling window described in the next subsection, it is worth looking into the average impacts of those predictors as some of the contrary facts motivate us to
% [-] How do we conduct this adaptive method?\\

The adaptive method mimics an investor who updates the forecasting model based on the most recent information.
A simple case is assuming that such updates are based on a fixed amount of lagged information.
The window size $T$ of the adaptive HAR models employed here is 90-days, i.e models are estimated by using past 90-days samples.
And all the models are re-estimated every day.
After the re-estimation of each day, the out-of-sample forecasts are performed in horizons $h=1, 7, 30$, spontaneously.
As a result, we re-estimate each model 744-times for BTC-D and 763-times for BTC-G.

\afterpage{\begin{landscape}
  \begin{figure}[!htb]
    \begin{subfigure}{\linewidth}
      \centering
      \caption{BTC-D Coefficients and $t$-values of evolving. From Feb. 2017 to Feb. 2019}\label{fig:B_d_evolving_BTCD}
      \includegraphics[width=22cm]{figures/BTCD_CB_Log_RV_1_5min_AllJump_91_90_1_day_RVChange.png}
      % \includegraphics[width=22cm]{figures/BTC_RV_1_5min_AllJump_91_90_1_dayRVChange.png}

      \end{subfigure}\\%[1ex]
      \begin{subfigure}{\linewidth}
        \centering
        \caption{BTC-G Coefficients and $t$-values of evolving. From Feb. 2017 to Apr. 2019}\label{fig:B_d_evolving_BTCG}
        \includegraphics[width=22cm]{figures/BTCG_CB_Log_RV_1_5min_AllJump_91_90_1_day_RVChange.png}
        % \includegraphics[width=22cm]{figures/gemini_BTC_RV_1_5min_AllJump_91_90_1_dayRVChange.png}

      \end{subfigure}
      \caption{Point estimation of parameter (solid red line) and the confidence interval with 95\% confidence level (blue dash line) change over time.
      Panel (a) reports BTC-D case from Feb. 2017 to Feb. 2019 and panel (b) reports BTC-G case from Feb. 2017 to Apr. 2019.
      For each panel, figures from left to right are coefficients of $RV_{D}$ from HAR model, $RSV^+_{D}$ and $RSV^-_{D}$ from RSV model, respectively.
      The green horizontal line represents the value of zero and vertical grey band marks the period from Dec. 17th 2017 to Feb. 6th 2018.
      }\label{fig:B_d_evolving}
  \end{figure}
  % \hfill \href{https://github.com/QuantLet/RCVJ_Forecasting}{\qlet{RiskBTC\_Plot}}
\end{landscape}
}

\afterpage{\begin{landscape}
  \begin{figure}[!htb]
    \begin{subfigure}{\linewidth}
      \centering
      \caption{BTC-D Coefficients and $t$-values of evolving. From Feb. 2017 to Feb. 2019}\label{fig:J_d_evolving_BTCD}
      \includegraphics[width=22cm]{figures/BTCD_CB_Log_RV_1_5min_AllJump_91_90_1_dayJumpChange.png}
      % \includegraphics[width=22cm]{figures/BTC_RV_1_5min_AllJump_91_90_1_dayRVChange.png}

      \end{subfigure}\\%[1ex]
      \begin{subfigure}{\linewidth}
        \centering
        \caption{BTC-G Coefficients and $t$-values of evolving. From Feb. 2017 to Apr. 2019}\label{fig:J_d_evolving_BTCG}
        \includegraphics[width=22cm]{figures/BTCG_CB_Log_RV_1_5min_AllJump_91_90_1_dayJumpChange.png}
        % \includegraphics[width=22cm]{figures/gemini_BTC_RV_1_5min_AllJump_91_90_1_dayRVChange.png}

      \end{subfigure}
      \caption{Point estimation of parameter (solid red line) and the confidence interval with 95\% confidence level (blue dash line) change over time.
      Panel (a) reports BTC-D case from Feb. 2017 to Feb. 2019 and panel (b) reports BTC-G case from Feb. 2017 to Apr. 2019.
      For each panel, figures from left to right are coefficients of $J_{D}$ from RVJ model, $J^+_{D}$ and $J^-_{D}$ from RSVSJ model, respectively.
      The green horizontal line represents the value of zero and vertical grey band marks the period from Dec. 17th 2017 to Feb. 6th 2018.}\label{fig:J_d_evolving}
  \end{figure}
  % \hfill \href{https://github.com/QuantLet/RCVJ_Forecasting}{\qlet{RiskBTC\_Plot}}
\end{landscape}
}
% [-] Elaborate on the arguments why market structures change and the implications\\

Fig. \ref{fig:B_d_evolving} shows the changing of parameters $\beta_D^{(+/-)}$ of the unsigned and signed one-day estimator in HAR and RSV model.
The parameters are evolving systematically which justify the adaptive forecasting method.
The red solid lines represent the point estimation of parameters, the blue lines are the confidence interval with a 95\% confidence level, and the green horizontal line indicates the zero value.
The left figure of each panel confirms that the significant positive impact of 1-day lagged $RV$ is persistent during the whole sample.
The other two figures show the upside and downside risk estimators play "complementary" roles in forecasting over time.
Over the 2 years, the upside risk coefficients $\beta_D^+$ evolve as a u-shape curve, and oppositely the pattern of the downside risk coefficients $\beta_D^-$ are similar to an inverse u-shape curve.
Despite the full-sample fitting suggesting that both upside risk and downside risk lead to higher future realized variances, one can see that the coefficient of downside risk $RSV_D^-$ tends to be positive in the whole sample, and significant in a long period.
Fig. \ref{fig:J_d_evolving} contains the evolving of the parameter of one-day lagged estimator, i.e $\beta_{JD}$ in RVJ and $\beta_{JD}^{+/-}$ RSVSJ model.
The left figure of each panel suggests that jumps will lead to a significant higher future realized variances.
The right two figures show that the parameters of signed jump estimators are fluctuating below zero most of the time, which indicates the negative (insignificant) impact of signed jumps.
Comparing with the negative jumps, the positive jumps $J^+$ have a more consistent negative relationship between future realized variances.

% We can link the impacts of upside/downside risk and positive/negative jumps link to the market status.
% Specifically, the downside risk plays a more important role in forecasting $RV$ during volatile periods.
% For example in the period from late-2017 to mid-2018 when Bitcoin price reached the peak price around 20,000 U.S. dollars in December 2017 and then was plunged more than 50\%.
% During the volatile period, on one hand, $RSV_D^-$ has a significant positive impact on the next day realized variance which implies that the downside risk would cause higher volatility.
% On the other hand, the upside risk $RSV_D^+$ tends to reduce market volatility during the same sample period, however, such an effect is not significant.
% Such finding is consistent with conclusion in \cite{patton2015good} which shows that $RSV^-$ has stronger impact on future $RV$.

One of the most interesting periods of BTC is the huge market crash at the beginning of 2018.
We mark the period from December 27th, 2017 (peak price day) to February 6th, 2018 (the lowest point in this crash) with grey shadow in Fig. \ref{fig:B_d_evolving} and \ref{fig:J_d_evolving}.
Both the parameters $\beta_D$ and $\beta_{JD}$ in both BTC-D and BTC-G (left figure of each panel in Fig. \ref{fig:B_d_evolving} and \ref{fig:J_d_evolving}) reach a high level in this period which means that future realized variances are positively impacted by realized variances and jumps, significantly.
More importantly, one can see that the negative realized variances and positive jumps lead to significant changes in future realized variances as shown in the right figures of Fig. \ref{fig:B_d_evolving} and \ref{fig:J_d_evolving}.
Specifically, the downside risk has a significant positive relationship with future risk, while the positive jumps bring lower future risk during this bearish market.
The rationale behind this finding is that when the market is seen to be falling, on one hand, higher the downside risk more of the investors incline to escape, hence the market gets more volatile.
On the other hand, the positive price jumps may create the illusion of market bouncing back which could calm down the market and decrease the volatility.

% Noted that all results are drawn from models in logarithmic form, nevertheless, results from square form models show consistent results.


% \afterpage{\begin{figure}[!htb]
%   \begin{subfigure}{\linewidth}
%     \centering
%     \caption{BTC-D Coefficients and $t$-values of evolving. From Feb. 2017 to Feb. 2019}\label{fig:J_d_evolving_BTCD}
%     \includegraphics[width=16cm]{figures/BTC_Log_RV_1_5min_AllJump_91_90_1_dayJumpChange.png}
%     % \includegraphics[width=16cm]{figures/BTC_RV_1_5min_AllJump_91_90_1_dayJumpChange.png}
%
%     \end{subfigure}\\%[1ex]
%     \begin{subfigure}{\linewidth}
%       \centering
%       \caption{BTC-G Coefficients and $t$-values of evolving. From Feb. 2017 to Apr. 2019}\label{fig:J_d_evolving_BTCG}
%       \includegraphics[width=16cm]{figures/gemini_BTC_Log_RV_1_5min_AllJump_91_90_1_dayJumpChange.png}
%       % \includegraphics[width=16cm]{figures/gemini_BTC_RV_1_5min_AllJump_91_90_1_dayJumpChange.png}
%
%     \end{subfigure}
%     \caption{Parameter (in red line) and its corresponding $t$-value (blue dots) changes over time. For each panel, figures from (lower) upper left to (lower) upper right are coefficients of $(T)J_{D}$ from RV(T)J model, of $(T)J^+_{D}$ from RVS(T)J model, and $(T)J^-_{D}$ from RVS(T)J model, respectively. The dash line represents $t\mbox{-}value=\pm 1.987$. All models are in logarithmic form and horizon $h=1$}\label{fig:J_d_evolving}
%     \hfill \href{https://github.com/QuantLet/RCVJ_Forecasting}{\qlet{RiskBTC\_Plot}}
% \end{figure}
% }


==> sections/subsections/Liquidity.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Liquidity of Bitcoin Market}

Bitcoin market is trading all-day and all-year globally akin to the foreign exchange market which prompt the issue of removing the illiquidity periods, such as weekends/holidays, and inactive trading hours.
We break down this issue into two parts.

The first part is the "calendar" effect which suggests that in some of the trading days when there are not enough trading activities, such as weekends or some national holidays,
information can only be incorporated into prices in the very next "real" trading day.
Removing those inactive days could reduce the "calender" effect but might also introduce biases.

We do not remove any trading days because many of the non-institutional investors who trade during non-business days in the cryptocurrency market.
Also, program trading is common in such "high-tech" centered market evidenced by Fig.\ref{fig:program_trade} in which we show that the very same logarithmic returns (rounded to 19 decimals) appears over 100 times in 2016 and it appears 7 times on March 3rd, 2016.

\begin{figure}[!htb]
\centerline{
\includegraphics[width=6in]{figures/program_trade.png}
}
\caption{Same logarithmic return appears multiple times on March 3rd, 2016.}\label{fig:program_trade}
\hfill \href{https://github.com/QuantLet/RCVJ_Forecasting}{\qlet{RiskBTC\_Plot}}
\end{figure}

The second issue comes from the definition of "day".
As documented in previous literature, one could define a day as "21:05 GMT one night to 21:00 GMT next evening" (\cite{andersen2001distributionexchangerate}).
Truncating the "night periods" is also commonly seen in the literature.

The answer relies on whether Bitcoin market is a truly global market which has the same liquidity over the day or it is liquidity restricted for certain periods of the day.
We justify the problem by investigating the trading volume pattern regarding BTC-D and BTC-G price processes.
First, we define the Average Relative Trading Intensity $ARTI_{j\Delta}$ for each 5-minute interval $\left[(j-1)\Delta,j\Delta\right]$ to compare liquidity differences over time periods in Bitcoin market.

\begin{equation}
  \begin{split}
    ARTI_{j\Delta}&\overset{def}{=}\frac{1}{N}\sum^{N}_{t=1}RTI_{t+j\Delta}\\
    RTI_{t+j\Delta}&\overset{def}{=}\frac{vol_{t+j\Delta} - Minvol_{t+j\Delta,K}}{Maxvol_{t+j\Delta,K} - Minvol_{t+j\Delta,K}}
  \end{split}
\end{equation}

Where $Minvol_{t+j\Delta,K}=\min_{k=-K\dots,0,\dots K}vol_{t+(j+k)\Delta}$ is the local minimum trading volume around $t+j\Delta$,
Likewise $Maxvol_{t+j\Delta,K}$ is the local maximum trading volume value.
Here we fix the window length $K=288$ which can be referred to 48-hour ($\Delta=5\mbox{-}minute$) relative trading intensity.
And the $N$ is the number of days in our sample.

$RTI_{t+j\Delta}\in[0,1]$ is essentially a rolling-window min-max transformation which assigns the maximum values to 1 and the minimum values to 0.
If the liquidity is almost equally distributed over time in day $t$, then $ARTI_{j\Delta}$ should evolve stably.

\begin{figure}
  \includegraphics[width=6in]{figures/volume_acrossday.png}
  \caption{Average Relative Trading Intensity of BTC-D (left) and BTC-G (right) in 5-minute interval. Year of 2016, 2017, and 2018.}\label{fig:volume_acrossday}
  \hfill \href{https://github.com/QuantLet/RCVJ_Forecasting}{\qlet{RiskBTC\_Plot}}
\end{figure}

In this article, we define the day as 0:00 GMT to 23:55 GMT.
Fig.\ref{fig:volume_acrossday} shows the $ARTI_{j\Delta},j=1,\dots,288$ for BTC-D and BTC-G.
As stated in the previous section, three out of four exchanges in our dataset are based on the U.S.
Consistently, the active trading time period for both BTC-D and BTC-G are both around 15:00 GMT which is the likely the trading hour of the U.S market.
However, in our dataset, one can see that many trades were also generated during European, Asian market trading hours.
It would be biased if one takes account only the U.S. market trading hours.
Despite the fact that some $ARTI$ extreme outliers exist for BTC-G, we still see similar trading volume pattern between those two prices processes.


==> sections/subsections/PriceProcess.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Price Process of BTC}\label{sec:price_process}



==> sections/subsections/RSVJ.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Realized Semivariance and Signed Jumps}

In this subsection, we go further to discuss the detection of positive and negative jumps.
Recall that under the continuous jump diffusion model assumption, the jump component of quadratic variation $QV_{t+1}$ is the accumulated sum of squared infinitesimal changes $\Delta p_s=p_s - p_{s_-}$, i.e $\sum_{t<s\leq t+1} (\Delta p)^2(s)$.
Hence, the jump component is guaranteed to be non-negative as defined in \eqref{eq:tj_sig}.
On the other hand, from the finance perspective, investors are keen to understand the dynamics of the positive and negative jump, especially how those estimators impact the market of their interests.
For example, the asymmetric effect of positive and negative risk on asset returns is well investigated in previous literature.

Realized semivariance $RSV$ (\cite{barndorff2008measuring}) provides us one way to separate positive and negative jumps from the realized variance process.
The definition of positive (negative) $RSV^{+(-)}$ shown in \eqref{eq:sv} is essentially the the sum of the squared positive (negative) logarithmic returns.

\begin{equation}\label{eq:sv}
  RSV^{+(-)}_{t+1} = \sum^{1/\Delta}_{j=1}r_{t+j\Delta}^2\cdot \mathbf{I}\{r_{t_j\Delta}>(<)0\}
\end{equation}

It is straight forward that $RV$ can be decomposed into $RSV^+$ and $RSV^-$ completely, i.e $RV = RSV^+ + RSV^-$, for both finite sample and large sample cases.
As sampling frequency $1/\Delta$ goes infinite, the limiting behavior of $RSV$ given by \eqref{eq:sv_convg} under infill asymptotics shows that $RSV^{+(-)}$ converges to one-half of the integrated variance and positive (negative) sum of squared jumps.
For example,
% Such decomposition is also evidenced by our empirical result that the sum of the average value of $RSV^+$ and $RSV^-$ is almost the average value of $RV$.

\begin{equation}\label{eq:sv_convg}
  RSV^+_{t+1}\overset{p}{\to} \underbrace{\frac{1}{2}\int^{t+1}_{t} \sigma^2(s)ds}_{\frac{1}{2}IV_{t+1}} + \underbrace{\sum_{t<s\leq t+1} (\Delta p_s)^2\cdot\mathbf{I}\{\Delta p_s>0\}}_{J^+_{t+1}}.
\end{equation}

With this convergence property above and the property of $BPV$ described in \eqref{eq:bpv_j_conv_def}, one can easily separate the Positive (Negative) Jumps $J^{+(-)}$ by subtracting $RSV^{+(-)}$ by $TBPV$.
As defined in \eqref{eq:signed_j}.

\begin{equation}\label{eq:signed_j}
  J^{+(-)}_{t+1} \stackrel{\operatorname{def}}{=} \operatorname{max}\left\{RSV^{+(-)}_{t+1} - \frac{1}{2}TBPV_{t+1},0\right\}
\end{equation}


==> sections/subsections/RVJ.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Realized Variance and Jump} \label{subsec:RVJ}

Realized variance $RV_{t,t+1}$ is simply the cumulative squared logarithmic returns over time period $[t,t+1]$:
(For convenience, we omit one $t$, i.e $RV_{t+1}=RV_{t,t+1}$)

\begin{equation}\label{eq:def_rv}
  RV_{t+1}(\Delta) \stackrel{\operatorname{def}}{=} \sum^{1/\Delta}_{j=1}r^2_{t+j\Delta}
\end{equation}

To calculate \eqref{eq:def_rv}, $[t,t+1]$ is partitioned into $N$ intervals evenly.
The sampling step is $\Delta=1/N$, for example, with 288 observations each day, $\Delta=1/288$.
By the theory of quadratic variation, the increment of Quadratic Variation $QV$ of $p(t)$ can be expressed as:

\begin{equation}
  \begin{split}
    QV_{t+1} &= \plim_{\Delta\to 0}\sum^{1/\Delta}_{j=1}r^2_{t+j\Delta}\\
             &= \int^{t+1}_{t} \sigma^2(s)ds + \sum_{t<s\leq t+1} \kappa^2(s)
  \end{split}
\end{equation}

The variation of $p(t)$ measured by $QV$ comes from two sources, one is driven by the c\`adl\`ag process and one is caused by the jump process.
A series of literature discusses the convergence properties of $RV$.
\cite{andersen2001distributionexchangerate}, \cite{barndorff2002econometric}, \cite{barndorff2002estimating} document the absence of jumps.
Later, \cite{barndorff2004power}, \cite{barndorff2006econometrics}, \cite{andersen2007roughing} generalize to possible jumps.
$RV$ converges in probability to $QV$ as $\Delta$ goes to 0:

\begin{equation}\label{eq:rv_decomp}
  RV_{t+1}(\Delta) \stackrel{\operatorname{p}}{\to} \underbrace{\int^{t+1}_{t} \sigma^2(s)ds}_{IV_{t+1}} + \underbrace{\sum_{t<s\leq t+1} \kappa^2(s)}_{J_{t+1}}
\end{equation}

Hence, $RV$ consists of two components: The continuous $IV$ component, and the Jump component $J$.
The BiPower Variation $BPV$ measuring the continuous process allows separating the components

\begin{equation}\label{eq:bpv}
  BPV_{t+1}(\Delta) = \mu_{1}^{-2}\sum_{j=2}^{1/\Delta} |r_{t+j\Delta}| \cdot |r_{t+(j-1)\Delta}|,
\end{equation}

where $\mu_1=\sqrt{2/\pi}$.
$BPV$ converges in probability to $IV$ in \eqref{eq:rv_decomp} as $\Delta$ goes to 0.  % A general form of $BPV$ is the MultiPower Variance, see Appendix \ref{app_mpv}.
Intuitively, $BPV$ is robust to an infrequent jump process as it is smoothed by cumulating the adjacent logarithmic returns.
$J$ can, therefore, be isolated by taking the difference of $RV$ and $BPV$.
And then the difference is truncated to guarantee that $J$ is non-negative, see \eqref{eq:bpv_j_conv_def}.

\begin{align}\label{eq:bpv_j_conv_def}
  \begin{split}
      BPV_{t+1}(\Delta) &\stackrel{\operatorname{p}}{\to} \int^{t+1}_{t} \sigma^2(s)ds\\
      \vspace{-0.2cm}
      RV_{t+1}(\Delta) - BPV_{t+1}(\Delta) &\stackrel{\operatorname{p}}{\to} \sum_{t<s\leq t+1}\kappa^2(s)\\
      \vspace{-0.2cm}
      J_{t+1} &\stackrel{\operatorname{def}}{=} \max\left\{RV_{t+1}(\Delta) - BPV_{t+1}(\Delta),0\right\}
    \end{split}
\end{align}


==> sections/subsections/RV_Distribution.tex <==
%!TEX root = ../../RCVJ.tex

\subsection{Conditional Distribution of Realized Variance}

One of the motivations of jump detection is observing how jump shocks the distribution of future $RV$, i.e the conditional distribution of $RV$.
Each subfigure in Fig.\ref{fig:rv_impact_jtj} shows the distribution of $RV$ unconditional, conditional on having (T)J, and conditional on having no-(T)J.
Figures in Fig.\ref{fig:rv_impact_jtj} show consistently that if a jump being detected at day $t$, the distribution of next day's $\log(RV_{t+1})$ would shift negatively implying that jump possibly reduce risk on the next day.
On the other hand, if there is no jump being detected, the bitcoin market is, on average, more volatile in the next day.\textbf{[add figures for h=7,30 in appendix]}
In this article, by inserting the jump measures into the HAR model, we will further discuss how jumps impact realized volatility in the future.
% However, it is ambiguous to draw any conclusion from Fig.\ref{fig:rv_impact_npjtj} as the empirical distributions of $\log(RV_{t+1})$ conditioning on having jumps/no-jumps on time $t$ under all measures are entangled.

% \subsection{In-sample Forecasting}
\begin{figure}[!htb]
  \begin{center}
    \includegraphics[width=6in]{figures/By_JTJ_1.png}
  \end{center}
  \caption{Distribution of \textbf{BTC-D} and \textbf{BTC-G} $\log(RV_{t+1})$ conditioning on jumps/no-jumps appear on day $t$.}\label{fig:rv_impact_jtj}
\end{figure}

\begin{figure}[!htb]
  \begin{center}
    \includegraphics[width=6in]{figures/By_NPJTJ_1.png}
  \end{center}
  \caption{Distribution of \textbf{BTC-D} and \textbf{BTC-G} $\log(RV_{t+1})$ conditioning on signed-jumps/no-signed-jumps appear on day $t$.}\label{fig:rv_impact_npjtj}
\end{figure}


==> sections/subsections/TJ.tex <==
%!TEX root = ../../RCVJ.tex
\subsection{Threshold Bipower Variance and Jump}\label{sec:tj}

% \begin{figure}[!htb]
%   \centering{
%   \includegraphics[width=16cm]{figures/extremly_volatile_day.png}
%   \caption{$BPV$ is biased to consecutive jumps: A trajectory of the intraday behavior of BTC-G, 17th May 2019.
%   $RV=6.09$, $BPV=6.44$ imply that no jump has happened in this day.
%   Upper panel shows the logarithmic return process and the bottom panel is the corresponding trading volume. Both in 5-minute sampling frequency.}\label{fig:jumps_intraday}
%   }
% \end{figure}

$BPV$ is effective in the sense of smoothing a variation process when both size and quantity in the jump process are relatively small,
in other words, $BPV$ is biased to large and consecutive jumps which are not evidently appropriated for investigating cryptocurrencies.

For example, Fig.\ref{fig:jumps_intraday} shows that consecutive jumps occurred in case the variation process is not smoothed by $BPV$.
We can observe three big price jumps on 17th May 2019, consecutively, around 3 o'clock in the morning (GMT), however, the annualized $RV=6.09$ and $BPV=6.44$ imply that no jump happened during that day.
% And such a realization can be found frequently in the Bitcoin market.
% Empirical evidence shown in Fig.\ref{fig:jumps_sig} indicates that the $BPV^{1/2}$ process is very similar to the $RV^{1/2}$ process which in turn cause the $J^{1/2}$ estimator biased.

We correct such bias by implementing the threshold variation model.
The main idea of Thresholded MultiPower Variation $TMPV$ is documented in \cite{mancini2009non} which essentially truncates any logarithmic return when it exceeds a certain level of $\theta$.
At time point $t+j\Delta$, the threshold value $\theta_{t+j\Delta}$ is varying along with local variance $\widehat{V}_{t+j\Delta}$ for given constant coefficient, i.e $\theta_{t+j\Delta} = c_{\theta}^2\cdot\widehat{V}_{t+j\Delta}$.
\cite{corsi2010threshold} show that any unbiased estimator for realized local variance $\sigma^2$ can be implemented, e.g the \cite{fan2008nonlinear} estimator we use detailed in Appendix \ref{app_local_V} which is essentially a kernel smoothing estimator.
The constant $c_{\theta}$ also impacts $TMPV$, i.e as $c_{\theta}$ goes larger, $TMPV$ truncates less values.
In our main empirical results, we follow the literature and choose $c_{\theta}=3$.
After the estimation of threshold value $\theta_{t+j\Delta}$, one can directly truncate the returns exceeded the threshold.
However, this could also annihilate some of the price changes for $TBPV$ that are not "real" jumps which in turn cause more "fake" jumps been detected.
Hence, we implement the corrected version of $TMPV$ that relieves the "double-sword" bias (\cite{corsi2010threshold}).
To avoid confusion, $TMPV$ is short for the corrected version of $TMPV$ hereafter.

Essentially, instead of eliminating every of the points that has square-returns $r^2_{t+j\Delta}$ larger than certain threshold value $\theta_{t+j\Delta}$, the corrected $TMPV$ replaces the $\eta\mbox{-}th$ power logarithmic return $|r|^{\eta}_{t+j\Delta}$ with $r^e(\theta_{t+j\Delta},\eta)$ which is the expected value under assumption that $r_{t+j\Delta}\thicksim N(0,\sigma^2)$.
The conditional replacement logarithmic return $C_{\eta}(r_{t+j\Delta},\theta)$ can be written as:

\begin{equation}
  C_{\eta}(r_{t+j\Delta},\theta_{t+j\Delta}) = \left\{
            \begin{array}{lr}
            |r_{t+j\Delta}|^{\eta} & ,r^2_{t+j\Delta}\leq \theta\\
            r^e_{t+j\Delta}\left(\theta_{t+j\Delta}, \eta\right) & ,r^2_{t+j\Delta}>\theta
            \end{array}
          \right.
\end{equation}

More details about expected logarithmic return $r^e_t\left(\theta_t, \eta\right)$ is documented in Appendix \ref{app_conditional_return}.

Similar to procedure for detecting $J$, two special cases of $TMPV$ are used here.
$TBPV$ estimates $\int_{t}^{t+1}\sigma^2(s)ds$ and $TTPV$ estimates $\int_{t}^{t+1}\sigma^4(s)ds$.
Two estimators are defined as follows.
% The general form of corrected $TMPV$ is detailed in the Appendix \ref{app_ctmpv}.

\begin{alignat}{2}
    TBPV_{t+1}(\Delta)&=\mu_1^{-2}&&\cdot\sum_{j=2}^{1/\Delta}C_1(r_{t+j\Delta},\theta_{t+j\Delta})C_1(r_{t+(j-1)\Delta},\theta_{t+(j-1)\Delta})\\
    TTPV_{t+1}(\Delta)&=\mu_{\frac{4}{3}}^{-3}&&\cdot\Delta^{-1}\cdot\sum_{j=3}^{1/\Delta}C_{\frac{4}{3}}\left(r_{t+j\Delta},\theta_{t+j\Delta}\right)\\
                      &                        &&\cdot C_{\frac{4}{3}}\left(r_{t+(j-1)\Delta},\theta_{t+(j-1)\Delta}\right)\nonumber\\
                      &                        &&\cdot C_{\frac{4}{3}}\left(r_{t+(j-2)\Delta},\theta_{t+(j-2)\Delta}\right)\nonumber
\end{alignat}

Test for thresholded jumps $t\mbox{-}z$ is given by \eqref{eq:tj_test},
provided by \cite{corsi2010threshold} which is based on the ratio statistic from \cite{10.1093/jjfinec/nbi025}, detailed in \cite{andersen2007roughing} under continuous jump diffusion model.
Where $\zeta=\frac{\pi^2}{4}+\pi-5$.
Under a series assumptions, for the null hypothesis that no jump exists, $t\mbox{-}z$ converges to standard normal distribution as $\Delta$ goes to 0, i.e $t\mbox{-}z \stackrel{\mathcal{L}}{\rightarrow}N(0,1)$.

\begin{equation}\label{eq:tj_test}
  t\mbox{-}z_{t+1}=\frac{\left\{RV_{t+1}(\Delta)-TBPV_{t+1}(\Delta)\right\}RV_{t+1}^{-1}(\Delta)} {\sqrt{\Delta\cdot\zeta\cdot\max\left\{{1,\frac{TTPV_{t+1}(\Delta)}{\{TBPV_{t+1}(\Delta)\}^2}}\right\}}}
\end{equation}

% TJ part
Then, we redefine the corrected version of realized Jumps $J$ taking account only the significant jumps by $t\mbox{-}z$ test.

\begin{equation}\label{eq:tj_sig}
  J_{t+1}(\Delta)\stackrel{\operatorname{def}}{=}\max\left\{{RV_{t+1}(\Delta)-TBPV_{t+1}(\Delta)},0\right\}\cdot\mathbf{I}\left\{t\mbox{-}z_{t+1}>\Phi^{-1}_{\alpha}\right\}
\end{equation}

Consequently, we can enforce the $RV=C+J$ by defining continuous component $C_{t+1}(\Delta)\stackrel{\operatorname{def}}{=}RV_{t+1}(\Delta)-J_{t+1}(\Delta)$.


% \begin{figure}[!htb]
%   \begin{subfigure}{\linewidth}
%     \centering
%     \caption{Jump of \textbf{BTC-D} separated from \textbf{BPV}. From 1st January 2017 to 31st May 2019}\label{fig:jumps_sig_btcd}
%     \includegraphics[width=16cm]{figures/BTC_5min_BPVSignificantJumps_3.png}
%   \end{subfigure}\\%[1ex]
%   \begin{subfigure}{\linewidth}
%       \centering
%       \caption{Jump of \textbf{BTC-G} separated from \textbf{BPV}. From 1st January 2017 to 31st July 2019}\label{fig:jumps_sig_btcg}
%       \includegraphics[width=16cm]{figures/gemini_BTC_5min_BPVSignificantJumps_3.png}
%   \end{subfigure}
%     \caption{Jump Separation by $BPV$ estimator. The panels from top to bottom are the 5-minute logarithmic returns, realized volatility ($RV^{1/2}$), bipower volatility ($BPV^{1/2}$) and separated significant jump in square root form ($J^{1/2}$) under confidence level $\alpha=99.99\%$. Test for significant $J$ is detailed in Appendix\ref{app_jump_z_test}}\label{fig:jumps_sig}
% \end{figure}


% By the comparison between Fig.(\ref{fig:tjumps_sig}) with Fig.(\ref{fig:jumps_sig}), under confidence level $\alpha=99.99\%$, the threshold method $TBPV$ detects more significant jumps than $BPV$ method.
% We will further discuss the dynamics of those two estimators and compare the performance under forecasting models.
%
% \begin{figure}[!htb]
%   \begin{subfigure}{\linewidth}
%     \centering
%     \caption{BTC-D Jump separation from 1st January 2017 to 31st May 2019}\label{fig:tjumps_sig_btcd}
%     \includegraphics[width=16cm]{figures/BTC_5min_CTBPVSignificantJumps_3.png}
%     \end{subfigure}\\[1ex]
%     \begin{subfigure}{\linewidth}
%       \centering
%       \caption{BTC-G Jump separation from 1st January 2017 to 31st July 2019}\label{fig:tjumps_sig_btcg}
%       \includegraphics[width=16cm]{figures/gemini_BTC_5min_CTBPVSignificantJumps_3.png}
%     \end{subfigure}
%     \caption{The panels from top to bottom are logarithmic return, square-root form of realized volatility ($RV^{1/2}$), square-root form of threshold bipower variance ($TBPV^{1/2}$) with $c_{\theta}=3$ and separated significant jump process in square-root form ($J^{1/2}$) under confidence level $\alpha=99.99\%$}\label{fig:tjumps_sig}
%   \end{figure}


==> tabs/Tab_EconomicValue_logform.tex <==
%!TEX root = ../RCVJ.tex

\begin{table}[!htb]
  %% local redefinitions
  \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
  \renewrobustcmd{\boldmath}{}

  \centering % centering table
  \begin{threeparttable}
    \caption{Economic Values Evaluation of Log-Log Models Out-of-Sample Forecasts (\%)}\label{tab:economic_evaluation_logform}
    \footnotesize
    \begin{tabular}{l*{4}{S[table-format=1.3, table-number-alignment = center]}c*{4}{S[table-format=1.3, table-number-alignment = center]}} % ,table-number-alignment = center
  \toprule
  \toprule
  \multicolumn{1}{c}{}
  & \multicolumn{4}{c}{\textbf{BTC-D}}
  & \multicolumn{1}{c}{}
  & \multicolumn{4}{c}{\textbf{BTC-G}}
  \\
  \cline{3-4}
  \cline{8-9}
\\
  \multicolumn{1}{c}{}
  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RSV}
  &\multicolumn{1}{c}{RSVSJ}
  &\multicolumn{1}{c}{}
  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RSV}
  &\multicolumn{1}{c}{RSVSJ}

  \\
  \cline{2-5}
  \cline{7-10}
  \\

  \textbf{h=1}  & \bfseries 2.619 & 2.404 & 2.583           & 2.146           & & \bfseries 2.098 & 1.728 & 2.019 & 1.393           \\
  \textbf{h=7}  & 3.133           & 3.128 & 3.140           & \bfseries 3.143 & & \bfseries 2.793 & 2.549 & 2.710 & 2.631           \\
  \textbf{h=30} & 3.479           & 3.591 & \bfseries 3.671 & 3.665           & & 3.576           & 3.633 & 3.635 & \bfseries 3.662 \\

    \bottomrule
    \bottomrule
    \end{tabular}
% Day-ahead Forecast Regression Results on BTC-G, $\alpha=0.9999$, $c_{\theta}=3$, 5-minutes frequency
\begin{tablenotes}
  \scriptsize
  \item The table reports the economic value gained in terms of realized utility of BTC-D (left part) and BTC-G (right part).
  The columns of each part from left to right are realized utility from four different models including HAR, RVJ, RSV, and RSVSJ model detailed in section \ref{subsec:har_model}.
  Each of the forecasting models is in logarithmic form, and then the realized utility is calculated after transforming forecasts to squared form.
  The rows are realized utility in three different forecasting horizons, $h=1,7,30$.
  The highest utility of each forecasting horizon is bolded for both BTC-D and BTC-G.
  All the realized utility are reported in percentage.
\end{tablenotes}
\end{threeparttable}
  \end{table}


==> tabs/Tab_EconomicValue_squareform.tex <==
%!TEX root = ../RCVJ.tex


\begin{table}[H]
  %% local redefinitions
  \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}
  \renewrobustcmd{\boldmath}{}

  \centering % centering table
  \begin{threeparttable}
    \caption{Economic Values Evaluation of Out-of-Sample Forecasts (\%)}\label{tab:economic_evaluation_squareform}
    \footnotesize
    \begin{tabular}{l*{4}{S[table-format=1.3, table-number-alignment = center]}c*{4}{S[table-format=1.3, table-number-alignment = center]}} % ,table-number-alignment = center
  \toprule
  \toprule
  \multicolumn{1}{c}{}
  & \multicolumn{4}{c}{\textbf{BTC-D}}
  & \multicolumn{1}{c}{}
  & \multicolumn{4}{c}{\textbf{BTC-G}}
  \\
  \cline{3-4}
  \cline{8-9}
\\
  \multicolumn{1}{c}{}
  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RSV}
  &\multicolumn{1}{c}{RSVSJ}
  &\multicolumn{1}{c}{}
  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RSV}
  &\multicolumn{1}{c}{RSVSJ}

  \\
  \cline{2-5}
  \cline{7-10}
  \\

  \textbf{h=1}  & \bfseries 2.938 & 2.496 & 2.626           & 1.421     &  & \bfseries 2.650 & 1.330 & 2.041           & -1.843  \\
  \textbf{h=7}  & \bfseries 3.071 & 3.048 & 2.916           & 2.874     &  & \bfseries 3.164 & 1.862 & 2.906           & 1.100   \\
  \textbf{h=30} & 3.569           & 3.642 & \bfseries 3.708 & 3.678     &  & 3.585           & 3.637 & \bfseries 3.689 & 3.621   \\

    \bottomrule
    \bottomrule
    \end{tabular}
% Day-ahead Forecast Regression Results on BTC-G, $\alpha=0.9999$, $c_{\theta}=3$, 5-minutes frequency
\begin{tablenotes}
  \scriptsize
  \item The table reports the economic value gained in terms of realized utility of BTC-D (left part) and BTC-G (right part).
  The columns of each part from left to right are realized utility from four different models including HAR, RVJ, RSV, and RSVSJ model detailed in section \ref{subsec:har_model}.
  Each of the forecasting models is in squared form, and then the forecast is used to calculate the realized utility.
  The rows are realized utility in three different forecasting horizons, $h=1,7,30$.
  The highest utility of each forecasting horizon is bolded for both BTC-D and BTC-G.
  All the realized utility are reported in percentage.
\end{tablenotes}
\end{threeparttable}
  \end{table}


==> tabs/Tab_InSampleFit_BTCD_old.tex <==
%!TEX root = ../RCVJ.tex

\begin{landscape}

  \begin{table}[!ht]
    \centering % centering table
    \begin{threeparttable}

      \caption{Regression Results of Full-Sample Fitting, \textbf{BTC-D}}\label{tab:InSampleReg_BTCD}
      \scriptsize
      \begin{tabular}{l*{7}{S[table-format=1.2]}l*{7}{S[table-format=1.2]}} % ,table-number-alignment = center
        % >{\raggedleft\arraybackslash}p{5em}
    \toprule
    \toprule
    \multicolumn{1}{c}{\textbf{h=1}}&\multicolumn{7}{c}{\textbf{Square form}} & \multicolumn{1}{c}{} & \multicolumn{7}{c}{\textbf{Logarithmic form}}\\
    \cline{4-6}
    \cline{12-14}\\

    % \multicolumn{2}{c}{HAR:}
    % & \multicolumn{10}{l}{${RV}_{t,t+h}
    % =\alpha+\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} +\varepsilon_{t,t+1} $}\\
    % %
    % \multicolumn{2}{c}{RVJ:}
    % & \multicolumn{10}{l}{${RV}_{t,t+h}
    % =\alpha+\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} +
    % \beta_{JD} {J}_{D}+\beta_{JW} {J}_{W}+\beta_{JM} {J}_{M} + \varepsilon_{t,t+1} $}\\
    %
    % \multicolumn{2}{c}{RVTJ:}
    % & \multicolumn{10}{l}{${RV}_{t,t+h}
    % =\alpha+\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} +
    % \beta_{JD} {TJ}_{D}+\beta_{JW} {TJ}_{W}+\beta_{JM} {TJ}_{M} + \varepsilon_{t,t+1}$}\\
    %
    % \multicolumn{2}{c}{RV(T)SJ:}
    % & \multicolumn{10}{l}{
    % $\begin{array} {lll} {RV}_{t,t+h} & = & \alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} \\
    % & + & \beta_{JD}^{+} (T)J^{+}_{D}+\beta_{JW}^{+} (T)J^{+}_{W}+\beta_{JM}^{+} (T)J^{+}_{M}\\
    % & + & \beta_{JD}^{-} (T)J^{-}_{D}+\beta_{JW}^{-} (T)J^{-}_{W}+\beta_{JM}^{-} (T)J^{-}_{M} +\varepsilon_{t,t+h} \end{array}$
    % }\\


    % \multicolumn{10}{l}{RV(T)J$^{+(-)}$:${RV}_{t,t+h}=\alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M}$}\\
    % \multicolumn{2}{c}{RV(T)SJ:}
    % & \multicolumn{10}{l}{
    % $\begin{array} {rcl} {RV}_{t,t+h} & = & \alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} \\
    % & + & \beta_{JD}^{+} (T)J^{+}_{D}+\beta_{JW}^{+} (T)J^{+}_{W}+\beta_{JM}^{+} (T)J^{+}_{M}\\
    % & + & \beta_{JD}^{-} (T)J^{-}_{D}+\beta_{JW}^{-} (T)J^{-}_{W}+\beta_{JM}^{-} (T)J^{-}_{M} +\varepsilon_{t,t+h} \end{array}$
    % }\\
    \multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\alpha$}
    &\multicolumn{1}{c}{$\beta_{D}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{W}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{M}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JD}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JW}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JM}^{(+/-)}$}
    &\multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\alpha$}
    &\multicolumn{1}{c}{$\beta_{D}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{W}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{M}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JD}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JW}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JM}^{(+/-)}$}
    \\
\cmidrule{2-8}
\cmidrule{10-16}\\

  \multirow{2}{*}{HAR}                & 0.175   & 0.437    & 0.100    & 0.311   &          &          &          && -0.122   & 0.568    & 0.236   & 0.132    &          &          &          \\
              {}                      & (2.460) & (6.284)  & (2.119)  & (2.722) &          &          &          && (-4.341) & (15.758) & (5.387) & (2.797)                                   \\
                                                                                                                                                                                              \\
  \multirow{2}{*}{RVJ}                & 0.335   & 0.430    & 0.089    & 0.292   & 0.680    & -0.179   & -4.216   && -0.053   & 0.570    & 0.227   & 0.116    & -0.426   & -0.595   & -1.500   \\
              {}                      & (2.953) & (6.466)  & (1.862)  & (2.523) & (0.781)  & (-0.195) & (-2.494) && (-1.335) & (15.879) & (5.002) & (2.434)  & (-1.094) & (-1.151) & (-1.789) \\
                                                                                                                                                                                              \\
  \multirow{2}{*}{RVTJ}               & 0.271   & 0.457    & 0.089    & 0.292   & -0.476   & -0.046   & -0.538   && -0.006   & 0.600    & 0.225   & 0.096    & -0.574   & -0.534   & -0.489   \\
              {}                      & (1.696) & (6.470)  & (1.743)  & (2.452) & (-2.303) & (-0.112) & (-0.489) && (-0.147) & (17.108) & (4.745) & (2.164)  & (-3.053) & (-1.932) & (-1.35)  \\
                                                                                                                                                                                              \\
  \multirow{4}{*}{RVSJ$^{\dagger}$}   &         &          &          &         & -1.071   & -0.647   & -3.063   &&          &          &         &          & -0.514   & -1.308   & 0.299    \\
              {}                      & 0.382   & 0.431    & 0.065    & 0.521   & (-1.958) & (-0.572) & (-2.095) && 0.115    & 0.581    & 0.315   & 0.133    & (-2.139) & (-2.503) & (0.448)  \\\cline{6-8}\cline{14-16}
              {}                      & (2.464) & (3.785)  & (0.765)  & (3.224) & 0.800    & 1.126    & -4.111   && (1.171)  & (13.658) & (4.817) & (1.792)  & -0.134   & -0.91    & -0.943   \\
              {}                      &         &          &          &         & (0.515)  & (0.683)  & (-1.803) &&          &          &         &          & (-0.418) & (-1.301) & (-0.855) \\
                                                                                                                                                                                              \\
  \multirow{4}{*}{RVTSJ$^{\dagger}$}  &         &          &          &         & -1.357   & -0.925   & -1.547   &&          &          &         &          & -0.602   & -1.245   & 0.312    \\
              {}                      & 0.305   & 0.495    & 0.089    & 0.363   & (-3.593) & (-1.063) & (-1.210) && 0.097    & 0.605    & 0.301   & 0.103    & (-3.211) & (-3.225) & (0.555)  \\\cline{6-8}\cline{14-16}
              {}                      & (1.994) & (5.193)  & (1.134)  & (3.141) & -0.086   & 0.798    & -0.303   && (1.195)  & (13.871) & (4.841) & (1.778)  & -0.223   & -0.334   & -0.455   \\
              {}                      &         &          &          &         & (-0.138) & (1.085)  & (-0.198) &&          &          &         &          & (-0.98)  & (-0.768) & (-0.746) \\
                                                                                                                                                                                              \\
  \multirow{4}{*}{RSV$^{\dagger}$}    &         & -0.161   & -0.803   & -0.217  &          &          &          &&          & 0.202    & 0.045   & 0.069    &          &          &          \\
                {}                    & 0.170   & (-0.379) & (-1.599) & (-0.27) &          &          &          && 0.534    & (2.999)  & (0.434) & (0.519)  &          &          &          \\\cline{3-5}\cline{11-13}
                {}                    & (2.257) & 1.008    & 0.986    & 0.834   &          &          &          && (14.328) & 0.375    & 0.182   & 0.057    &          &          &          \\
                {}                    &         & (2.417)  & (1.877)  & (0.989) &          &          &          &&          & (5.939)  & (1.719) & (0.421)  &          &          &          \\
                                                                                                                                                                                              \\
  \multirow{4}{*}{RSVSJ$^{\dagger}$}  &         & 0.839    & -1.858   & 0.094   & -1.608   & 2.091    & -2.449   &&          & 0.233    & 0.126   & -0.005   & -0.319   & -1.228   & 0.574    \\
                {}                    & 0.407   & (0.615)  & (-1.069) & (0.023) & (-0.909) & (0.883)  & (-0.41)  && 0.833    & (3.025)  & (1.027) & (-0.027) & (-1.284) & (-2.255) & (0.728)  \\\cline{3-5}\cline{11-13}\cline{6-8}\cline{14-16}
                {}                    & (2.364) & 0.023    & 1.979    & 0.948   & 1.381    & -1.968   & -4.853   && (6.268)  & 0.349    & 0.182   & 0.137    & -0.157   & -0.989   & -1.279   \\
                {}                    &         & (0.015)  & (1.084)  & (0.231) & (0.473)  & (-0.471) & (-0.682) &&          & (4.473)  & (1.379) & (0.671)  & (-0.456) & (-1.23)  & (-0.902) \\
                                                                                                                                                                                              \\
  \multirow{4}{*}{RSVSTJ$^{\dagger}$} &         & -1.603   & -1.049   & 3.722   & 1.095    & 0.623    & -5.764   &&          & 0.255    & 0.212   & -0.005   & -0.454   & -1.367   & 0.542    \\
                {}                    & 0.317   & (-1.376) & (-0.629) & (0.656) & (0.827)  & (0.399)  & (-0.874) && 0.786    & (3.299)  & (1.713) & (-0.029) & (-2.164) & (-3.09)  & (0.755)  \\\cline{3-5}\cline{11-13}\cline{6-8}\cline{14-16}
                {}                    & (2.14)  & 2.568    & 1.176    & -2.905  & -2.307   & -0.446   & 3.128    && (7.646)  & 0.353    & 0.079   & 0.104    & -0.264   & -0.178   & -0.586   \\
                {}                    &         & (2.161)  & (0.682)  & (-0.52) & (-1.657) & (-0.228) & (0.482)  &&          & (4.557)  & (0.624) & (0.54)   & (-1.106) & (-0.363) & (-0.746) \\

      \bottomrule
      \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \scriptsize
        \item $\dagger$: Results from positive (above) and Negative (below) estimators are separated by horizontal lines.
        \item $t$-values are denoted with parantheses.
        \item Explain the details on regressions
      \end{tablenotes}
    \end{threeparttable}
    \end{table}
\end{landscape}


==> tabs/Tab_InSampleFit_BTCG.tex <==
\begin{landscape}

  \begin{table}[!htb]
    \centering % centering table
    \begin{threeparttable}

      \caption{Regression Results of Full-Sample Fitting, \textbf{BTC-G}}\label{tab:InSampleReg_BTCG}
      \scriptsize
      \begin{tabular}{l*{7}{S[table-format=1.2]}l*{7}{S[table-format=1.2]}} % ,table-number-alignment = center
        % >{\raggedleft\arraybackslash}p{5em}
    \toprule
    \toprule

    \multicolumn{1}{c}{\textbf{h=1}}&\multicolumn{7}{c}{\textbf{Square form}} & \multicolumn{1}{c}{} & \multicolumn{7}{c}{\textbf{Logarithmic form}}\\
    \cline{4-6}
    \cline{12-14}\\

    % \multicolumn{2}{c}{HAR:}
    % & \multicolumn{10}{l}{${RV}_{t,t+h}
    % =\alpha+\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} +\varepsilon_{t,t+1} $}\\
    % %
    % \multicolumn{2}{c}{RVJ:}
    % & \multicolumn{10}{l}{${RV}_{t,t+h}
    % =\alpha+\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} +
    % \beta_{JD} {J}_{D}+\beta_{JW} {J}_{W}+\beta_{JM} {J}_{M} + \varepsilon_{t,t+1} $}\\
    %
    % \multicolumn{2}{c}{RVTJ:}
    % & \multicolumn{10}{l}{${RV}_{t,t+h}
    % =\alpha+\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} +
    % \beta_{JD} {TJ}_{D}+\beta_{JW} {TJ}_{W}+\beta_{JM} {TJ}_{M} + \varepsilon_{t,t+1}$}\\
    %
    % \multicolumn{2}{c}{RV(T)SJ:}
    % & \multicolumn{10}{l}{
    % $\begin{array} {lll} {RV}_{t,t+h} & = & \alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} \\
    % & + & \beta_{JD}^{+} (T)J^{+}_{D}+\beta_{JW}^{+} (T)J^{+}_{W}+\beta_{JM}^{+} (T)J^{+}_{M}\\
    % & + & \beta_{JD}^{-} (T)J^{-}_{D}+\beta_{JW}^{-} (T)J^{-}_{W}+\beta_{JM}^{-} (T)J^{-}_{M} +\varepsilon_{t,t+h} \end{array}$
    % }\\


    % \multicolumn{10}{l}{RV(T)J$^{+(-)}$:${RV}_{t,t+h}=\alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M}$}\\
    % \multicolumn{2}{c}{RV(T)SJ:}
    % & \multicolumn{10}{l}{
    % $\begin{array} {rcl} {RV}_{t,t+h} & = & \alpha +\beta_D {RV}_{D} +\beta_W {RV}_{W} +\beta_M {RV}_{M} \\
    % & + & \beta_{JD}^{+} (T)J^{+}_{D}+\beta_{JW}^{+} (T)J^{+}_{W}+\beta_{JM}^{+} (T)J^{+}_{M}\\
    % & + & \beta_{JD}^{-} (T)J^{-}_{D}+\beta_{JW}^{-} (T)J^{-}_{W}+\beta_{JM}^{-} (T)J^{-}_{M} +\varepsilon_{t,t+h} \end{array}$
    % }\\
    \multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\alpha$}
    &\multicolumn{1}{c}{$\beta_{D}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{W}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{M}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JD}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JW}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JM}^{(+/-)}$}
    &\multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\alpha$}
    &\multicolumn{1}{c}{$\beta_{D}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{W}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{M}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JD}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JW}^{(+/-)}$}
    &\multicolumn{1}{c}{$\beta_{JM}^{(+/-)}$}
    \\
\cmidrule{2-8}
\cmidrule{10-16}\\

  \multirow{2}{*}{HAR}                & 0.178   & 0.333    & 0.163    & 0.326    &          &          &          && -0.182   & 0.532    & 0.262   & 0.127    &          &          &          \\
              {}                      & (2.315) & (4.560)  & (3.016)  & (2.654)  &          &          &          && (-5.267) & (16.773) & (6.793) & (2.856)  &          &          &          \\
                                                                                                                                                                                               \\
  \multirow{2}{*}{RVJ}                & 0.278   & 0.379    & 0.175    & 0.273    & -0.493   & -0.500   & -0.372   && -0.048   & 0.528    & 0.301   & 0.107    & -0.436   & -0.863   & -0.51    \\
              {}                      & (3.591) & (5.110)  & (2.677)  & (2.251)  & (-2.676) & (-1.977) & (-0.824) && (-0.981) & (16.499) & (7.329) & (2.462)  & (-2.17)  & (-3.112) & (-1.425) \\
                                                                                                                                                                                               \\
  \multirow{2}{*}{RVTJ}               & 0.302   & 0.393    & 0.171    & 0.259    & -0.333   & -0.241   & -0.266   && -0.002   & 0.55     & 0.313   & 0.071    & -0.412   & -0.643   & -0.232   \\
              {}                      & (3.94)  & (4.732)  & (2.446)  & (2.045)  & (-2.106) & (-1.596) & (-0.877) && (-0.032) & (16.423) & (7.01)  & (1.525)  & (-2.452) & (-3.275) & (-0.835) \\
                                                                                                                                                                                               \\
  \multirow{4}{*}{RVSJ$^{\dagger}$}   &         &          &          &          & -1.347   & -3.877   & -3.297   &&          &          &         &          & -0.584   & -1.875   & -0.954   \\
              {}                      & 0.513   & 0.424    & 0.343    & 0.414    & (-2.356) & (-2.565) & (-1.467) && 0.254    & 0.543    & 0.376   & 0.158    & (-1.828) & (-3.856) & (-0.896) \\\cline{6-8}\cline{14-16}
              {}                      & (4.279) & (4.243)  & (2.858)  & (2.21)   & -0.502   & -0.434   & -0.605   && (1.828)  & (13.176) & (6.949) & (2.351)  & -0.252   & -0.805   & -0.673   \\
              {}                      &         &          &          &          & (-1.769) & (-1.771) & (-1.300) &&          &          &         &          & (-0.872) & (-2.862) & (-1.553) \\
                                                                                                                                                                                               \\
  \multirow{4}{*}{RVTSJ$^{\dagger}$}  &         &          &          &          & -1.211   & -2.857   & -2.372   &&          &          &         &          & -0.658   & -1.64    & -0.52    \\
              {}                      & 0.519   & 0.437    & 0.304    & 0.348    & (-2.857) & (-2.593) & (-1.631) && 0.226    & 0.555    & 0.373   & 0.113    & (-2.615) & (-3.839) & (-0.661) \\\cline{6-8}\cline{14-16}
              {}                      & (5.051) & (4.347)  & (2.745)  & (2.199)  & -0.219   & 0.173    & -0.194   && (1.968)  & (13.653) & (6.69)  & (1.873)  & -0.141   & -0.349   & -0.445   \\
              {}                      &         &          &          &          & (-0.941) & (1.022)  & (-0.526) &&          &          &         &          & (-0.673) & (-1.473) & (-1.303) \\
                                                                                                                                                                                               \\
  \multirow{4}{*}{RSV$^{\dagger}$}    &         & 0.406    & -0.216   & 0.382    &          &          &          &&          & 0.238    & 0.103   & 0.235    &          &          &          \\
                {}                    & 0.169   & (1.289)  & (-0.619) & (0.719)  &          &          &          && 0.485    & (4.129)  & (1.032) & (2.205)  &          &          &          \\\cline{3-5}\cline{11-13}
                {}                    & (2.048) & 0.267    & 0.501    & 0.302    &          &          &          && (10.05)  & 0.303    & 0.146   & -0.109   &          &          &          \\
                {}                    &         & (0.856)  & (1.45)   & (0.621)  &          &          &          &&          & (5.47)   & (1.566) & (-0.98)  &          &          &          \\
                                                                                                                                                                                               \\
  \multirow{4}{*}{RSVSJ$^{\dagger}$}  &         & -0.862   & -0.883   & -2.210   & 0.640    & -2.097   & 0.582    &&          & 0.268    & 0.229   & 0.218    & -0.490   & -1.969   & -1.422   \\
                {}                    & 0.421   & (-1.544) & (-0.526) & (-0.830) & (0.634)  & (-0.752) & (0.136)  && 1.009    & (3.665)  & (1.768) & (1.101)  & (-1.413) & (-3.457) & (-1.124) \\\cline{3-5}\cline{11-13}\cline{6-8}\cline{14-16}
                {}                    & (3.819) & 1.633    & 1.512    & 3.027    & -1.761   & -1.75    & -3.478   && (5.733)  & 0.279    & 0.132   & -0.063   & -0.21    & -0.648   & -0.362   \\
                {}                    &         & (3.089)  & (0.934)  & (1.155)  & (-2.949) & (-1.035) & (-1.254) &&          & (3.848)  & (1.163) & (-0.324) & (-0.698) & (-2.16)  & (-0.594) \\
                                                                                                                                                                                               \\
  \multirow{4}{*}{RSVSTJ$^{\dagger}$} &         & -0.671   & -3.545   & -7.760   & 0.085    & 1.586    & 7.011    &&          & 0.317    & 0.259   & 0.150    & -0.689   & -1.799   & -0.710   \\
                {}                    & 0.443   & (-0.574) & (-1.207) & (-1.058) & (0.058)  & (0.541)  & (0.861)  && 0.949    & (4.115)  & (1.883) & (0.715)  & (-2.241) & (-3.397) & (-0.689) \\\cline{3-5}\cline{11-13}\cline{6-8}\cline{14-16}
                {}                    & (4.441) & 1.511    & 4.076    & 8.361    & -1.329   & -3.779   & -8.551   && (6.580)  & 0.247    & 0.100   & -0.044   & -0.06    & -0.152   & -0.228   \\
                {}                    &         & (1.289)  & (1.359)  & (1.123)  & (-1.044) & (-1.251) & (-1.109) &&          & (3.271)  & (0.84)  & (-0.213) & (-0.258) & (-0.557) & (-0.385) \\

      \bottomrule
      \bottomrule
      \end{tabular}

      \begin{tablenotes}
        \scriptsize
        \item $\dagger$: Results from positive (above) and Negative (below) estimators are separated by horizontal lines.
      \end{tablenotes}
    \end{threeparttable}
    \end{table}


\end{landscape}


==> tabs/Tab_InSampleFit_RSV_final_BTCG.tex <==
%!TEX root = ../RCVJ.tex

\begin{landscape}

  \begin{table}[!ht]
    \centering % centering table
    \begin{threeparttable}

      \caption{Full-Sample Fitting Regression Results of Signed Estimators}\label{tab:InSampleReg_SRVtype_BTCDG}
      \scriptsize
      \begin{tabular}{l*{6}{S[table-format=1.2]}cl*{6}{S[table-format=1.2]}c} % ,table-number-alignment = center

        \multicolumn{5}{l}{\textbf{RSV:} $\log\left(RV_{t,t+h}\right) = \alpha + \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \varepsilon_{t,t+h}$}
        &\multicolumn{1}{c}{} & \multicolumn{9}{l}{\textbf{RSVSJ:} $\log\left(RV_{t,t+h}\right) = \alpha+ \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \log\left(X_{J^{+-}}^{\top}\right)\beta_{J^{+-}} + \varepsilon_{t,t+h}$}\T\B\B\\
        % \multicolumn{1}{c}{RSV:} & \multicolumn{14}{l}{$\log\left(RV_{t,t+h}\right) = \alpha + \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \varepsilon_{t,t+h}$} \T\B\B\\
        % \multicolumn{1}{c}{RSVSJ:} & \multicolumn{14}{l}{$\log\left(RV_{t,t+h}\right) = \alpha+ \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \log\left(X_{J^{+-}}^{\top}\right)\beta_{J^{+-}} + \varepsilon_{t,t+h}$}\T\B\B\\
        \multicolumn{16}{l}{Regressors vectors $\log\left(X_{RSV}^{\top}\right)=\left(\log(RSV_{D}^+), \log(RSV_{W}^+), \log(RSV_{M}^+), \log(RSV_{D}^-), \log(RSV_{W}^-), \log(RSV_{M}^-)\right)$, }\T\B\B\\
        \multicolumn{16}{l}{and $\log(X_{J^{+-}}^{\top})=\left(\log(J_{D}^{+}+1), \log(J_{W}^{+}+1), \log(J_{M}^{+}+1), \log(J_{D}^{-}+1), \log(J_{W}^{-}+1), \log(J_{M}^{-}+1)\right)$}\T\B\B\\
        \multicolumn{16}{l}{Parameters vectors: $\beta_{RSV}=\left(\beta_{D}^{+},\beta_{W}^{+},\beta_{M}^{+}, \beta_{D}^{-},\beta_{W}^{-},\beta_{M}^{-}\right)^{\top}$,
        and $\beta_{J^{+-}}=\left(\beta_{JD}^{+},\beta_{JW}^{+},\beta_{JM}^{+}, \beta_{JD}^{-},\beta_{JW}^{-},\beta_{JM}^{-}\right)^{\top}$}\T\B\B\\


    \toprule
    \toprule
    \multicolumn{1}{c}{}&\multicolumn{7}{c}{\textbf{BTC-D}} & \multicolumn{1}{c}{} & \multicolumn{7}{c}{\textbf{BTC-G}}\\
    \cline{4-6}
    \cline{12-14}\\
    \multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\beta_{D}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{W}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{M}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JD}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JW}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JM}^{+/-}$}
    &\multicolumn{1}{c}{M-Z R$^2$}
    &\multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\beta_{D}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{W}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{M}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JD}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JW}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JM}^{+/-}$}
    &\multicolumn{1}{c}{M-Z R$^2$}
    \\
\cmidrule{2-8}
\cmidrule{10-16}\\

\multicolumn{2}{c}{\textbf{h=1}}\\
\cline{1-2}


\multirow{4}{*}{RSV}    & 0.202    & 0.045    & 0.069    &          &          &          & \multirow{4}{*}{0.339} && 0.238    & 0.103    & 0.235    &          &          &          & \multirow{4}{*}{0.259}\\
              {}                    & (2.999)  & (0.434)  & (0.519)  &          &          &          &                        && (4.129)  & (1.032)  & (2.205)  &          &          &          &                       \\\cline{2-4}\cline{10-12}
              {}                    & 0.375    & 0.182    & 0.057    &          &          &          &                        && 0.303    & 0.146    & -0.109   &          &          &          &                       \\
              {}                    & (5.939)  & (1.719)  & (0.421)  &          &          &          &                        && (5.47)   & (1.566)  & (-0.98)  &          &          &          &                       \\\\
\multirow{4}{*}{RSVSJ}   & 0.255    & 0.212    & -0.005   & -0.454   & -1.367   & 0.542    & \multirow{4}{*}{0.360} && 0.317    & 0.259    & 0.150    & -0.689   & -1.799   & -0.710   & \multirow{4}{*}{0.299}\\
              {}                    & (3.299)  & (1.713)  & (-0.029) & (-2.164) & (-3.09)  & (0.755)  &                        && (4.115)  & (1.883)  & (0.715)  & (-2.241) & (-3.397) & (-0.689) &                       \\\cline{2-4}\cline{10-12}\cline{5-7}\cline{13-15}
              {}                    & 0.353    & 0.079    & 0.104    & -0.264   & -0.178   & -0.586   &                        && 0.247    & 0.100    & -0.044   & -0.060   & -0.152   & -0.228   &                       \\
              {}                    & (4.557)  & (0.624)  & (0.54)   & (-1.106) & (-0.363) & (-0.746) &                        && (3.271)  & (0.840)  & (-0.213) & (-0.258) & (-0.557) & (-0.385) &                       \\


  \multicolumn{2}{c}{\textbf{h=7}}                                                                                                                                                                                        \\
  \cline{1-2}

  \multirow{4}{*}{RSV}  & 0.156   & 0.012   & 0.273    &          &          &          & \multirow{4}{*}{0.351} && 0.170   & 0.122    & 0.368    &          &          &          & \multirow{4}{*}{0.323}\\
                {}                  & (2.463) & (0.058) & (0.892)  &          &          &          &                        && (2.944) & (0.671)  & (1.311)  &          &          &          &                       \\\cline{2-4}\cline{10-12}
                {}                  & 0.230   & 0.192   & -0.033   &          &          &          &                        && 0.18    & 0.077    & -0.165   &          &          &          &                       \\
                {}                  & (3.972) & (0.935) & (-0.1)   &          &          &          &                        && (3.226) & (0.453)  & (-0.574) &          &          &          &                       \\\\
  \multirow{4}{*}{RSVSJ} & 0.293   & 0.386   & 0.341    & -0.989   & -2.345   & -0.825   & \multirow{4}{*}{0.362} && 0.340   & 0.389    & 0.354    & -1.246   & -1.998   & -3.376   & \multirow{4}{*}{0.381}\\
                {}                  & (4.456) & (1.632) & (0.785)  & (-4.011) & (-2.672) & (-0.581) &                        && (4.667) & (1.544)  & (0.707)  & (-4.516) & (-2.492) & (-1.74)  &                       \\\cline{2-4}\cline{10-12}\cline{5-7}\cline{13-15}
                {}                  & 0.169   & -0.141  & -0.071   & -0.456   & 0.474    & -1.101   &                        && 0.086   & -0.196   & 0.001    & -0.088   & 0.929    & -0.977   &                       \\
                {}                  & (2.544) & (-0.57) & (-0.153) & (-2.001) & (0.443)  & (-0.536) &                        && (1.164) & (-0.876) & (0.003)  & (-0.43)  & (1.673)  & (-0.815) &                       \\

  \multicolumn{2}{c}{\textbf{h=30}}                                                                                                                                                                                       \\
  \cline{1-2}


  \multirow{4}{*}{RSV}  & 0.093    & 0.033    & 0.489    &          &          &          & \multirow{4}{*}{0.402} && 0.082    & 0.039    & 0.348    &          &          &          & \multirow{4}{*}{0.430}\\
                {}                  & (1.234)  & (0.134)  & (0.916)  &          &          &          &                        && (1.498)  & (0.27)   & (1.014)  &          &          &          &                       \\\cline{2-4}\cline{10-12}
                {}                  & 0.122    & 0.121    & -0.191   &          &          &          &                        && 0.08     & 0.101    & -0.117   &          &          &          &                       \\
                {}                  & (2.362)  & (0.518)  & (-0.334) &          &          &          &                        && (1.947)  & (0.731)  & (-0.305) &          &          &          &                       \\\\
  \multirow{4}{*}{RSVSJ} & 0.195   & 0.272    & 0.583    & -0.743   & -1.52    & -2.978  & \multirow{4}{*}{0.388} && 0.185    & 0.239    & -0.095   & -0.77    & -2.039   & -3.162   & \multirow{4}{*}{0.469}\\
                {}                  & (3.493) & (1.252)  & (0.659)  & (-3.533) & (-2.422) & (-1.514)  &                        && (3.199)  & (1.664)  & (-0.162) & (-4.088) & (-3.769) & (-1.28)  &                       \\\cline{2-4}\cline{10-12}\cline{5-7}\cline{13-15}
                {}                  & 0.07    & -0.101   & -0.071   & -0.354   & -0.095   & -3.716  &                        && -0.011   & -0.046   & 0.579    & 0.098    & 0.336    & -3.214   &                       \\
                {}                  & (1.648) & (-0.464) & (-0.075) & (-1.213) & (-0.112) & (-1.281) &                        && (-0.313) & (-0.347) & (1.012)  & (0.668)  & (1.107)  & (-2.193) &                       \\

      \bottomrule
      \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \footnotesize
      \end{tablenotes}
    \end{threeparttable}
    \end{table}




\end{landscape}

































































==> tabs/Tab_InSampleFit_RV_final_BTCG.tex <==
%!TEX root = ../RCVJ.tex

% \begin{landscape}

%   \begin{table}[!ht]
%     \centering % centering table
%     \begin{threeparttable}
%       \caption{}\label{tab:InSampleReg_RVtype_BTCDG}
%       \scriptsize
%       \begin{tabular}{l*{6}{S[table-format=1.2]}cl*{6}{S[table-format=1.2]}c} % ,table-number-alignment = center

%         \multicolumn{5}{l}{\textbf{HAR:} $\log\left(RV_{t,t+h}\right)=\alpha+ \log\left(X_{RV}^{\top}\right)\beta_{RV} +\varepsilon_{t,t+h}$}
%         &\multicolumn{1}{c}{} & \multicolumn{8}{l}{\textbf{RVJ:} $\log\left(RV_{t,t+h}\right)=\alpha+ \log\left(X_{RV}^{\top}\right)\beta_{RV}+ \log\left(X_{J}^{\top}\right)\beta_{J}+\varepsilon_{t,t+h}$}\T\B\B\\
%         % \multicolumn{1}{c}{RVJ:} & \multicolumn{14}{l}{$\log\left(RV_{t,t+h}\right)=\alpha+ \log\left(X_{RV}^{\top}\right)\beta_{RV}+ \log\left(X_{J}^{\top}\right)\beta_{J}+\varepsilon_{t,t+h}$}\T\B\B\\
%         \multicolumn{16}{l}{Regressors vectors: $\log\left(X_{RV}^{\top}\right)=\left(\log(RV_{D}), \log(RV_{W}), \log(RV_{M})\right)$,
%         and $\log\left(X_{J}^{\top}\right)=\left(\log(J_{D}+1), \log(J_{W}+1), \log(J_{M}+1)\right)$}\T\B\B\\
%         \multicolumn{16}{l}{Parameters vectors: $\beta_{RV}=\left(\beta_{D},\beta_{W},\beta_{M}\right)^{\top}$,
%         and $\beta_{J}= \left(\beta_{JD},\beta_{JW},\beta_{JM}\right)^{\top}$}\T\B\B\\

%     \toprule
%     \toprule
%     \multicolumn{1}{c}{}&\multicolumn{7}{c}{\textbf{BTC-D}}\\
%     \cline{4-6}
%     \cline{12-14}\\

%     \multicolumn{1}{c}{}
%     &\multicolumn{1}{c}{$\beta_{D}$}
%     &\multicolumn{1}{c}{$\beta_{W}$}
%     &\multicolumn{1}{c}{$\beta_{M}$}
%     &\multicolumn{1}{c}{$\beta_{JD}$}
%     &\multicolumn{1}{c}{$\beta_{JW}$}
%     &\multicolumn{1}{c}{$\beta_{JM}$}
%     &\multicolumn{1}{c}{M-Z R$^2$}
%     &\multicolumn{1}{c}{}
%     &\multicolumn{1}{c}{$\beta_{D}$}
%     &\multicolumn{1}{c}{$\beta_{W}$}
%     &\multicolumn{1}{c}{$\beta_{M}$}
%     &\multicolumn{1}{c}{$\beta_{JD}$}
%     &\multicolumn{1}{c}{$\beta_{JW}$}
%     &\multicolumn{1}{c}{$\beta_{JM}$}
%     &\multicolumn{1}{c}{M-Z R$^2$}
%     \\
% \cmidrule{2-8}
% \cmidrule{10-16}\\

% \multicolumn{2}{c}{\textbf{h=1}}\\
% \cline{1-2}

%   \multirow{2}{*}{HAR} & 0.568    & 0.236   & 0.132   &          &          &          &\multirow{2}{*}{0.333} && 0.532    & 0.262   & 0.127   &          &          &          &\multirow{2}{*}{0.255} \\
%               {}       & (15.758) & (5.387) & (2.797) &          &          &          &                       && (16.773) & (6.793) & (2.856) &          &          &          &                       \\\\
%   \multirow{2}{*}{RVJ} & 0.600    & 0.225   & 0.096   & -0.574   & -0.534   & -0.489   &\multirow{2}{*}{0.330} && 0.550     & 0.313   & 0.071   & -0.412   & -0.643   & -0.232   &\multirow{2}{*}{0.248} \\
%               {}       & (17.108) & (4.745) & (2.164) & (-3.053) & (-1.932) & (-1.350) &                       && (16.423) & (7.01)  & (1.525) & (-2.452) & (-3.275) & (-0.835) &                       \\\\

%   \multicolumn{2}{c}{\textbf{h=7}}                                                                                                                                                                      \\
%   \cline{1-2}


%   \multirow{2}{*}{HAR} & 0.374    & 0.209   & 0.248   &          &          &          &\multirow{2}{*}{0.348} && 0.342    & 0.208   & 0.203   &          &          &          &\multirow{2}{*}{0.319} \\
%               {}       & (9.679)  & (3.199) & (2.439) &          &          &          &                       && (8.917)  & (3.473) & (2.556) &          &          &          &                       \\\\
%   \multirow{2}{*}{RVJ} & 0.417    & 0.175   & 0.21    & -0.811   & -0.684   & -2.057   &\multirow{2}{*}{0.327} && 0.393    & 0.158   & 0.233   & -0.605   & 0.019    & -1.312   &\multirow{2}{*}{0.323} \\
%               {}       & (10.367) & (2.435) & (2.13)  & (-4.258) & (-1.078) & (-2.426) &                       && (9.605)  & (2.405) & (2.819) & (-3.791) & (0.049)  & (-2.48)  &                       \\\\

%   \multicolumn{2}{c}{\textbf{h=30}}                                                                                                                                                                     \\
%   \cline{1-2}


%   \multirow{2}{*}{HAR} & 0.202    & 0.15    & 0.312   &          &          &          &\multirow{2}{*}{0.397} && 0.154    & 0.149   & 0.228   &          &          &          &\multirow{2}{*}{0.417} \\
%               {}       & (5.199)  & (1.885) & (2.783) &          &          &          &                       && (5.046)  & (2.642) & (1.703) &          &          &          &                       \\\\
%   \multirow{2}{*}{RVJ} & 0.222    & 0.125   & 0.268   & -0.750    & -1.237   & -4.386   &\multirow{2}{*}{0.366} && 0.155    & 0.138   & 0.293   & -0.340    & -0.402   & -2.366   &\multirow{2}{*}{0.416} \\
%               {}       & (6.117)  & (1.519) & (2.602) & (-3.343) & (-1.833) & (-4.972) &                       && (4.831)  & (2.201) & (2.934) & (-2.015) & (-1.121) & (-5.339) &                       \\\\

%       \bottomrule
%       \bottomrule
%       \end{tabular}
%       \begin{tablenotes}
%         \footnotesize
%       \end{tablenotes}
%     \end{threeparttable}
%     \end{table}

% \end{landscape}














==> tabs/Tab_InSampleFit_RVtype_BTCDG.tex <==
%!TEX root = ../RCVJ.tex

\begin{landscape}

  \begin{table}[!ht]
    \centering % centering table
    \begin{threeparttable}
      \caption{Full-Sample Fitting Regression Results of Unsigned Estimators}\label{tab:InSampleReg_RVtype_BTCDG}
      \scriptsize
      \begin{tabular}{l*{6}{S[table-format=1.2]}cl*{6}{S[table-format=1.2]}c} % ,table-number-alignment = center

        \multicolumn{5}{l}{\textbf{HAR:} $\log\left(RV_{t,t+h}\right)=\alpha+ \log\left(X_{RV}^{\top}\right)\beta_{RV} +\varepsilon_{t,t+h}$}
        &\multicolumn{1}{c}{} & \multicolumn{8}{l}{\textbf{RVJ:} $\log\left(RV_{t,t+h}\right)=\alpha+ \log\left(X_{RV}^{\top}\right)\beta_{RV}+ \log\left(X_{J}^{\top}\right)\beta_{J}+\varepsilon_{t,t+h}$}\T\B\B\\
        % \multicolumn{1}{c}{RVJ:} & \multicolumn{14}{l}{$\log\left(RV_{t,t+h}\right)=\alpha+ \log\left(X_{RV}^{\top}\right)\beta_{RV}+ \log\left(X_{J}^{\top}\right)\beta_{J}+\varepsilon_{t,t+h}$}\T\B\B\\
        \multicolumn{16}{l}{Regressors vectors: $\log\left(X_{RV}^{\top}\right)=\left(\log(RV_{D}), \log(RV_{W}), \log(RV_{M})\right)$,
        and $\log\left(X_{J}^{\top}\right)=\left(\log(J_{D}+1), \log(J_{W}+1), \log(J_{M}+1)\right)$}\T\B\B\\
        \multicolumn{16}{l}{Parameters vectors: $\beta_{RV}=\left(\beta_{D},\beta_{W},\beta_{M}\right)^{\top}$,
        and $\beta_{J}= \left(\beta_{JD},\beta_{JW},\beta_{JM}\right)^{\top}$}\T\B\B\\

    \toprule
    \toprule
    \multicolumn{1}{c}{}&\multicolumn{7}{c}{\textbf{BTC-D}} & \multicolumn{1}{c}{} & \multicolumn{7}{c}{\textbf{BTC-G}}\\
    \cline{4-6}
    \cline{12-14}\\

    \multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\beta_{D}$}
    &\multicolumn{1}{c}{$\beta_{W}$}
    &\multicolumn{1}{c}{$\beta_{M}$}
    &\multicolumn{1}{c}{$\beta_{JD}$}
    &\multicolumn{1}{c}{$\beta_{JW}$}
    &\multicolumn{1}{c}{$\beta_{JM}$}
    &\multicolumn{1}{c}{M-Z R$^2$}
    &\multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\beta_{D}$}
    &\multicolumn{1}{c}{$\beta_{W}$}
    &\multicolumn{1}{c}{$\beta_{M}$}
    &\multicolumn{1}{c}{$\beta_{JD}$}
    &\multicolumn{1}{c}{$\beta_{JW}$}
    &\multicolumn{1}{c}{$\beta_{JM}$}
    &\multicolumn{1}{c}{M-Z R$^2$}
    \\
\cmidrule{2-8}
\cmidrule{10-16}\\

\multicolumn{2}{c}{\textbf{h=1}}\\
\cline{1-2}

  \multirow{2}{*}{HAR} & 0.568    & 0.236   & 0.132   &          &          &          &\multirow{2}{*}{0.333} && 0.532    & 0.262   & 0.127   &          &          &          &\multirow{2}{*}{0.255} \\
              {}       & (15.758) & (5.387) & (2.797) &          &          &          &                       && (16.773) & (6.793) & (2.856) &          &          &          &                       \\\\
  \multirow{2}{*}{RVJ} & 0.600    & 0.225   & 0.096   & -0.574   & -0.534   & -0.489   &\multirow{2}{*}{0.330} && 0.550     & 0.313   & 0.071   & -0.412   & -0.643   & -0.232   &\multirow{2}{*}{0.248} \\
              {}       & (17.108) & (4.745) & (2.164) & (-3.053) & (-1.932) & (-1.350) &                       && (16.423) & (7.01)  & (1.525) & (-2.452) & (-3.275) & (-0.835) &                       \\\\

  \multicolumn{2}{c}{\textbf{h=7}}                                                                                                                                                                      \\
  \cline{1-2}


  \multirow{2}{*}{HAR} & 0.374    & 0.209   & 0.248   &          &          &          &\multirow{2}{*}{0.348} && 0.342    & 0.208   & 0.203   &          &          &          &\multirow{2}{*}{0.319} \\
              {}       & (9.679)  & (3.199) & (2.439) &          &          &          &                       && (8.917)  & (3.473) & (2.556) &          &          &          &                       \\\\
  \multirow{2}{*}{RVJ} & 0.417    & 0.175   & 0.21    & -0.811   & -0.684   & -2.057   &\multirow{2}{*}{0.327} && 0.393    & 0.158   & 0.233   & -0.605   & 0.019    & -1.312   &\multirow{2}{*}{0.323} \\
              {}       & (10.367) & (2.435) & (2.13)  & (-4.258) & (-1.078) & (-2.426) &                       && (9.605)  & (2.405) & (2.819) & (-3.791) & (0.049)  & (-2.48)  &                       \\\\

  \multicolumn{2}{c}{\textbf{h=30}}                                                                                                                                                                     \\
  \cline{1-2}


  \multirow{2}{*}{HAR} & 0.202    & 0.15    & 0.312   &          &          &          &\multirow{2}{*}{0.397} && 0.154    & 0.149   & 0.228   &          &          &          &\multirow{2}{*}{0.417} \\
              {}       & (5.199)  & (1.885) & (2.783) &          &          &          &                       && (5.046)  & (2.642) & (1.703) &          &          &          &                       \\\\
  \multirow{2}{*}{RVJ} & 0.222    & 0.125   & 0.268   & -0.750    & -1.237   & -4.386   &\multirow{2}{*}{0.366} && 0.155    & 0.138   & 0.293   & -0.340    & -0.402   & -2.366   &\multirow{2}{*}{0.416} \\
              {}       & (6.117)  & (1.519) & (2.602) & (-3.343) & (-1.833) & (-4.972) &                       && (4.831)  & (2.201) & (2.934) & (-2.015) & (-1.121) & (-5.339) &                       \\\\

      \bottomrule
      \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \footnotesize
        \item The table contains results for BTC-D (left-hand side part) and BTC-G (right-hand side part).
        Each of the panel of the two parts reports the regression results of HAR and RVJ models.
        Panels from top to bottom are realized variance forecasts in three different horizons, $h=1,7,30$.
        The first six columns of each panel show the coefficients and the last column is the Adj-R$^2$.
        The $t$-value is in the parenthesis.
        All parameters are estimated by OLS using Newey-West covariance matrix estimator with 7, 14 and 60 lags for $h=1,7,30$, respectively.
      \end{tablenotes}
    \end{threeparttable}
    \end{table}

\end{landscape}


==> tabs/Tab_InSampleFit_SRVtype_BTCDG.tex <==
%!TEX root = ../RCVJ.tex

\begin{landscape}

  \begin{table}[!ht]
    \centering % centering table
    \begin{threeparttable}

      \caption{Full-Sample Fitting Regression Results of Signed Estimators}\label{tab:InSampleReg_SRVtype_BTCDG}
      \scriptsize
      \begin{tabular}{l*{6}{S[table-format=1.2]}cl*{6}{S[table-format=1.2]}c} % ,table-number-alignment = center

        \multicolumn{5}{l}{\textbf{RSV:} $\log\left(RV_{t,t+h}\right) = \alpha + \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \varepsilon_{t,t+h}$}
        &\multicolumn{1}{c}{} & \multicolumn{9}{l}{\textbf{RSVSJ:} $\log\left(RV_{t,t+h}\right) = \alpha+ \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \log\left(X_{J^{+-}}^{\top}\right)\beta_{J^{+-}} + \varepsilon_{t,t+h}$}\T\B\B\\
        % \multicolumn{1}{c}{RSV:} & \multicolumn{14}{l}{$\log\left(RV_{t,t+h}\right) = \alpha + \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \varepsilon_{t,t+h}$} \T\B\B\\
        % \multicolumn{1}{c}{RSVSJ:} & \multicolumn{14}{l}{$\log\left(RV_{t,t+h}\right) = \alpha+ \log\left(X_{RSV}^{\top}\right)\beta_{RSV} + \log\left(X_{J^{+-}}^{\top}\right)\beta_{J^{+-}} + \varepsilon_{t,t+h}$}\T\B\B\\
        \multicolumn{16}{l}{Regressors vectors $\log\left(X_{RSV}^{\top}\right)=\left(\log(RSV_{D}^+), \log(RSV_{W}^+), \log(RSV_{M}^+), \log(RSV_{D}^-), \log(RSV_{W}^-), \log(RSV_{M}^-)\right)$, }\T\B\B\\
        \multicolumn{16}{l}{and $\log(X_{J^{+-}}^{\top})=\left(\log(J_{D}^{+}+1), \log(J_{W}^{+}+1), \log(J_{M}^{+}+1), \log(J_{D}^{-}+1), \log(J_{W}^{-}+1), \log(J_{M}^{-}+1)\right)$}\T\B\B\\
        \multicolumn{16}{l}{Parameters vectors: $\beta_{RSV}=\left(\beta_{D}^{+},\beta_{W}^{+},\beta_{M}^{+}, \beta_{D}^{-},\beta_{W}^{-},\beta_{M}^{-}\right)^{\top}$,
        and $\beta_{J^{+-}}=\left(\beta_{JD}^{+},\beta_{JW}^{+},\beta_{JM}^{+}, \beta_{JD}^{-},\beta_{JW}^{-},\beta_{JM}^{-}\right)^{\top}$}\T\B\B\\


    \toprule
    \toprule
    \multicolumn{1}{c}{}&\multicolumn{7}{c}{\textbf{BTC-D}} & \multicolumn{1}{c}{} & \multicolumn{7}{c}{\textbf{BTC-G}}\\
    \cline{4-6}
    \cline{12-14}\\
    \multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\beta_{D}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{W}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{M}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JD}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JW}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JM}^{+/-}$}
    &\multicolumn{1}{c}{M-Z R$^2$}
    &\multicolumn{1}{c}{}
    &\multicolumn{1}{c}{$\beta_{D}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{W}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{M}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JD}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JW}^{+/-}$}
    &\multicolumn{1}{c}{$\beta_{JM}^{+/-}$}
    &\multicolumn{1}{c}{M-Z R$^2$}
    \\
\cmidrule{2-8}
\cmidrule{10-16}\\

\multicolumn{2}{c}{\textbf{h=1}}\\
\cline{1-2}


\multirow{4}{*}{RSV}    & 0.202    & 0.045    & 0.069    &          &          &          & \multirow{4}{*}{0.339} && 0.238    & 0.103    & 0.235    &          &          &          & \multirow{4}{*}{0.259}\\
              {}                    & (2.999)  & (0.434)  & (0.519)  &          &          &          &                        && (4.129)  & (1.032)  & (2.205)  &          &          &          &                       \\\cline{2-4}\cline{10-12}
              {}                    & 0.375    & 0.182    & 0.057    &          &          &          &                        && 0.303    & 0.146    & -0.109   &          &          &          &                       \\
              {}                    & (5.939)  & (1.719)  & (0.421)  &          &          &          &                        && (5.47)   & (1.566)  & (-0.98)  &          &          &          &                       \\\\
\multirow{4}{*}{RSVSJ}   & 0.255    & 0.212    & -0.005   & -0.454   & -1.367   & 0.542    & \multirow{4}{*}{0.360} && 0.317    & 0.259    & 0.150    & -0.689   & -1.799   & -0.710   & \multirow{4}{*}{0.299}\\
              {}                    & (3.299)  & (1.713)  & (-0.029) & (-2.164) & (-3.09)  & (0.755)  &                        && (4.115)  & (1.883)  & (0.715)  & (-2.241) & (-3.397) & (-0.689) &                       \\\cline{2-4}\cline{10-12}\cline{5-7}\cline{13-15}
              {}                    & 0.353    & 0.079    & 0.104    & -0.264   & -0.178   & -0.586   &                        && 0.247    & 0.100    & -0.044   & -0.060   & -0.152   & -0.228   &                       \\
              {}                    & (4.557)  & (0.624)  & (0.54)   & (-1.106) & (-0.363) & (-0.746) &                        && (3.271)  & (0.840)  & (-0.213) & (-0.258) & (-0.557) & (-0.385) &                       \\


  \multicolumn{2}{c}{\textbf{h=7}}                                                                                                                                                                                        \\
  \cline{1-2}

  \multirow{4}{*}{RSV}  & 0.156   & 0.012   & 0.273    &          &          &          & \multirow{4}{*}{0.351} && 0.170   & 0.122    & 0.368    &          &          &          & \multirow{4}{*}{0.323}\\
                {}                  & (2.463) & (0.058) & (0.892)  &          &          &          &                        && (2.944) & (0.671)  & (1.311)  &          &          &          &                       \\\cline{2-4}\cline{10-12}
                {}                  & 0.230   & 0.192   & -0.033   &          &          &          &                        && 0.18    & 0.077    & -0.165   &          &          &          &                       \\
                {}                  & (3.972) & (0.935) & (-0.1)   &          &          &          &                        && (3.226) & (0.453)  & (-0.574) &          &          &          &                       \\\\
  \multirow{4}{*}{RSVSJ} & 0.293   & 0.386   & 0.341    & -0.989   & -2.345   & -0.825   & \multirow{4}{*}{0.362} && 0.340   & 0.389    & 0.354    & -1.246   & -1.998   & -3.376   & \multirow{4}{*}{0.381}\\
                {}                  & (4.456) & (1.632) & (0.785)  & (-4.011) & (-2.672) & (-0.581) &                        && (4.667) & (1.544)  & (0.707)  & (-4.516) & (-2.492) & (-1.74)  &                       \\\cline{2-4}\cline{10-12}\cline{5-7}\cline{13-15}
                {}                  & 0.169   & -0.141  & -0.071   & -0.456   & 0.474    & -1.101   &                        && 0.086   & -0.196   & 0.001    & -0.088   & 0.929    & -0.977   &                       \\
                {}                  & (2.544) & (-0.57) & (-0.153) & (-2.001) & (0.443)  & (-0.536) &                        && (1.164) & (-0.876) & (0.003)  & (-0.43)  & (1.673)  & (-0.815) &                       \\

  \multicolumn{2}{c}{\textbf{h=30}}                                                                                                                                                                                       \\
  \cline{1-2}


  \multirow{4}{*}{RSV}  & 0.093    & 0.033    & 0.489    &          &          &          & \multirow{4}{*}{0.402} && 0.082    & 0.039    & 0.348    &          &          &          & \multirow{4}{*}{0.430}\\
                {}                  & (1.234)  & (0.134)  & (0.916)  &          &          &          &                        && (1.498)  & (0.27)   & (1.014)  &          &          &          &                       \\\cline{2-4}\cline{10-12}
                {}                  & 0.122    & 0.121    & -0.191   &          &          &          &                        && 0.08     & 0.101    & -0.117   &          &          &          &                       \\
                {}                  & (2.362)  & (0.518)  & (-0.334) &          &          &          &                        && (1.947)  & (0.731)  & (-0.305) &          &          &          &                       \\\\
  \multirow{4}{*}{RSVSJ} & 0.195   & 0.272    & 0.583    & -0.743   & -1.52    & -2.978  & \multirow{4}{*}{0.388} && 0.185    & 0.239    & -0.095   & -0.77    & -2.039   & -3.162   & \multirow{4}{*}{0.469}\\
                {}                  & (3.493) & (1.252)  & (0.659)  & (-3.533) & (-2.422) & (-1.514)  &                        && (3.199)  & (1.664)  & (-0.162) & (-4.088) & (-3.769) & (-1.28)  &                       \\\cline{2-4}\cline{10-12}\cline{5-7}\cline{13-15}
                {}                  & 0.07    & -0.101   & -0.071   & -0.354   & -0.095   & -3.716  &                        && -0.011   & -0.046   & 0.579    & 0.098    & 0.336    & -3.214   &                       \\
                {}                  & (1.648) & (-0.464) & (-0.075) & (-1.213) & (-0.112) & (-1.281) &                        && (-0.313) & (-0.347) & (1.012)  & (0.668)  & (1.107)  & (-2.193) &                       \\

      \bottomrule
      \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \footnotesize
        \item The table contains results for BTC-D (left-hand side part) and BTC-G (right-hand side part).
        Each of the panel of the two parts reports the regression results of RSV and RSVSJ models.
        Panels from top to bottom are realized variance forecasts in three different horizons, $h=1,7,30$.
        The first six columns of each panel show the coefficients and the last column is the Adj-R$^2$.
        Each regression model of the three panels is separated by line in which upper (bottom) part reports the results of the positive (negative) signed estimators.
        The $t$-value is in the parenthesis.
        All parameters are estimated by OLS using Newey-West covariance matrix estimator with 7, 14 and 60 lags for $h=1,7,30$, respectively.
      \end{tablenotes}
    \end{threeparttable}
    \end{table}




\end{landscape}


==> tabs/Tab_OutOfSampleForecasts_logform.tex <==
% !TEX root = ../RCVJ.tex

\begin{table}[!htb]
  \centering % centering table
  \begin{threeparttable}
    \caption{Adaptive Log-Log HAR Models Out-of-Sample Forecasts Performance Evaluation}\label{tab:OutSampleForecasts_logform}
    \footnotesize
    \begin{tabular}{l*{4}{S[table-format=1.2, table-number-alignment = center]}c*{4}{S[table-format=1.2, table-number-alignment = center]}} % ,table-number-alignment = center
  \toprule
  \toprule
  \multicolumn{1}{c}{}
  & \multicolumn{4}{c}{\textbf{BTC-D}}
  & \multicolumn{1}{c}{}
  & \multicolumn{4}{c}{\textbf{BTC-G}}
  \\
  \cline{3-4}
  \cline{8-9}
\\
  \multicolumn{1}{c}{}
  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RSV}
  &\multicolumn{1}{c}{RSVSJ}
  &\multicolumn{1}{c}{}
  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RSV}
  &\multicolumn{1}{c}{RSVSJ}

  \\
  \cline{2-5}
  \cline{7-10}
  \\
  \multicolumn{1}{l}{\textbf{h=1}}                                                                                                             \\
  \cline{1-3}
  MZ-R$^2$             & 0.299 & 0.287              & 0.289              & 0.241             & & 0.261 & 0.218              & 0.266             & 0.235              \\
  MSE                  & 3.260 & 3.356              & 3.313              & 3.680             & & 2.217 & 2.353              & 2.209             & 2.298              \\
  HRMSE                & 0.760 & 0.822 $^{\dagger}$ & 0.807$^{\dagger}$  & 0.937$^{\dagger}$ & & 0.979 & 1.004              & 0.985             & 1.143              \\
  QLIKE                & 0.902 & 0.972              & 0.920              & 1.085$^{\dagger}$ & & 0.906 & 1.017              & 0.945             & 1.170$^{\dagger}$  \\ \\

  \multicolumn{1}{l}{\textbf{h=7}}                                                                                                             \\
  \cline{1-3}
  MZ-R$^2$             & 0.327 & 0.366              & 0.333              & 0.392             & & 0.329 & 0.277              & 0.352             & 0.406              \\
  MSE                  & 1.576 & 1.514              & 1.691              & 1.588             & & 0.949 & 1.016              & 0.955             & 0.931              \\
  HRMSE                & 0.881 & 0.903              & 1.091 $^{\dagger}$ & 0.969             & & 0.908 & 0.989 $^{\dagger}$ & 0.888             & 0.971              \\
  QLIKE                & 0.946 & 0.947              & 0.946              & 0.930             & & 0.906 & 1.001 $^{\dagger}$ & 0.929             & 0.978              \\ \\

  \multicolumn{1}{l}{\textbf{h=30}}                                                                                                            \\
  \cline{1-3}
  MZ-R$^2$             & 0.504 & 0.680              & 0.569              & 0.604             & & 0.591 & 0.635              & 0.632             & 0.708              \\
  MSE                  & 0.729 & 0.488\oneS         & 0.611\oneS         & 0.584\oneS        & & 0.348 & 0.305\oneS         & 0.307\oneS        & 0.247\oneS         \\
  HRMSE                & 0.628 & 0.488\oneS         & 0.543\oneS         & 0.451\oneS        & & 0.582 & 0.549\oneS         & 0.509\oneS        & 0.384\oneS         \\
  QLIKE                & 0.965 & 0.910\oneS         & 0.885\oneS         & 0.878\oneS        & & 0.773 & 0.746\oneS         & 0.744\oneS        & 0.725\oneS         \\

    \bottomrule
    \bottomrule
    \end{tabular}
% Day-ahead Forecast Regression Results on BTC-G, $\alpha=0.9999$, $c_{\theta}=3$, 5-minutes frequency
\begin{tablenotes}
  \scriptsize
  \item The table reports the out-of-sample forecasting performance of BTC-D (left part) and BTC-D (right part) in different forecasting horizons $h=1,7,30$ separated into three panels.
  The columns of each panel from left to right are HAR, RVJ, RSV, and RSVSJ models detailed in section \ref{subsec:har_model}.
  The rows of each panel from top to down are R$^2$ of Mincer-Zarnowitz forecasting regression, mean squared error, heteroscedasticity adjusted root mean squared error, and mean of gaussian quasi-likelihood error.
  The $\dagger$ marks when the HAR model outperforms significantly other models, while the $*$ denotes that the HAR model underperforms other models significantly, and the significance is confirmed by D-M test at 5\% significant level.
  The forecasts are conducted in logarithmic forms, and then transformed by to squared form for the performance evaluation.
\end{tablenotes}
\end{threeparttable}
  \end{table}


==> tabs/Tab_OutOfSampleForecasts_old.tex <==
% !TEX root = ../RCVJ.tex

\begin{landscape}
  \begin{table}[!htb]
    \centering % centering table
    \begin{threeparttable}
      \caption{Adaptive HAR Model Out-of-Sample Forecasts Performance Evaluation}\label{tab:OutSampleForecasts}
      \scriptsize
      \begin{tabular}{l*{8}{S[table-format=1.1, table-number-alignment = center]}c*{8}{S[table-format=1.1, table-number-alignment = center]}} % ,table-number-alignment = center
    \toprule
    \toprule
    \multicolumn{1}{c}{}
    & \multicolumn{8}{c}{\textbf{BTC-D}}
    & \multicolumn{1}{c}{}
    & \multicolumn{8}{c}{\textbf{BTC-G}}
    \\
    \cline{5-6}
    \cline{14-15}
\\
    \multicolumn{1}{c}{}
    &\multicolumn{1}{c}{HAR}
    &\multicolumn{1}{c}{RVJ}
    &\multicolumn{1}{c}{RVTJ}
    &\multicolumn{1}{c}{RVSJ}
    &\multicolumn{1}{c}{RVSTJ}
    &\multicolumn{1}{c}{RSV}
    &\multicolumn{1}{c}{RSVSJ}
    &\multicolumn{1}{c}{RSVSTJ}
    &\multicolumn{1}{c}{}
    &\multicolumn{1}{c}{HAR}
    &\multicolumn{1}{c}{RVJ}
    &\multicolumn{1}{c}{RVTJ}
    &\multicolumn{1}{c}{RVSJ}
    &\multicolumn{1}{c}{RVSTJ}
    &\multicolumn{1}{c}{RSV}
    &\multicolumn{1}{c}{RSVSJ}
    &\multicolumn{1}{c}{RSVSTJ}

    \\
    % \midrule
    \cline{2-9}
    \cline{11-18}
    \\
    \multicolumn{2}{l}{\textbf{Square form}}\\
    \cline{1-3}
    \multicolumn{2}{c}{}&\multicolumn{1}{l}{\textbf{h=1}}\\
    MZ-R$^2$                   & 0.267 & 0.227              & 0.248              & 0.228              & 0.219              & 0.285              & 0.215              & 0.165             &
                               & 0.213 & 0.179              & 0.182              & 0.182              & 0.190              & 0.226              & 0.144              & 0.151 \\
    MSE                        & 3.636 & 4.023$^{\dagger}$  & 3.850              & 4.032              & 3.984              & 3.676              & 4.414$^{\dagger}$  & 4.812$^{\dagger}$ &
                               & 2.437 & 2.537              & 2.508              & 2.682              & 2.580              & 2.411              & 2.943              & 2.872 \\
    HRMSE                      & 1.569 & 2.031 $^{\dagger}$ & 1.576              & 1.792$^{\dagger}$  & 1.737$^{\dagger}$  & 1.767$^{\dagger}$  & 1.841$^{\dagger}$  & 1.756$^{\dagger}$ &
                               & 1.976 & 2.251 $^{\dagger}$ & 2.080              & 2.497$^{\dagger}$  & 2.385$^{\dagger}$  & 2.022              & 2.762$^{\dagger}$  & 2.583$^{\dagger}$ \\
    QLIKE                      & 0.846 & 1.151 $^{\dagger}$ & 1.100 $^{\dagger}$ & 1.000 $^{\dagger}$ & 1.172$^{\dagger}$  & 0.988$^{\dagger}$  & 1.176$^{\dagger}$  & 1.545$^{\dagger}$ &
                               & 0.749 & 1.418 $^{\dagger}$ & 1.636 $^{\dagger}$ & 3.367$^{\dagger}$  & 2.406$^{\dagger}$  & 1.139$^{\dagger}$  & 3.548$^{\dagger}$  & 4.706$^{\dagger}$ \\ \\

    \cline{1-3}
    \multicolumn{2}{c}{}       &\multicolumn{1}{l}{\textbf{h=7}} \\
    MZ-R$^2$                   & 0.365 & 0.360              & 0.416              & 0.440              & 0.470              & 0.431       & 0.508              & 0.458       &
                               & 0.355 & 0.349              & 0.360              & 0.420              & 0.425              & 0.424       & 0.481              & 0.435 \\
    MSE                        & 1.643 & 1.789 $^{\dagger}$ & 1.437              & 1.552              & 1.285 \oneS        & 1.573       & 1.328\oneS         & 1.272 \oneS &
                               & 0.990 & 0.905              & 0.888              & 0.889              & 0.830 \oneS        & 0.875 \oneS & 0.812\oneS         & 0.818\oneS \\
    HRMSE                      & 1.359 & 1.646 $^{\dagger}$ & 1.278              & 1.358              & 1.303              & 1.455       & 1.243              & 1.279       &
                               & 1.278 & 1.433 $^{\dagger}$ & 1.366 $^{\dagger}$ & 1.247              & 1.305              & 1.050 \oneS & 1.232              & 1.624 \\
    QLIKE                      & 0.984 & 1.146 $^{\dagger}$ & 0.997              & 1.026              & 0.996              & 1.037       & 0.880 \oneS        & 1.043       &
                               & 0.797 & 1.152 $^{\dagger}$ & 1.341 $^{\dagger}$ & 1.818 $^{\dagger}$ & 1.618 $^{\dagger}$ & 0.878       & 1.679 $^{\dagger}$ & 1.738 $^{\dagger}$ \\ \\


    \cline{1-3}
    \multicolumn{2}{c}{}       &\multicolumn{1}{l}{\textbf{h=30}} \\
    MZ-R$^2$                   & 0.543 & 0.583      & 0.682      & 0.717      & 0.623      & 0.628      & 0.743      & 0.677      &
                               & 0.635 & 0.667      & 0.682      & 0.702      & 0.693      & 0.707      & 0.791      & 0.813 \\
    MSE                        & 0.673 & 0.649      & 0.462\oneS & 0.398\oneS & 0.558\oneS & 0.514\oneS & 0.357\oneS & 0.440\oneS &
                               & 0.314 & 0.261\oneS & 0.256\oneS & 0.243\oneS & 0.239\oneS & 0.235\oneS & 0.178\oneS & 0.147\oneS \\
    HRMSE                      & 0.779 & 0.637\oneS & 0.614\oneS & 0.525\oneS & 0.528\oneS & 0.698\oneS & 0.483\oneS & 0.444\oneS &
                               & 0.696 & 0.611\oneS & 0.554\oneS & 0.490\oneS & 0.487\oneS & 0.529\oneS & 0.456\oneS & 0.404\oneS \\
    QLIKE                      & 0.937 & 0.943      & 0.898\oneS & 0.847\oneS & 0.883\oneS & 0.877\oneS & 0.842\oneS & 0.874\oneS &
                               & 0.770 & 0.725\oneS & 0.743\oneS & 0.727\oneS & 0.754      & 0.722\oneS & 0.715\oneS & 0.741 \\ \\

    \multicolumn{2}{l}{\textbf{Logarithmic form}} \\
    \cline{1-3}
    \multicolumn{2}{c}{}       &\multicolumn{1}{l}{\textbf{h=1}} \\
    MZ-R$^2$                   & 0.299 & 0.264              & 0.287              & 0.239              & 0.265              & 0.289              & 0.236              & 0.241             &
                               & 0.261 & 0.221              & 0.218              & 0.238              & 0.249              & 0.266              & 0.243              & 0.235 \\
    MSE                        & 3.260 & 3.419$^{\dagger}$  & 3.356              & 3.657              & 3.501              & 3.313              & 3.773              & 3.680             &
                               & 2.217 & 2.329              & 2.353              & 2.284              & 2.260              & 2.209              & 2.262              & 2.298 \\
    HRMSE                      & 0.760 & 0.893$^{\dagger}$  & 0.822 $^{\dagger}$ & 0.963$^{\dagger}$  & 0.898$^{\dagger}$  & 0.807$^{\dagger}$  & 1.022$^{\dagger}$  & 0.937$^{\dagger}$ &
                               & 0.979 & 0.986              & 1.004              & 1.167              & 1.118              & 0.985              & 1.161              & 1.143 \\
    QLIKE                      & 0.902 & 0.950              & 0.972              & 0.902              & 0.956              & 0.920              & 0.985              & 1.085$^{\dagger}$ &
                               & 0.906 & 0.998$^{\dagger}$  & 1.017              & 1.056$^{\dagger}$  & 1.074$^{\dagger}$  & 0.945              & 1.112$^{\dagger}$  & 1.170$^{\dagger}$\\ \\

    \cline{1-3}
    \multicolumn{2}{c}{}       &\multicolumn{1}{l}{\textbf{h=7}} \\
    MZ-R$^2$                   & 0.327 & 0.330              & 0.366              & 0.381              & 0.443              & 0.333              & 0.374              & 0.392             &
                               & 0.329 & 0.281              & 0.277              & 0.344              & 0.377              & 0.352              & 0.352              & 0.406 \\
    MSE                        & 1.576 & 1.642              & 1.514              & 1.530              & 1.459              & 1.691              & 1.657              & 1.588             &
                               & 0.949 & 1.014              & 1.016              & 0.968              & 0.912              & 0.955              & 1.082              & 0.931 \\
    HRMSE                      & 0.881 & 1.209              & 0.903              & 1.027              & 1.080              & 1.091 $^{\dagger}$ & 0.986              & 0.969             &
                               & 0.908 & 0.906              & 0.989 $^{\dagger}$ & 0.865              & 0.862              & 0.888              & 1.022              & 0.971 \\
    QLIKE                      & 0.946 & 1.008 $^{\dagger}$ & 0.947              & 0.917              & 0.904              & 0.946              & 0.907              & 0.930             &
                               & 0.906 & 0.909              & 1.001 $^{\dagger}$ & 1.000              & 1.009 $^{\dagger}$ & 0.929              & 0.945              & 0.978 \\ \\

    \cline{1-3}
    \multicolumn{2}{c}{}       &\multicolumn{1}{l}{\textbf{h=30}} \\
    MZ-R$^2$                   & 0.504 & 0.549      & 0.680      & 0.604      & 0.591      & 0.569      & 0.639      & 0.604      &
                               & 0.591 & 0.626      & 0.635      & 0.651      & 0.671      & 0.632      & 0.678      & 0.708 \\
    MSE                        & 0.729 & 0.681\oneS & 0.488\oneS & 0.531\oneS & 0.616\oneS & 0.611\oneS & 0.489\oneS & 0.584\oneS &
                               & 0.348 & 0.303\oneS & 0.305\oneS & 0.288\oneS & 0.276\oneS & 0.307\oneS & 0.267\oneS & 0.247\oneS \\
    HRMSE                      & 0.628 & 0.493\oneS & 0.488\oneS & 0.691      & 0.654      & 0.543\oneS & 0.459\oneS & 0.451\oneS &
                               & 0.582 & 0.514\oneS & 0.549\oneS & 0.481\oneS & 0.461\oneS & 0.509\oneS & 0.397\oneS & 0.384\oneS \\
    QLIKE                      & 0.965 & 0.936\oneS & 0.910\oneS & 0.900\oneS & 0.891\oneS & 0.885\oneS & 0.872\oneS & 0.878\oneS &
                               & 0.773 & 0.731\oneS & 0.746\oneS & 0.726\oneS & 0.736\oneS & 0.744\oneS & 0.715\oneS & 0.725\oneS \\

      \bottomrule
      \bottomrule
      \end{tabular}
  % Day-ahead Forecast Regression Results on BTC-G, $\alpha=0.9999$, $c_{\theta}=3$, 5-minutes frequency
  \begin{tablenotes}
    \scriptsize
    \item All jumps are estimated under confidence level $\alpha=99.99\%$.
    \item $\dagger$: Better forecasts from HAR model against of any other models by D-M test at 5\% significant level.
    \item $*$: Worse forecasts from HAR model against of any other models by D-M test at 5\% significant level.
  \end{tablenotes}
  \end{threeparttable}
    \end{table}
\end{landscape}


==> tabs/Tab_OutOfSampleForecasts_squareform.tex <==
% !TEX root = ../RCVJ.tex

\begin{table}[H]
  \centering % centering table
  \begin{threeparttable}
    \caption{Adaptive HAR Model Out-of-Sample Forecasts Performance Evaluation}\label{tab:OutSampleForecasts_squareform}
    \footnotesize
    \begin{tabular}{l*{4}{S[table-format=1.2, table-number-alignment = center]}c*{4}{S[table-format=1.2, table-number-alignment = center]}} % ,table-number-alignment = center
  \toprule
  \toprule
  \multicolumn{1}{c}{}
  & \multicolumn{4}{c}{\textbf{BTC-D}}
  & \multicolumn{1}{c}{}
  & \multicolumn{4}{c}{\textbf{BTC-G}}
  \\
  \cline{3-4}
  \cline{8-9}
\\
  \multicolumn{1}{c}{}
  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RSV}
  &\multicolumn{1}{c}{RSVSJ}
  &\multicolumn{1}{c}{}
  &\multicolumn{1}{c}{HAR}
  &\multicolumn{1}{c}{RVJ}
  &\multicolumn{1}{c}{RSV}
  &\multicolumn{1}{c}{RSVSJ}

  \\
  \cline{2-5}
  \cline{7-10}
  \\
  \multicolumn{1}{l}{\textbf{h=1}}\\
  \cline{1-3}
  MZ-R$^2$             & 0.267 & 0.248              & 0.285              & 0.165             & & 0.213 & 0.182              & 0.226             & 0.151              \\
  MSE                  & 3.636 & 3.850              & 3.676              & 4.812$^{\dagger}$ & & 2.437 & 2.508              & 2.411             & 2.872              \\
  HRMSE                & 1.569 & 1.576              & 1.767$^{\dagger}$  & 1.756$^{\dagger}$ & & 1.976 & 2.080              & 2.022             & 2.583$^{\dagger}$  \\
  QLIKE                & 0.846 & 1.100 $^{\dagger}$ & 0.988$^{\dagger}$  & 1.545$^{\dagger}$ & & 0.749 & 1.636 $^{\dagger}$ & 1.139$^{\dagger}$ & 4.706$^{\dagger}$  \\ \\

  \multicolumn{1}{l}{\textbf{h=7}}                                                                                                             \\
  \cline{1-3}
  MZ-R$^2$             & 0.365 & 0.416              & 0.431              & 0.458             & & 0.355 & 0.360              & 0.424             & 0.435              \\
  MSE                  & 1.643 & 1.437              & 1.573              & 1.272 \oneS       & & 0.990 & 0.888              & 0.875 \oneS       & 0.818\oneS         \\
  HRMSE                & 1.359 & 1.278              & 1.455              & 1.279             & & 1.278 & 1.366 $^{\dagger}$ & 1.050 \oneS       & 1.624              \\
  QLIKE                & 0.984 & 0.997              & 1.037              & 1.043             & & 0.797 & 1.341 $^{\dagger}$ & 0.878             & 1.738 $^{\dagger}$ \\ \\


  \multicolumn{1}{l}{\textbf{h=30}}                                                                                                            \\
  \cline{1-3}
  MZ-R$^2$             & 0.543 & 0.682              & 0.628              & 0.677             & & 0.635 & 0.682              & 0.707             & 0.813              \\
  MSE                  & 0.673 & 0.462\oneS         & 0.514\oneS         & 0.440\oneS        & & 0.314 & 0.256\oneS         & 0.235\oneS        & 0.147\oneS         \\
  HRMSE                & 0.779 & 0.614\oneS         & 0.698\oneS         & 0.444\oneS        & & 0.696 & 0.554\oneS         & 0.529\oneS        & 0.404\oneS         \\
  QLIKE                & 0.937 & 0.898\oneS         & 0.877\oneS         & 0.874\oneS        & & 0.770 & 0.743\oneS         & 0.722\oneS        & 0.741              \\ \\

    \bottomrule
    \bottomrule
    \end{tabular}
% Day-ahead Forecast Regression Results on BTC-G, $\alpha=0.9999$, $c_{\theta}=3$, 5-minutes frequency
\begin{tablenotes}
  \scriptsize
  \item The table reports the out-of-sample forecasting performance of BTC-D (left part) and BTC-D (right part) in different forecasting horizons $h=1,7,30$ separated into three panels.
  The columns of each panel from left to right are HAR, RVJ, RSV, and RSVSJ models detailed in section \ref{subsec:har_model}.
  The rows of each panel from top to down are R$^2$ of Mincer-Zarnowitz forecasting regression, mean squared error, heteroscedasticity adjusted root mean squared error, and mean of gaussian quasi-likelihood error.
  The $\dagger$ marks when the HAR model outperforms significantly other models, while the $*$ denotes that the HAR model underperforms other models significantly, ant the significance is confirmed by D-M test at 5\% significant level.
  The forecasts are conducted in the squared forms and then used for the performance evaluation.
\end{tablenotes}
\end{threeparttable}
  \end{table}

